Thermodynamic Formalism for Generalized Markov Shifts on Infinitely Many States

Given a 0-1 infinite matrix $A$ and its countable Markov shift $\Sigma_A$, one of the authors and M. Laca have introduced a kind of {\it generalized countable Markov shift} $X_A=\Sigma_A \cup Y_A$, where $Y_A$ is a special set of finite admissible words. For some of the most studied countable Markov shifts $\Sigma_A$, $X_A$ is a compactification of $\Sigma_A$, and always it is at least locally compact. We developed the thermodynamic formalism on the space $X_A$, exploring the connections with standard results on $\Sigma_A$. New phenomena appear, such as new conformal measures and a {\it length-type phase transition}: the eigenmeasure lives on $\Sigma_A$ at high temperature and lives on $Y_A$ at low temperature. Using a pressure-point definition proposed by M. Denker and M. Yuri for iterated function systems, we proved that the Gurevich pressure is a natural definition for the pressure function in the generalized setting. For the gauge action, the Gurevich entropy is a critical temperature for the existence of new conformal measures (KMS states) living on $Y_A$. We exhibit examples with infinitely (even uncountable) many new extremal conformal measures, undetectable in the usual formalism. We prove that conformal measures always exist at low temperatures when the potential is coercive enough. We characterized a basis of the topology of $X_A$ to study the weak$^*$ convergence of measures on $X_A$, and we show some cases where the conformal measure living on $Y_A$ converges to a conformal one living on $\Sigma_A$. We prove the equivalence among several notions of conformality for locally compact Hausdorff second countable spaces, including quasi-invariant measures for generalized Renault-Deaconu groupoids.

==> paper_velho.tex <==

\subsection{Conformal measures}\\





%%%%%%%% Noções de conformidade

 Consider $X$ a locally compact, Hausdorff and second countable topological space endowed with a local homeomorphism  $\sigma:U \to X$, $U$ open subset of $X$. Let $\mathcal{G}(X,\sigma)$ be its respective Renault-Deaconu groupoid. For a given continuous potential $F:U \to \mathbb{R}$ and inverse of the temperature $\beta >0$, we define, inspired in the Ruelle operator, the Ruelle transformation $L_{-\beta F}$ as
\begin{align}
    L_{-\beta F}:C_c(U) &\to C_c(X) \nonumber\\
    f  & \mapsto L_{-\beta F}(f)(x):= \sum_{\sigma(y)=x}e^{-\beta F(y)}f(y).\label{eq:general_Ruelle}
\end{align}  


%Note that we cannot simply define such operator on $C_c(X)$ since we could have, e.g., $f$ supported on a neighborhood of $x \in \partial U \setminus U$, and we could set a sequence $x_n \to x$ such that $\sigma(x_n)=y$ and that would give an infinite set of elements of $\mathcal{G}(X,\sigma)$ in the form $\gamma_n = (x_n,1,\sigma(x_n)) = (x_n,1,\sigma(x_n))$, and therefore the series in \eqref{eq:general_Ruelle} could diverge. Also inspired on the classical CITAR case we define the notion of conformal measure in the sense of the Ruelle transformation as below.

\begin{definition}[Eigenmeasure associated to the Ruelle Transformation] Given the Borel $\sigma$-algebra $\mathbb{B}$ on $X$, $\sigma:U \to X$ the shift map defined in this section, $F:U \to \mathbb{R}$ a continuous potential and $\beta >0$. A measure $\mu$ on $\mathbb{B}$ is said to be a \textit{eigenmeasure} (with eigenvalue 1) for the Ruelle transformation $L_{-\beta F}$ when
\begin{equation}\label{eq:conformal_eigenmeasure_functions}
    \int_{X} L_{-\beta F}(f)(x)d\mu(x) = \int_{U} f(x)d\mu(x),
\end{equation}
for all $f \in C_c(U)$.
\end{definition}
In other words, the equation \eqref{eq:conformal_eigenmeasure_functions} can be rewritten by using \eqref{eq:general_Ruelle} as
\begin{equation}\label{eq:conformal_eigenmeasure_functions_2}
    \int_{X} \sum_{\sigma(y) = x} e^{-\beta F(y)}f(y) d\mu(x) = \int_{U} f(x)d\mu(x),
\end{equation}
for all $f \in C_c(U)$. As in the standard theory of countable Markov shifts, when a measure $m$ satisfies the equation \eqref{eq:conformal_eigenmeasure_functions_2} we write $L_{-\beta F}^*\mu =\mu$.

On the classical theory we have different notions of conformal measure and, in some cases, they are equivalent. A very important one is the conformal measure in the sense of Denker and Urba\'nski \cite{DenUr1991}, which was originally introduced by Patterson \cite{Pa}.


\begin{definition}[Conformal measure - Denker-Urba\'nski] Let $(X,\mathcal{F})$ be a measurable space, $\sigma:U\subseteq X \to X$ a measurable endomorphism and $D:U \to [0,\infty)$ also measurable. A set $A\subseteq U$ is called special if $A\in \mathcal{F}$ and $\sigma_A:=\sigma\restriction_A: A\to \sigma(A)$ is injective. A measure $\mu$ in $X$ is said to be $D$-conformal in the sense of Denker-Urba\'nski if
\begin{equation}\label{eq:conformal_Ur_sets_potential}
    \mu(\sigma(A)) = \int_A D d\mu,
\end{equation}
for all special sets $A$.
\end{definition}

\begin{definition}
Let $X$ be a locally compact Hausdorff and second countable topological space. Let $\sigma:U\subseteq X\to X$ a local homeomorphism. Given a borel measure $\mu$ on $X$ we define the measure $\mu\odot\sigma$ on $U$ by
$$\mu\odot\sigma(E):=\sum_{i\in \mathbb{N}}\mu(\sigma(E_i)).$$
For all measurable $E\subseteq U$, where the $E_i$ are pairwise disjoint measurable sets such that $\sigma\restriction E_i$ is injective, for each $i$, and $E =\sqcup_i E_i$. 


\end{definition}

\begin{remark}
We show that $\mu\odot\sigma$ is well defined. First we prove the existence of at least one countable family $\{E_i\}$, as above. Indeed, if $E\subseteq U$, since $\sigma$ is a local homeomorphism for each $x\in$ E there is an open subset $H_x\ni x$ such that $\sigma$ is injective, we have $E\subseteq \cup_{x\in E} H_x$. For each of those $H_x$ there is an open basic set $U_x$ such that $x\in U_x$, but the topology basis is countable, so we can enumerate $\{U_x\}=\{U_1,U_2,...\}$ and we observe that $\sigma$ is injective on each $U_i$. Take $E_1:=E\cap U_1$, $E_n:=E\cap U_n\setminus\bigsqcup_{i=1}^{n-1}E_i$ and we have what we claimed. 

Now we shall see that the definition does not depend on the decomposition of $E$. Let $E=\bigsqcup E_i=\bigsqcup F_j$, then $E=\bigsqcup_{i,j}E_i\cap F_j$. Therefore,
$$\sum_i\mu(\sigma(E_i))=\sum_i\mu(\sigma(\sqcup_j E_i\cap F_j))=\sum_i\mu(\sqcup_j\sigma( E_i\cap F_j))=\sum_{i,j}\mu(\sigma(E_i\cap F_j))$$
Doing analogously for $\{F_j\}$ instead of $\{E_i\}$ we conclude that
$$\sum_i\mu(\sigma(E_i))=\sum_j\mu(\sigma(F_j)) $$
We therefore have that the measure $\mu\odot\sigma$ is well defined.
\end{remark}

Now, we present the notion of conformal measure introduced by Sarig \cite{Sarig1999}.
\begin{definition}[Conformal measure - Sarig]
A measure $\mu$ in $X$ is called $(\beta F, \lambda)$-conformal in the sense of Sarig if there exists $\lambda >0$ such that
\begin{equation*}
\dfrac{d\mu\odot\sigma}{d\mu}(x)= \lambda e^{-\beta F(x)}\quad \mu\; a.e \; x\in U.
\end{equation*}
\end{definition}


%%%%%% TEOREMA PRINCIPAL 1
\section{Conformal measures on generalized Renault-Deaconu groupoids}

The next result extend some equivalences from the classical setting to the context of the generalized Renault-Deaconu Groupoids.



\begin{theorem}\label{theorem.princial.1} Let $X$ be locally compact, Hausdorff and second countable space, $U \subseteq X$ open and $\sigma: U \to X$ a local homeomorphism. Let $\mu$ be a borel measure that is finite on compacts. For a given continuous potential $F:U\to \mathbb{R}$, the following are equivalent.

\begin{itemize}
    \item[$(i)$] $\mu$ is $e^{\beta F}$-conformal measure in the sense of Denker-Urba\'nski;
    \item[$(ii)$] $\mu$ is a eigenmeasure associated with the Ruelle Transformation $L_{-\beta F}$, that is
    \begin{equation*}
        \int_{X} \sum_{\sigma(y)=x} f(y) e^{-\beta F(y)} d\mu(x) = \int_{U} f(x) d\mu(x),
    \end{equation*}
    for all $f \in C_c(U)$;
    \item[$(iii)$] $\mu$ is  $e^{-\beta c_F}$-quasi-invariant on $\mathcal{G}(X,\sigma)$, i.e
    \begin{equation}\label{eq:quasi-invariant-measure}
\int_{X} \sum_{r(\gamma)=x} e^{\beta c_F(\gamma)} f(\gamma)  d\mu(x) = \int_{X}\sum_{s(\gamma)=x}f(\gamma)  d\mu(x).
    \end{equation}
    for all $f \in C_c(\mathcal{G}(X,\sigma))$;
    \item[$(iv)$] $\mu$ is $(-\beta F, 1)$-conformal in the sense of Sarig.
\end{itemize}

\end{theorem}

\begin{proof} 
\vv
$(iii)\implies (ii)$ is analogous to Proposition 4.2 in \cite{Renault2003}, but we repeat the proof. For any $f\in C_c(U)$, consider:
$$\int_X \sum_{\sigma(y)=x}f(y)e^{-\beta F(y)}d\mu(x)=\int_X\sum_{s(\gamma)=x}(fe^{-\beta F}\circ r)(\gamma)\mathbbm{1}_{S}(\gamma)d\mu(x). $$
where $S$ is the set $\{(x,1,\sigma(x)): x\in U\}$. Now, we use that $\mu$ is quasi-invariant to conclude that
$$\int_X\sum_{s(\gamma)=x}(fe^{-\beta F}\circ r)(\gamma)\mathbbm{1}_{S}(\gamma)d\mu(x)=\int_X\sum_{r(\gamma)=x}(fe^{-\beta F})\circ r(\gamma)\mathbbm{1}_{S}(\gamma)e^{\beta c_F(\gamma)}d\mu(x)=\int_U f d\mu. $$
Proving the implication we were interested.
\vv 
For $(ii) \implies (i)$ let $V$ be an open subset of $U$ such that $\sigma\restriction_V$ is injective, and let $W = \sigma(V)$. Also denote by $\tau : W \to V$ the inverse of the restriction of $\sigma$ to $V$. We then have two measures of interest on $V$, namely
\begin{equation*}
\tau^*(\mu\restriction_W)\quad and \quad e^{\beta F}\mu\restriction_V.    
\end{equation*}
We claim that the above measures on $V$ are equal. By the uniqueness part of the Riesz-Markov theorem, it is enough to prove that
\begin{equation}\label{eq:urbanski_integrated}
    \int_V gd\tau^*(\mu\restriction_W)=\int_V ge^{\beta F}d\mu\restriction_V,
\end{equation}
for every $g$ in $C_c(V)$. Given such a $g$, we consider its extension to the whole of $U$ by setting it to be zero on $U \setminus V$ . The extended function is then in $C_c(U)$. Defining $f = ge^{\beta F}$ , we then have that

\begin{align*}
    \int_V g e^{\beta F} d\mu\restriction_V&=\int_U f d\mu \stackrel{(\ref{theorem.princial.1}.ii)}{=}\int_X \sum_{\sigma(y)=x}f(y)e^{-\beta F(y)}d\mu(y)\\
    &=\int_W f(\tau(x))e^{-\beta F(\tau(x))}d\mu(x)=\int_W g(\tau(x))d\mu(x)=\int_V g d\tau^*(\mu).
\end{align*}
This proves \eqref{eq:urbanski_integrated}, and hence also that $\tau^*(\mu\restriction_W)=e^{\beta F}\mu\restriction_V$. It follows that, for every measurable set $E\subseteq V$,
\begin{equation*}
    \mu(\sigma(E))=\mu(\tau^{-1}(E))=\tau^*(\mu\restriction_W)(E)=\int_E e^{\beta F}d\mu.
\end{equation*}
Now, suppose $E\subseteq U$ is a special set, since $\sigma$ is a local homeomorphism and $X$ is second countable, there exists a countable collection of open sets $\{V_i\}_{i\in \mathbb{N}}$ such that $\sigma\restriction_{V_i}$ is injective and $E\subseteq \bigcup_{i\in \mathbb{N}}V_i$. Then we have a countable collection of measurable sets $\{E_i\}_{i\in\mathbb{N}}$, pairwise disjoint, such that $E_i\subseteq V_i$ and $E=\sqcup_{i\in \mathbb{N}}E_i$. We conclude, using that $E$ is special, that
\begin{equation*}
    \mu(\sigma(E))=\sum_{i\in \mathbb{N}}\mu(\sigma(E_i))=\sum_{i\in \mathbb{N}}\int_{E_i}e^{\beta F} d\mu=\int_E e^{\beta F}.
\end{equation*}

$(i)\implies (iii)$. We consider the open bisections defined in the preliminaries $W(n,m,C,B)$. W.l.o.g we can consider $\sigma^n(C)=\sigma^m(B)$, since if not we could take open sets $C'\subseteq C$ and $B'\subseteq B$ such that $\sigma^n(C')=\sigma^n(C)\cap \sigma^m(B)=\sigma^m(B')$. Also, we can suppose that $\sigma^n$ is injective when restricted $C$, similarly for $\sigma^m$ and $B$. In this setting, we can define the map $\sigma^{n-m}_{CB}:=\sigma^{-m}_B\circ\sigma^n_C$ and similarly $\sigma^{m-n}_{BC}:=\sigma^{-n}_C\circ \sigma^{m}_B$.
\[
\begin{tikzcd}
 & \sigma^n(C)=\sigma^m(B)  \\
C \arrow{ur}{\sigma^n_C} \arrow[rr,dashed,"\sigma^{n-m}_{CB}"] && B \arrow[ul,"\sigma^m_B"'] \arrow[ll,dashed,"\sigma^{m-n}_{BC}", bend left]
\end{tikzcd}
\]
Let $f \in C_c(\mathcal{G}(X,\sigma)$ s.t. $supp(f)\subseteq W(n,m,C,B)$. Let us see how the equation \eqref{eq:quasi-invariant-measure} on item $(iii)$ simplifies in this case. Observe first the left hand side. If $x \notin C$, clearly there is no $\gamma\in W(n,m,C,B)$ such that $r(\gamma)=x$, so the integration can be done in $C$. Now, for $x\in C$, consider $\gamma_1,\gamma_2\in W(n,m,C,B)$ such that $r(\gamma_1)=r(\gamma_2)=x$. Since the range map is injective in such set we have $\gamma_1=\gamma_2$ and we conclude the summation on the left hand side of equation \eqref{eq:quasi-invariant-measure} have at most one non-zero term for each $x\in C$. Denoting this term by $\gamma_x$, we see this term is written as $\gamma_x=(x,n-m,\sigma_{CB}^{n-m}(x))$. So, the left hand side of equation \eqref{eq:quasi-invariant-measure} is
\begin{equation}\label{eq:theorem3,LHS}
\int_C e^{\beta c_F(\gamma_x)} f(\gamma_x)  d\mu(x)=\int_C e^{\beta c_F((x,n-m,\sigma_{CB}^{n-m}(x)))} f(x,n-m,\sigma_{CB}^{n-m}(x))  d\mu(x).    
\end{equation}
Calculation on the right hand side of equation \eqref{eq:quasi-invariant-measure} is done in a similar fashion, we have:
\begin{equation}\label{eq:theorem3,RHS}
    \int_B f(\sigma_{BC}^{m-n}(y),n-m,y)d\mu(y).
\end{equation}
Now let $g:C\to \mathbb{C}$ defined by $g(x)=f(x,n-m,\sigma_{CB}^{n-m}(x)).$ Observe that $g(\sigma^{m-n}_{BC}(y))=f(\sigma^{m-n}_{BC}(y),n-m,y)$, which is the function in the equation \eqref{eq:theorem3,RHS}. We rewrite the quasi-invariant condition with the considerations from above
\begin{equation}\label{eq:QIC}
    \int_C e^{\beta c_F(x,n-m,\sigma^{n-m}(x))}g(x)d\mu(x)=\int_B g(\sigma^{m-n}_{BC}(y))d\mu(y),
\end{equation}
for $g\in C_c(C)$. We just need to prove that item $(i)$ implies equation \eqref{eq:QIC}. First, observe that item $(i)$ implies for all $C$ open subset of $U$, $\sigma\restriction_C$ injective that
\begin{equation}\label{eq:urbanski_the_not_so_good}
\int_C g(x) e^{\beta F(x)} d\mu(x) = \int_{\sigma(C)} g(\sigma^{-1}(x)) d\mu(x),    
\end{equation}
for all $g\in C_c(C)$. We observe as well that equation \eqref{eq:urbanski_the_not_so_good} is equation \eqref{eq:QIC} when $m=0$ and $n=1$. To prove \eqref{eq:QIC} we proceed by induction on $n+m$. If $n+m=0$ we have $C=B$ , $\sigma_{BC}^{n-m}=Id$ and $c_F(x,0,x)=0$, so equation (\ref{eq:QIC}) is clearly satisfied. Take $n\neq 0$.%% Figure CBsigma_g.png %%

\[
\begin{tikzcd}[row sep=5em]
 & \mathbb{C} &  \\[-2em]
C\arrow[ur,"g"]\arrow[rr,"\sigma"]\arrow[d,"\sigma^{n-m}_{CB}"']& & \sigma(C)=C'\arrow[ul,"g'"']\arrow[d,"\sigma^{n-1}"]\\
B\arrow[urr,"\sigma^{m-(n-1)}_{BC'}",dashed]\arrow[rr,"\sigma^m_B"']& & \sigma^n(C)=\sigma^m(B)
\end{tikzcd}
\]
\vv \noindent
Let $g':C'=\sigma(C)\to  \mathbb{C}$ defined by $g'(x)=g(\sigma^{-1}(x))$, $g'\in C_c(C')$. By induction hypothesis,
$$\int_B g'(\sigma_{BC'}^{m-(n-1)}(y))d\mu(y)=\int_{C'}e^{\beta c_F(x,n-1-m,\sigma^{(n-1)-m}(x))}g'(x)d\mu(x).$$
On the other hand, using as reference the figure above
$$\int_B g'(\sigma_{BC'}^{m-(n-1)}(y))d\mu(y)=\int_B g(\sigma^{-1}\sigma_{BC'}^{m-(n-1)}(y))d\mu(y)=\int_B g(\sigma_{BC}^{m-n}(y))d\mu(y)$$
Which is the right hand side of equation \eqref{eq:QIC}. Then,
\begin{equation}\label{eq:g_2}
\int_{C'}e^{\beta c_F(x,n-1-m,\sigma^{(n-1)-m}(x))}g'(x)d\mu=\int_{\sigma(C)}\underbrace{e^{\beta c_F(x,n-1-m,\sigma^{(n-1)-m}(x))}g(\sigma^{-1}(x))}_{g_2(x)}d\mu.    
\end{equation}
The equation \eqref{eq:urbanski_the_not_so_good}, using a change of variables, can be seen as well as
$$\int_C g_2(\sigma(x))e^{\beta F(x)} d\mu(x)=\int_{\sigma(C)}g_2(x)d\mu\quad \forall g_2\in C_c(\sigma(C)). $$
Applying it to \eqref{eq:g_2}, we obtain
\begin{align*}
\int_{C'}e^{\beta c_F(x,n-1-m,\sigma^{(n-1)-m}(x))}g'(x)d\mu(x)&=\int_C g_2(\sigma(x))e^{\beta F(x)} d\mu(x)\\
&= \int_C e^{\beta c_F(\sigma(x),n-1-m,\sigma^{(n-1)-m}(\sigma(x)))}g(x)e^{\beta F(x)}d\mu(x).
\end{align*}
It is left to verify that
$$c_F(\sigma(x),n-1-m,\sigma^{n-1-m}(\sigma(x)))+F(x)=c_F(x,n-m,\sigma^{n-m}(x)),$$
because that is the left hand side of equation \eqref{eq:QIC}.
It is true by the cocycle property of $c_F$ and the fact that $F(x)=c_F(x,1,\sigma(x))$ along with the observation that $$(x,1,\sigma(x))(\sigma(x),n-1-m,\sigma^{n-m}(x))=(x,n-m,\sigma(x)).$$
The implication $(i)\implies (iii)$ is proved for $f$ supported on the open bisection $W(n,m,C,B)$, therefore proved for every $f\in C_c(\mathcal{G}(X,\sigma)).$
\vv \noindent
Now, we prove $(i) \iff (iv)$. Suppose that $\dfrac{d\mu\odot\sigma}{d\mu}=e^{\beta F}\quad \mu\; a.e\; x\in U$. Take $E\subseteq U$ such that $\sigma|_E$ is injective. Then,
$$\mu(\sigma(E))=\mu\odot\sigma(E)=\int_U \mathbbm{1}_{E}\,d\mu\odot\sigma=\int_U \mathbbm{1}_E e^{\beta F(x)}d\mu(x)=\int_E e^{\beta F(x)} d\mu(x)$$
and we have proved item $(i)$.
\vv \noindent
Now the converse. Let $E\subseteq$ U and $\{E_i\}_{i\in \mathbb{N}}$ be its decomposition. Hence,
\begin{align*}
\mu\odot\sigma(E)= \sum_{i\in \mathbb{N}}\mu(\sigma(E_i))=\sum_{i\in \mathbb{N}}  \int_X \mathbbm{1}_{E_i} e^{\beta F(x)}\mu(x)=\int_E e^{\beta F(x)} d\mu(x). \nonumber
\end{align*}
Since this is true for every measurable set $E\subseteq U$, we have
$$\dfrac{d\mu\odot\sigma}{d\mu}(x)=e^{\beta F(x)}\quad \mu\; a.e \; x\in U.$$
This concludes the theorem.\qed
\end{proof}

\begin{remark}
The above theorem is of particular interest, since it is known that if a measure $\mu$  is $e^{-\beta c_F}$-quasi-invariant on $\mathcal{G}(X,\sigma)$, then the state defined by 
\begin{equation}
\varphi_\mu(f)=\int_X f(x,0,x)d\mu(x),\quad f\in C_c(\mathcal{G}(X,\sigma))
\end{equation}

is a $KMS_\beta$ state of the full groupoid $C^*$-algebra $C^*(\mathcal{G}(X,\sigma))$ for the one parameter group of automorphisms $(\eta_t)$ defined as

$$\eta_t(f)(\gamma)=e^{itc_F(\gamma)}f(\gamma) , \quad f\in C_c(\mathcal{G}(X,\sigma)), \gamma\in \mathcal{G}(X,\sigma).$$

More than that, if the subgroupoid $c_F^{-1}(0)$ is \textit{principal}, then every $KMS_\beta$ state of $C^*(\mathcal{G}(X,\sigma))$ for $\eta$ is of the form $\varphi_\mu$, for a measure $\mu$ that is $e^{-\beta c_F}$-quasi-invariant (see Theorem 3.3.12 of \cite{Renault2009} for these assertions).  By principal we mean that the \textit{isotropy} subgroupoid  ${Iso(\mathcal{G}):=\{\gamma\in \mathcal{G}: r(\gamma)=s(\gamma) \}= \mathcal{G}^{(0)}}$. Observe that the units of $c_F^{-1}(0)$ are $X$.

As an example, suppose $F>0$. Then for $\gamma=(x,n-m,x)\in Iso(c_F^{-1}(0))$, we have

$$\sum_{i=0}^{n-1}F(\sigma^i(x))=\sum_{i=0}^{m-1}F(\sigma^i(x))$$

which can only happen if $n=m$, thus $\gamma=(x,0,x)\in X$ and we conclude that $c_F^{-1}(0)$ is principal.




\end{remark}


\begin{figure}[H]
\begin{center}
\begin{tikzpicture}[scale=1.5]
\draw   (0,0) -- (7,0);
\node[circle, draw=black, fill=white, inner sep=1pt,minimum size=5pt] (1) at (0,0) {1};
\node[circle, draw=black, fill=white, inner sep=1pt,minimum size=5pt] (2) at (1,0) {2};
\node[circle, draw=black, fill=white, inner sep=1pt,minimum size=5pt] (3) at (2,0) {3};
\node[circle, draw=black, fill=white, inner sep=1pt,minimum size=5pt] (4) at (3,0) {4};
\node[circle, draw=black, fill=white, inner sep=1pt,minimum size=5pt] (5) at (4,0) {5};
\node[circle, draw=black, fill=white, inner sep=1pt,minimum size=5pt] (6) at (5,0) {6};
\node[circle, draw=black, fill=white, inner sep=1pt,minimum size=5pt] (7) at (6,0) {7};
\draw[->, >=stealth] (2)  to (1);
\draw[->, >=stealth] (3)  to (2);
\draw[->, >=stealth] (4)  to (3);
\draw[->, >=stealth] (5)  to (4);
\draw[->, >=stealth] (6)  to (5);
\draw[->, >=stealth] (7)  to (6);
\node [minimum size=10pt,inner sep=0pt,outer sep=0pt] {} edge [in=200,out=100,loop, >=stealth] (0);
\draw[->, >=stealth] (1)  to [out=90,in=90, looseness=1] (2);
\draw[->, >=stealth] (1)  to [out=90,in=90, looseness=1] (3);
\draw[->, >=stealth] (1)  to [out=90,in=90, looseness=1] (4);
\draw[->, >=stealth] (1)  to [out=90,in=90, looseness=1] (5);
\draw[->, >=stealth] (1)  to [out=90,in=90, looseness=1] (6);
\draw[->, >=stealth] (1)  to [out=90,in=90, looseness=1] (7);
\end{tikzpicture}
\end{center}
\caption{The renewal shift}\label{fig:renewal}
\end{figure}


\begin{definition} Given an irreducible transition matrix $A$ on the alphabet $\mathbb{N}$, define the sets
\begin{equation*}
    X_A := \text{spec}\,\mathcal{D}_A \quad \text{and} \quad \widetilde{X}_A := \text{spec}\,\widetilde{\mathcal{D}}_A
\end{equation*}
where the second one is only considered in the case that $\mathcal{O}_A$ is non-unital.
\end{definition}


Note that $X_A$ is locally compact (weak$^*$ topology) and $\widetilde{X}_A$ is always compact. Also, both $\widetilde{\mathcal{D}}_A$ and $\mathcal{D}_A$ are $C^*$-subalgebras of the diagonal operators of $\mathfrak{B}(l^2(\Sigma_A))$. 

At this point we have the necessary structure to present the inclusion of $\Sigma_A$ in $X_A$, as defined below.


\begin{definition} Given $A$ an irreducible matrix and its corresponding Markov shift space $\Sigma_A$, we define the inclusion $i_1: \Sigma_A \xhookrightarrow{} X_A: \Sigma_A \ni \omega \mapsto \varphi_{\omega}\restriction_{\mathcal{D}_A} \in X_A,$ where $\varphi_{\omega}$ is the evaluation map
\begin{equation}\label{eq:varphi_omega_definition}
    \varphi_\omega(R)= (R\delta_\omega,\delta_\omega), \quad R \in \mathfrak{B}(l^2(\Sigma_A)).
\end{equation}
will be denoted by $i_1$ and the context will clarify if the codomain is $X_A$ or $\widetilde{X}_A$.
\end{definition}


\vv


From now we will omit the notations of restriction to $\widetilde{\mathcal{D}}_A$ and $\mathcal{D}_A$ on $\varphi_\omega$.

\begin{remark}\label{rem:i_1_inj_cont} The inclusion $i_1$ is an injective continuous function in both cases.
\end{remark}



Two of the most important results about the inclusions $i_1$ are the facts that $i_1(\Sigma_A)$ is dense in $X_A$ (respect. $\widetilde{X}_A$) and that the Borel sets of $\Sigma_A$ are included as Borel sets of $X_A$ (respect. $\widetilde{X}_A$). In order to prove the density mentioned, we need the following lemma, which is a direct consequence of the Gelfand representation theorem for commutative $C^*$-algebras.

\begin{lemma}\label{lemma:dense_character_general} Given a commutative $C^*$ algebra $B$, let $Y \subseteq \text{spec}\,B$ such that for any $a \in B$ it follows that
\begin{equation}\label{eq:Y_separates_spectrum_version}
    \varphi(a) = 0 \quad \forall \varphi \in Y \implies a=0,
\end{equation}
i.e., $Y$ separates points in $B$. Then $Y$ is dense in $\text{spec}\,B$ (weak$^*$ topology).
\end{lemma}



\begin{corollary}\label{prop:i_1_Sigma_A_dense} $i_1(\Sigma_A)$ is dense in $X_A$. Also, $i_1(\Sigma_A)$ is dense in $\widetilde{X}_A$ when $\mathcal{O}_A$ is not unital.
\end{corollary}



\vv


\vv

The proposition \ref{prop:D_A_isomorphic_e_g} gives us a easier way to see $X_A$ (repect. $\widetilde{X}_A$). Given $\varphi \in X_A$ or $\widetilde{X}_A$, we can determine its image completely simply by taking its values on the generators $(e_g)_{g \in \mathbb{F}}$. Since $e_g$ is idempotent for any $g$, it follows that $\varphi(e_g) \in \{0,1\}$ and $(\varphi(e_g))_{g \in \mathbb{F}} \in \{0,1\}^{\mathbb{F}}$. Here, $\{0,1\}^{\mathbb{F}}$ is endowed with the product topology of the discrete topology in $\{0,1\}$. Then, the values of the characters on the aforementioned generators define the inclusions  (same definition for $\widetilde{X}_A$)
\begin{align}\label{eq:unit_D_A_01}
    X_A &\to \{0,1\}^{\mathbb{F}},\\
    \varphi &\mapsto (\varphi(e_g))_{g \in \mathbb{F}}, \nonumber
\end{align}
which will be identified with the same notation, namely $i_2$. The map $i_2$ is a topological embedding. 

Now we can see the characters in $X_A$ and $\widetilde{X}_A$ as configurations in the Cayley graph generated by $\mathbb{F}$, where the words $g$ are the vertices and the oriented edges multiply the word in the source vertex by a letter $a$, leading to the range vertex. Of course, the inverse way of the edge represents a multiplication by the inverse of the correspondent letter $a$.
\begin{figure}[H]
\begin{center}
		\begin{tikzpicture}[scale=1.5,decoration={markings, mark=at position 0.5 with {\arrow{>}}}]
		\node[circle, draw=black, fill=black, inner sep=1pt,minimum size=1pt] (0) at (0,0) {};
		\node[circle, draw=black, fill=black, inner sep=1pt,minimum size=1pt] (1) at (3,0) {};
    	\draw[postaction={decorate}, >=stealth] (0)  to (1);
   	    \node[above] at (0,0) {$g$};
   	    \node[above] at (1.5,0) {$a$};
        \node[above] at (3,0) {$ga$};
		\end{tikzpicture}
	\end{center}
\end{figure}
 
The next corollary is straightforward.

\begin{corollary}\label{cor:i_2_i_1_Sigma_A_dense} $i_2 \circ i_1(\Sigma_A)$ is dense in $i_2(X_A)$. Moreover, if $\mathcal{O}_A$ is not unital, then $i_2 \circ i_1(\Sigma_A)$ is dense in $i_2(\widetilde{X}_A)$.
\end{corollary}




From now we will describe $X_A$ (respect. $\widetilde{X}_A$) by its copy $i_2(X_A)$ (respect. $i_2(\widetilde{X}_A)$) contained in $\{0,1\}^\mathbb{F}$. Formally, and in terms of configurations in $\{0,1\}^\mathbb{F}$, we call that the word $g \in \mathbb{F}$ \textit{is filled in} $\xi \in \{0,1\}^\mathbb{F}$ when $\xi_g = 1$. The configuration $\xi$ is called \textit{convex} if for any two $a,b \in \mathbb{F}$ filled in $\xi$, the whole shortest path between $a$ and $b$ is also filled in $\xi$. Note that a configuration $\xi$ is convex and it $e$ is filled in $\xi$ if and only if for all $g \in \mathbb{F}$ which is filled it implies that subwords are also filled.

We recall the set
\begin{equation} \label{eq:Omega_A_tau}
    \Omega_A^{\tau} = \left\{ \begin{array}{l}
         \xi \in \{0,1\}^\mathbb{F}: \xi_e = 1, \text{ } \xi \text{ convex}, \\
         \text{if $\xi_\omega=1$, then there exists at most one $y \in \mathbb{N}$ s.t. $\xi_{\omega y}=1$}, \\
         \text{if $\xi_\omega= \xi_{\omega y}=1$, $y \in \mathbb{N}$, then for all $x \in \mathbb{N}$ } (\xi_{\omega x^{-1}}=1 \iff A(x,y)=1)
    \end{array}\right\}
\end{equation}
as in \cite{Exel}, which we will use to study $i_2(X_A)$ (respect. $i_2(\widetilde{X}_A)$). In fact $i_2(X_A)\subseteq \Omega^\tau_A$.
\begin{figure}[H]
\begin{center}
		\begin{tikzpicture}[scale=1.5,decoration={markings, mark=at position 0.5 with {\arrow{>}}}]
		\node[circle, draw=black, fill=black, inner sep=1pt,minimum size=5pt] (0) at (0,0) {0};
		\node[circle, draw=black, fill=black, inner sep=1pt,minimum size=5pt] (1) at (0,1) {1};
		\node[circle, draw=black, fill=black, inner sep=1pt,minimum size=5pt] (2) at (1,1) {2};
    	\draw[postaction={decorate}, >=stealth] (0)  to (1);
    	\draw[postaction={decorate}, >=stealth] (1)  to (2);
   		\node[left] at (0,0.5) {$x$};
   	    \node[above] at (0.5,1) {$y$};
   	    \node[above] at (0,1.1) {$w$};
        \node[above] at (1,1.1) {$wy$};
        \node[above] at (0.5,1.5) {$A(x,y)=1$};
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
       \node[circle, draw=black, fill=white, inner sep=1pt,minimum size=10pt] (3) at (3,0) {};
		\node[circle, draw=black, fill=black, inner sep=1pt,minimum size=5pt] (4) at (3,1) {4};
		\node[circle, draw=black, fill=black, inner sep=1pt,minimum size=5pt] (5) at (4,1) {5};
    	\draw[postaction={decorate},>=stealth] (3)  to (4);
    	\draw[postaction={decorate}, >=stealth] (4)  to (5);
   		\node[left] at (3,0.5) {$x$};
   	    \node[above] at (3.5,1) {$y$};
   	    \node[above] at (3,1.1) {$w$};
        \node[above] at (4,1.1) {$wy$};
        \node[above] at (3.5,1.5) {$A(x,y)=0$};
		\end{tikzpicture}
	\end{center}
	\caption{ Representation of the last condition of $\Omega_A^\tau$. The black dots represents that the configuration $\xi$ is filled. }
\end{figure}
	


\begin{remark} It is important to notice the difference between how the configurations of $\{0,1\}^\mathbb{F}$ are presented here and in \cite{Exel}. Here, for a given configuration $\xi$ and a word $g \in \mathbb{F}$ we will use $\xi_g = 1$ instead of $g \in \xi$ as used in \cite{Exel}, which is motivated by the Markov shift notation for sequences in $\Sigma_A$.
\end{remark}

Now, we introduce the definition of stem and root of a configuration in $i_2(X_A)$ (respect. $i_2(\widetilde{X}_A)$) as in \cite{Exel}. By a \textit{positive word} in $\mathbb{F}$ we mean any finite or infinite sequence $\omega = \omega_0 \omega_1 \cdots$ which $\omega_j \in \mathbb{F}_+$ for every $j$, and $\omega$ is said to be admissible if $A(\omega_j,\omega_{j+1}) = 1$ for all $j$.

Given an either finite or infinite positive word $\omega = \omega_0 \omega_1 \cdots$, define the set
\begin{equation*}
    \llbracket \omega \rrbracket := \{e,\omega_0,\omega_0 \omega_1,\omega_0\omega_1\omega_2,\cdots\}
\end{equation*}
of the subwords of $\omega$. For any configuration $\xi \in \Omega_A^\tau$ there exists a unique positive admissible word $\omega$ or $\omega=e$ (see proposition 5.4 of \cite{Exel}) called \textit{stem} which $\{g \in \mathbb{F}: \xi_g = 1\} \cap \mathbb{F}_+ = \llbracket \omega \rrbracket$. The stem of $\xi$ will be denoted by $\kappa(\xi)$. Roughly speaking, the stem of a configuration correponds to the `positive main river' of a configuration, that is, the longest path of positive finite words which are filled in the configuration. We say that a configuration $\xi \in \Omega_A^\tau$ is a \textit{bounded element} if its stem has finite length (defintion 5.5 of \cite{Exel}). If $\xi$ is not bounded we call it \textit{unbounded}. Also, by the proposition 7.3 of \cite{Exel} $i_2(X_A)$ (respect. $i_2(\widetilde{X}_A)$) is the closure of the unbounded elements of $\Omega_A^{\tau}$. 

 We recall the set $R_\xi(g):= \{j \in \mathbb{N}:\xi_{g j^{-1}}=1\}, \, g \in \mathbb{F} \text{ s.t. } \xi_g = 1$, named \textit{root} of $g$ relative to $\xi$ (see definition 5.6 of \cite{Exel}). In the section 5 of \cite{Exel} it is proved that there exists a bijection between the unbounded elements of $\Omega_A^\tau$ and the infinite positive admissible words, which is precisely the set $i_2\circ i_1(\Sigma_A)$. Moreover, accordingly to the corollary 7.7 of \cite{Exel}, $\xi$ is a bounded element in $i_2(X_A)$ if and only if $R_\xi(\kappa(\xi))$ is an accumulation point of the set $\{c_j\}_{j \in \mathbb{N}}$ in the product topology $\{0,1\}^\mathbb{N}$, where $c_j = \{k \in \mathbb{N}:A(k,j)=1\}$ is the $j$-th column of $A$. 



The following result is somehow contained in the original paper from Exel and Laca, we include here for sake of completeness.




\begin{proposition}\label{prop:characterization_of_elements_of_Y_A} Let $\xi \in \Omega_A^\tau$. Then $\xi \in Y_A$ if and only if it satisfies simultaneously the two following items:
\begin{itemize}
    \item[$(a)$] $\kappa(\xi) = e$ or $\kappa(\xi)$ ends in an infinite emmiter letter; 
    \item[$(b)$] If $\kappa(\xi)\neq e$, $R_\xi(\kappa(\xi))$ is a limit point of the sequence $(\mathfrak{c}(i))_{A(\kappa(\xi)_{|\kappa(\xi)|-1},i)=1}$ of columns of $A$, with these columns seen as elements of $\{0,1\}^\mathbb{N}$. If $\kappa(\xi)= e$, $R_\xi(\kappa(\xi))$ is a limit point of the sequence $(\mathfrak{c}(i))_{i \in \mathbb{N}}$.
\end{itemize}
\end{proposition} 

\begin{proof} Let $\xi \in Y_A$. By the corollary \ref{cor:i_2_i_1_Sigma_A_dense}, there exists a sequence $\{\xi^n\}_{\mathbb{N}}$ in $\Sigma_A$ converging to $\xi$. Then, we have that
\begin{equation*}
    (\xi^n)_{\kappa(\xi)} \to 1 \quad \text{and} \quad (\xi^n)_{\kappa(\xi) a} \to 0,
\end{equation*}
where the second convergence holds for every $a \in \mathbb{N}$. Since the convergence is inherited from the product topology of $\{0,1\}^\mathbb{F}$, for each $a \in \mathbb{N}$, the sequence  $\{(\xi^n)_{\kappa(\xi) a}\}_\mathbb{N}$ is eventually constant. Hence, we necessarily have that $\kappa(\xi) = e$ or it ends in an infinite emmiter, otherwise it would exist a symbol $b \in \mathbb{N}$ such that $(\xi^n)_{\kappa(\xi) b} = 1$ for infinitely many values of $n$, which gives a contradiction because this fact would imply that $\xi_{\kappa(\xi)b}=1$. On the other hand, suppose that $\kappa(\xi) \neq e$, we have
\begin{equation}
    R_{\xi^n}(\kappa(\xi)) = \{j \in \mathbb{N}: A(j,a_n) = 1\} = c(a_n)
\end{equation}
where $a_n \in \mathbb{N}$ is the unique symbol due to $(R3)$ s.t. $\xi^n_{\kappa(\xi)a_n} = 1$ and $c(a_n)$ is the $a_n$-th column of $A$ when we see $R_{\xi^n}(\kappa(\xi))$ as an element of $\{0,1\}^{\mathbb{N}}$. Since $\xi^n \to \xi$ we have that
\begin{equation*}
    R_{\xi^n}(\kappa(\xi))_j = \xi^n_{\kappa(\xi) j^{-1}} \to \xi_{\kappa(\xi) j^{-1}} = R_\xi(\kappa(\xi)_j),
\end{equation*}
for every $j \in \mathbb{N}$, that is, $c(a_n) \to R_\xi(\kappa(\xi)$, and therefore $R_\xi(\kappa(\xi))$ is an accumulation point of the set $\{c(i): A(\kappa(\xi)_{|\kappa(\xi)|-1},i)\}$ of the columns of $A$, and therefore it is a limit point since this set is countable. The proof is similar for $\kappa(\xi) = e$.

Conversely, suppose that $\xi \in \Omega_A^\tau$ satisfies $(a)$ and $(b)$. We construct a sequence $\{\xi^n\}_{\mathbb{N}}$ of elements $\Sigma_A$ converging to $Y_A$, by setting
\begin{equation*}
    \xi^n_{\kappa(\xi)} = \xi^n_{\kappa(\xi)i(n)} = 1,
\end{equation*}
where $\{i(n)\}_{\mathbb{N}}$ is an enumeration of distinct elements of an infinite subset of $\{k \in \mathbb{N}:A(\kappa(\xi)_{|\kappa(\xi)|},k)=1\}$ if $|\kappa(\xi)| > 0$, and an infinit subset of $\mathbb{N}$ otherwise, in both cases satisfying $\mathfrak{c}(i(n)) \to R_\xi(\kappa(\xi)$. In addition, for each $n \in \mathbb{N}$ we choose $\omega_n \in [\kappa(\xi)i(n)]$ and set $\xi^n_{u}:= 1$ for every $u \in \llbracket \omega_n \rrbracket$. This choice determines uniquely each $\xi^n$. It is straighforward that $\xi^n_{\kappa(\xi)} = 1$ for every $n \in \mathbb{N}$,
\begin{equation*}
    \xi^n_{\kappa(\xi)a} \to 0 \quad \text{and} \quad R_{\xi^n}(\kappa(\xi)) = \mathfrak{c}(i(n)) \to R_\xi(\kappa(\xi)).
\end{equation*}
We constructed a sequence in $\Sigma_A$ that converges to an element $\xi \in \Omega_A^\tau$, by density, we necessarily have that $\xi \in Y_A$. \qed
\end{proof}














Using these facts we can prove the following:
\begin{proposition}
$i_2\circ i_1(\Sigma_A)$ is a measurable set in the Borel $\sigma$-algebra of $i_2(X_A)$.
\end{proposition}
\begin{proof} Using the fact that $i_2$ is a homeomorphism,
\begin{equation*}
  i_2(X_A\setminus i_1(\Sigma_A)) = i_2(X_A)\setminus i_2\circ i_1(\Sigma_A) =\{\xi\in i_2(X_A):|\kappa(\xi)|<\infty\}=\bigcup_{\alpha\in \mathcal{L}}\{\xi\in i_2(X_A):\kappa(\xi)=\alpha\},  
\end{equation*}
where $\mathcal{L}$ is the set of all admissible finite words, which is a countable set. Note that
\begin{align*}
    H(\alpha):&=\{\xi\in i_2(X_A):\kappa(\xi) =\alpha\} = \{\xi\in i_2(X_A):\xi_\alpha=1 \text{ and } \xi_{\alpha s}=0,\text{ }\forall s\in \mathbb{N}\} \\
    &= \{\xi\in i_2(X_A):\xi_\alpha=1\} \cap \{\xi\in i_2(X_A): \xi_{\alpha s}=0,\text{ }\forall s\in \mathbb{N} \}.
\end{align*}
Since $H(\alpha)$ is an intersection of two closed sets, this means that $H(\alpha)$ is closed in $i_2(X_A)$.  As $i_2(X_A)\setminus i_2\circ i_1(\Sigma_A)$ is an countable union of those sets, we conclude $i_2(X_A)\setminus i_2\circ i_1(\Sigma_A)$ is a $F_\sigma$, hence $i_2\circ i_1(\Sigma_A)$ is a $G_\delta$, a borelian. \qed

\end{proof}

\begin{proposition}For every Borel set $B \subseteq \Sigma_A$, $i_1(B)$ is a Borel set in $X_A$.
\end{proposition} 

\begin{proof} It is equivalent to prove that $i_2 \circ i_1(B)$ is a Borel set. Also, it is sufficient to prove the result for the cylinders in $\Sigma_A$ because they do form an countable basis of the topology. Given a cylinder set $[\alpha]\subseteq \Sigma_A$, we have that $i_2 \circ i_1([\alpha]) = \{\xi \in i_2(X_A): \kappa(\xi) \text{ is infinite and $\xi_\alpha=1$}\}$.

Denoting by $\pi_g$ the projection of a word $g$ in the Cayley tree it follows that
\begin{equation*}
    i_2 \circ i_1([\alpha]) = \left(\bigcap_{\nu \in \llbracket\alpha\rrbracket}\pi_{\nu}^{-1}(\{1\})\right)\cap i_2\circ i_1(\Sigma_A)
\end{equation*}
is a Borel set in $i_2(X_A)$. \qed
\end{proof}
\vv
Our next step is to consider a specific Renewal shift and to construct conformal measures which are not detected in $\Sigma_A$ but they are found when we consider $X_A$ instead.
%Trivially the same result above is also valid for $\widetilde{X}_A$ in the place of $X_A$. It is important to notice that both $X_A$ and $\widetilde{X}_A$ have an analogue structure to the Markov shift space. Let $X = X_A$ if $\mathcal{O}_A$ is unital and $X= \widetilde{X}_A$ otherwise. Also, consider the sets
%\begin{equation*}
%    U_s := \{\xi \in i_2(X): \xi_s=1\}, \quad \forall s\in \mathbb{N}.
%\end{equation*}
%and
%\begin{equation*}
%    U_0 := \{\xi \in i_2(X): \xi_s=0, \quad \forall s \in \mathbb{N}\}.
%\end{equation*}
%We notice that,
%\begin{equation*}
%    U_s = \pi_s^{-1}(\{1\}) \cap i_2(X), \quad s \in \mathbb{N},
%\end{equation*}
%and therefore it is a open compact subset of $i_2(X)$ on the subspace topology for every $s \in \mathbb{N}$. For $U_0$ we have that 
%\begin{equation}\label{eq:U_0}
%    U_0 = \bigcap_{s \in \mathbb{N}}\pi_s^{-1}(\{0\}) \cap i_2(X),
%\end{equation}
%and then we have that $U_0$ is a compact subset of $i_2(X)$. We emphasize that the family of compact sets $\{U_s\}_{\mathbb{N}_0}$ is mutually disjoint since it is contained in $\Omega^\tau_A$ and therefore for any $g \in \mathbb{F}$ with $\xi_g=1$, there exists at most one $y \in \mathbb{N}$ s.t. $\xi_{g y}=1$. In particular we can take $g=e$ and therefore there is at most one letter $s \in \mathbb{N}$ s.t. $\xi_s=1$. This proves that $U_i \cap U_j = \emptyset$ for $i,j \in \mathbb{N}$ if $i\neq j$. On other hand we have trivially that $U_0 \cap U_j = \emptyset$ for all $i \in \mathbb{N}$. Summarizing, $\{U_s\}_\mathbb{N_0}$ is a family of compact mutually disjoints subsets of $i_2(X)$, where $U_s$ is open for every $s\in \mathbb{N}$. 
%The point is that the sets $U_s$' in $i_2(X_A)$ work as the cylinder sets $[s]$' in $\Sigma_A$. Note that $i_2(i_1([s])) \subset U_s$ for all $s \in \mathbb{N}$. Moreover, $U_s = i_2(i_1([s])) \sqcup [s]^*$, where $[s]^*:= \overline{i_2(i_1([s]))}\setminus i_2(i_1([s]))$ is the set of all configurations of finite stem starting with $s$ such that the last letter, we say $j$, corresponds to a non finitely supported line in the matrix $A$, i.e., $A(j,k) = 1$ for infinite $k$'s. The results achieved so far in this section are general and valid for $X_A$ compact, i.e., $i_2(X_A) = i_2(X_A)$. We recall that if $\mathcal{O}_A$ is unital, then $i_2(X_A)$ is compact. Also, it is sufficient that $A$ has at least one line of $1$'s in order to $\mathcal{O}_A$ be unital. 
%Now let us identify the elements of $X_A$ beyond $\Sigma_A$. Since $i_2 \circ i_1 (\Sigma_A)$ is dense in $i_2(X_A)$, the elements of $(i_2 \circ i_1 (\Sigma_A))^c$ are the bounded elements of $\Omega_A^\tau$ which are limit points of the elements in $i_2 \circ i_1 (\Sigma_A)$. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%\subsection{Convergence of measures living on $Y_A$}\\







\section{Conformal measures which vanish on $\Sigma_A$. The Renewal Shift}\label{sec:conformal_renewal}

Consider the Markov shift given by the graph of the Figure \ref{fig:renewal}, and $\phi:\Sigma_{A}\to \{c\}$ is a constant potential, where $c\in \mathbb{R}$. In this case the algebra $\mathcal{O}_A$ is unital since the row of the letter $1$ has only $1$'s. Indeed, consider for any $X,Y \subseteq \mathbb{N}$ finite sets and $j \in \mathbb{N}$ the function
\[
A(X,Y,j):= \prod_{x \in X}A(x,j) \prod_{y \in Y}(1 - A(y,j)),\]
and notice that for our Renewal shift it follows that $ A(\emptyset,\{1\},j) = 0$
for every $j \in \mathbb{N}$. Hence, by the proposition 8.5 of \cite{Exel}, it follows that $\mathcal{O}_A$ is unital.

Now we describe the bounded elements on $X_A$ for our Renewal shift. They are precisely the configurations associated to positive finite admissible words on $\mathbb{F}_+$ which ends with the letter `$1$' or a unique configuration $\xi^0$ with no positive stem. Indeed, the unique limit point of $\{c_k\}_{k \in \mathbb{N}}$ of the topology $\{0,1\}^\mathbb{N}$ is the element 
\begin{equation*}
    c = \begin{pmatrix} 1 \\ 0 \\0 \\ 0 \\\vdots
    \end{pmatrix}
\end{equation*}
and by the corollary 7.7 of \cite{Exel} we have that $R_\xi(\omega) = c$ in $\{0,1\}^\mathbb{N}$ for any possible stem $\omega$ of $\xi$. In the case $\omega \neq e$, this implies $\omega$ necessarily ends with $1$. On the other hand, if $\omega = e$ this will imply that there is only one configuration $\xi^0$ s.t. its stem is $e$. 

\begin{figure}[H]
    \centering
\scalebox{0.6}{
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,738); %set diagram left start at 0, and has height of 738

%Straight Lines [id:da7718154569127509] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (667.94,575.21) -- (652.41,510.49) ;
\draw [shift={(651.48,506.6)}, rotate = 436.51] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da26407415052363525] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (659.71,540.91) -- (643.25,472.29) ;



%Straight Lines [id:da8543996419941418] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (629.03,574.18) -- (637.36,509.26) ;
\draw [shift={(637.87,505.29)}, rotate = 457.31] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da014601186212476858] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (633.45,539.74) -- (642.28,470.85) ;



%Straight Lines [id:da0908505280803571] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (609.39,580.5) -- (585.89,522.72) ;
\draw [shift={(584.39,519.02)}, rotate = 427.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da4857187007512451] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (596.89,549.76) -- (571.88,488.28) ;



%Straight Lines [id:da6002236678480226] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (572.95,587.68) -- (569.89,524.53) ;
\draw [shift={(569.69,520.53)}, rotate = 447.22] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9748786227496797] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (571.32,554.11) -- (568.06,486.96) ;



%Straight Lines [id:da2915408631432912] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (571.42,680.98) -- (539.55,623.81) ;
\draw [shift={(537.61,620.32)}, rotate = 420.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da4886430857270365] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (554.51,650.65) -- (520.7,589.98) ;



%Straight Lines [id:da20109791673993938] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (522.84,691.78) -- (520.68,626.36) ;
\draw [shift={(520.55,622.36)}, rotate = 448.11] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9277173321303496] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (521.69,657.07) -- (519.4,587.65) ;



%Straight Lines [id:da9498395429610376] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (464.45,695.5) -- (463.23,630.06) ;
\draw [shift={(463.16,626.06)}, rotate = 448.94] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8782223524135282] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (463.8,660.78) -- (462.52,591.34) ;



%Straight Lines [id:da19440218309241253] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (416.5,682.17) -- (445.38,623.43) ;
\draw [shift={(447.14,619.84)}, rotate = 476.18] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da3467649189685993] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (431.82,651) -- (462.46,588.67) ;



%Straight Lines [id:da8658408539050857] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (521,591) -- (532.68,447.65) ;
\draw [shift={(533,443.67)}, rotate = 454.66] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da5166413385711035] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (527,517.33) -- (539,370) ;



%Straight Lines [id:da697321732090175] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (462,592) -- (447.73,447.98) ;
\draw [shift={(447.33,444)}, rotate = 444.34] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9869737400891978] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (454.67,518) -- (440,370) ;



%Straight Lines [id:da792639962333257] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (421.57,590.05) -- (416.13,527.91) ;
\draw [shift={(415.78,523.92)}, rotate = 445] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da3922142082449338] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (418.68,556.99) -- (412.89,490.86) ;



%Straight Lines [id:da5615327680986446] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (384.63,586.17) -- (400.3,524.92) ;
\draw [shift={(401.29,521.04)}, rotate = 464.35] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7619979236588721] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (392.96,553.61) -- (409.62,488.48) ;



%Straight Lines [id:da4451003686577464] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (356.14,576.61) -- (345.99,510.82) ;
\draw [shift={(345.38,506.87)}, rotate = 441.23] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da19180942485279662] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (350.76,541.74) -- (340,472) ;



%Straight Lines [id:da504715443679943] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (317.45,572.37) -- (331.09,508.36) ;
\draw [shift={(331.92,504.44)}, rotate = 462.03] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da18400330994336755] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (324.68,538.41) -- (339.15,470.48) ;



%Straight Lines [id:da16454973399334372] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (762.42,640.98) -- (730.55,583.81) ;
\draw [shift={(728.61,580.32)}, rotate = 420.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da37198373095580983] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (745.51,610.65) -- (711.7,549.98) ;



%Straight Lines [id:da310294461836804] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (713.84,651.78) -- (711.68,586.36) ;
\draw [shift={(711.55,582.36)}, rotate = 448.11] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da004210293601572657] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (712.69,617.07) -- (710.4,547.65) ;



%Straight Lines [id:da2680525125232769] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (274.45,653.5) -- (273.23,588.06) ;
\draw [shift={(273.16,584.06)}, rotate = 448.94] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8767516280381358] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (273.8,618.78) -- (272.52,549.34) ;



%Straight Lines [id:da2352926661357997] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (226.5,640.17) -- (255.38,581.43) ;
\draw [shift={(257.14,577.84)}, rotate = 476.18] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da19838623716694448] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (241.82,609) -- (272.46,546.67) ;



%Straight Lines [id:da9916377345642537] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (711.85,551.28) -- (652.2,401.29) ;
\draw [shift={(650.72,397.57)}, rotate = 428.31] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9132750516529802] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (681.28,474.43) -- (620.15,320.72) ;



%Straight Lines [id:da39534285709806305] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (569.79,489.02) -- (550.89,412.22) ;
\draw [shift={(549.93,408.34)}, rotate = 436.17] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da41961900928636653] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (559.86,448.68) -- (540,368) ;



%Straight Lines [id:da3410794235000656] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (412,490) -- (429.12,413.9) ;
\draw [shift={(430,410)}, rotate = 462.68] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8039570069063529] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (421,450) -- (439,370) ;



%Straight Lines [id:da5767317716189746] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (272,552) -- (329.25,401.07) ;
\draw [shift={(330.67,397.33)}, rotate = 470.77] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8199572271803517] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (301.33,474.67) -- (360,320) ;



%Straight Lines [id:da7805187991239197] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (640.65,470.91) -- (627.01,374.32) ;
\draw [shift={(626.45,370.36)}, rotate = 441.96] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da2679954746740738] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (633.55,420.64) -- (619.35,320.09) ;



%Straight Lines [id:da9139126818505943] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (340,471) -- (352.81,374.3) ;
\draw [shift={(353.33,370.33)}, rotate = 457.54] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da24622748847110998] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (346.67,420.67) -- (360,320) ;



%Straight Lines [id:da00020353845492770972] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (823.42,494.98) -- (791.55,437.81) ;
\draw [shift={(789.61,434.32)}, rotate = 420.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8854051200725124] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (806.51,464.65) -- (772.7,403.98) ;



%Straight Lines [id:da5290711488042574] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (774.84,505.78) -- (772.68,440.36) ;
\draw [shift={(772.55,436.36)}, rotate = 448.11] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da3533755812800199] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (773.69,471.07) -- (771.4,401.65) ;



%Straight Lines [id:da5147141282028127] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (943.64,391.62) -- (884.9,362.73) ;
\draw [shift={(881.31,360.97)}, rotate = 386.19] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da4352866638214645] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (912.48,376.29) -- (850.15,345.64) ;



%Straight Lines [id:da1225012928759932] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (900.68,439.61) -- (870.59,381.49) ;
\draw [shift={(868.75,377.94)}, rotate = 422.63] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da13334487652391913] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (884.71,408.78) -- (852.78,347.1) ;



%Straight Lines [id:da41572740420678267] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (621.76,323.65) -- (593.9,269.01) ;
\draw [shift={(592.08,265.45)}, rotate = 422.98] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7109429202502728] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (606.92,294.55) -- (577.24,236.35) ;



%Straight Lines [id:da09375180001795558] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (538.51,370.62) -- (561.61,283.66) ;
\draw [shift={(562.63,279.79)}, rotate = 464.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9409019980218534] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (550.57,325.2) -- (574.7,234.38) ;



%Straight Lines [id:da4129711446371902] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (439.21,370.99) -- (418.01,283.55) ;
\draw [shift={(417.07,279.66)}, rotate = 436.37] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da3472393386597188] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (428.14,325.33) -- (406,234) ;



%Straight Lines [id:da8729127927565754] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (359,322) -- (388.42,268.18) ;
\draw [shift={(390.33,264.67)}, rotate = 478.66] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da5234510641456187] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (374.67,293.33) -- (406,236) ;



%Straight Lines [id:da04295272493106861] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (941.34,218.07) -- (876.68,196.57) ;
\draw [shift={(872.89,195.31)}, rotate = 378.39] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da21349661887751203] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (907.11,206.69) -- (838.66,183.93) ;



%Straight Lines [id:da5576098015948623] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (899.77,272.27) -- (857.24,219.04) ;
\draw [shift={(854.74,215.91)}, rotate = 411.37] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8862710885186176] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (877.26,244.09) -- (832.23,187.73) ;



%Straight Lines [id:da3978270582356822] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (915.62,106.57) -- (849.35,90.74) ;
\draw [shift={(845.46,89.81)}, rotate = 373.43] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da03588911702849873] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (880.54,98.19) -- (810.38,81.43) ;



%Straight Lines [id:da9607655052834148] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (905.66,27.44) -- (845.94,61.68) ;
\draw [shift={(842.47,63.67)}, rotate = 330.16999999999996] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da37213858965076896] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (874.07,45.55) -- (810.87,81.78) ;



%Straight Lines [id:da48992770223503235] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (772.23,405.03) -- (765.03,340.3) ;
\draw [shift={(764.59,336.32)}, rotate = 443.66] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da591237258146921] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (768.41,370.68) -- (760.77,301.97) ;



%Straight Lines [id:da7185828253329849] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (855,345) -- (795.94,316.73) ;
\draw [shift={(792.33,315)}, rotate = 385.58000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da3251883969631266] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (823.67,330) -- (761,300) ;



%Straight Lines [id:da036905535004298384] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (762,300) -- (685.12,220.17) ;
\draw [shift={(682.35,217.29)}, rotate = 406.08000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7063392112123159] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (722.17,258.64) -- (642.52,175.93) ;



%Straight Lines [id:da6737793258206501] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (836.29,184.29) -- (771.94,164.22) ;
\draw [shift={(768.12,163.03)}, rotate = 377.33000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da6494293474776269] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (802.2,173.66) -- (734.03,152.39) ;



%Straight Lines [id:da2854032814293719] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (814.5,79) -- (764.99,124.74) ;
\draw [shift={(762.05,127.46)}, rotate = 317.27] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9310167568523808] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (788.27,103.23) -- (735.82,151.68) ;



%Straight Lines [id:da6650152521863433] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (738,153) -- (678.38,164.28) ;
\draw [shift={(674.45,165.03)}, rotate = 349.28] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7656751178280152] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (706.23,159.01) -- (642.68,171.04) ;



%Straight Lines [id:da3679511196013956] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (210.45,507.5) -- (209.23,442.06) ;
\draw [shift={(209.16,438.06)}, rotate = 448.94] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da3691009699932548] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (209.8,472.78) -- (208.52,403.34) ;



%Straight Lines [id:da7787183222922092] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (162.5,494.17) -- (191.38,435.43) ;
\draw [shift={(193.14,431.84)}, rotate = 476.18] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da36818001532447386] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (177.82,463) -- (208.46,400.67) ;



%Straight Lines [id:da8251304723632418] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (93.36,443.61) -- (114.87,381.8) ;
\draw [shift={(116.19,378.02)}, rotate = 469.19] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7462171026152358] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (104.78,410.82) -- (127.6,345.22) ;



%Straight Lines [id:da581832795245929] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (40.49,406.83) -- (94.51,369.87) ;
\draw [shift={(97.81,367.62)}, rotate = 505.63] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9353945480138346] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (69.15,387.22) -- (126.48,348.01) ;



%Straight Lines [id:da06701559271606028] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (207.5,409) -- (215.04,344.31) ;
\draw [shift={(215.5,340.33)}, rotate = 456.65] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da19917325639886196] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (211.5,374.67) -- (219.5,306) ;



%Straight Lines [id:da04531871858336167] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (125.46,346.84) -- (184.54,318.67) ;
\draw [shift={(188.15,316.95)}, rotate = 514.51] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da040034339354099835] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (156.81,331.89) -- (219.5,302) ;



%Straight Lines [id:da6530762845601967] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (219.5,302) -- (298.1,218.25) ;
\draw [shift={(300.83,215.33)}, rotate = 493.18] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da4932807483457349] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (260.17,258.67) -- (341.5,172) ;



%Straight Lines [id:da4667403648219859] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (93.96,270.86) -- (128.01,211.84) ;
\draw [shift={(130.01,208.38)}, rotate = 479.98] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da11576099924727479] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (111.99,239.62) -- (148.04,177.14) ;



%Straight Lines [id:da1557079719348149] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (45.35,210.12) -- (110.4,189.82) ;
\draw [shift={(114.22,188.63)}, rotate = 522.6600000000001] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da2888825768954728] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (79.78,199.37) -- (148.65,177.88) ;



%Straight Lines [id:da16002832594573912] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (69.27,105.13) -- (135.68,89.85) ;
\draw [shift={(139.58,88.96)}, rotate = 527.04] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da38675913457391875] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (104.42,97.04) -- (174.73,80.87) ;



%Straight Lines [id:da811126986989821] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (81.74,24.94) -- (140,60.28) ;
\draw [shift={(143.42,62.35)}, rotate = 211.24] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da20958359416805306] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (112.58,43.65) -- (174.26,81.06) ;



%Straight Lines [id:da9892613941262087] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (142.27,179.13) -- (208.68,163.85) ;
\draw [shift={(212.58,162.96)}, rotate = 527.04] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da1965062811921443] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (177.42,171.04) -- (247.73,154.87) ;



%Straight Lines [id:da8684947094990361] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (171.5,79) -- (217.36,125.49) ;
\draw [shift={(220.17,128.33)}, rotate = 225.39] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9515437154893183] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (195.83,103.67) -- (244.5,153) ;



%Straight Lines [id:da42844247384670475] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (244.34,155.67) -- (304.38,166.02) ;
\draw [shift={(308.32,166.7)}, rotate = 189.78] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da26369996177777955] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (276.33,161.18) -- (340.31,172.22) ;



%Straight Lines [id:da5157843117574503] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (643.64,174.09) -- (588.75,160.5) ;
\draw [shift={(584.87,159.54)}, rotate = 373.9] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da014237540465873666] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (614.25,166.81) -- (555.48,152.27) ;



%Straight Lines [id:da27748001915013076] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (573.95,236.19) -- (559.4,183.93) ;
\draw [shift={(558.33,180.08)}, rotate = 434.45] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9197855483600481] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (566.14,208.13) -- (550.52,152.03) ;



%Straight Lines [id:da9968276074230185] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (408.12,231.67) -- (419.57,183.14) ;
\draw [shift={(420.49,179.25)}, rotate = 463.27] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9665295464171277] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (414.3,205.46) -- (426.67,153.04) ;



%Straight Lines [id:da08999801209712532] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (340.5,173) -- (393.92,157.91) ;
\draw [shift={(397.77,156.82)}, rotate = 524.22] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da387316266663543] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (369.14,164.91) -- (426.41,148.73) ;



%Straight Lines [id:da000006065165543134299] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (552.22,149.93) -- (514.42,115.79) ;
\draw [shift={(511.45,113.1)}, rotate = 402.09000000000003] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da748591489313535] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (531.84,131.52) -- (491.07,94.69) ;



%Straight Lines [id:da3519598645730617] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (426.79,148.62) -- (464.94,114.86) ;
\draw [shift={(467.93,112.21)}, rotate = 498.48] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8708424435604669] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (447.36,130.42) -- (488.5,94) ;



%Straight Lines [id:da16951385086370085] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (490.67,82.67) -- (490.25,61.67) ;
\draw [shift={(490.17,57.67)}, rotate = 448.85] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da36976550533541164] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (490.42,70.17) -- (489.92,45.17) ;



%Shape: Circle [id:dp04917157739085254] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (490.33,50.53) .. controls (485.18,50.52) and (481.01,46.33) .. (481.03,41.17) .. controls (481.04,36.02) and (485.23,31.85) .. (490.38,31.86) .. controls (495.54,31.88) and (499.71,36.07) .. (499.69,41.22) .. controls (499.68,46.38) and (495.49,50.54) .. (490.33,50.53) -- cycle ;
%Shape: Circle [id:dp2952427104131581] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ] (490.62,101.33) .. controls (485.46,101.32) and (481.3,97.13) .. (481.31,91.98) .. controls (481.32,86.82) and (485.51,82.65) .. (490.67,82.67) .. controls (495.82,82.68) and (499.99,86.87) .. (499.98,92.02) .. controls (499.96,97.18) and (495.77,101.35) .. (490.62,101.33) -- cycle ;
%Shape: Circle [id:dp8318376815705786] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (421.97,153.72) .. controls (418.21,150.2) and (418.01,144.29) .. (421.53,140.53) .. controls (425.05,136.76) and (430.96,136.57) .. (434.72,140.09) .. controls (438.49,143.61) and (438.69,149.51) .. (435.16,153.28) .. controls (431.64,157.04) and (425.74,157.24) .. (421.97,153.72) -- cycle ;
%Shape: Circle [id:dp06952241330068132] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (334.45,179.23) .. controls (330.69,175.7) and (330.49,169.8) .. (334.01,166.03) .. controls (337.53,162.27) and (343.44,162.07) .. (347.2,165.59) .. controls (350.97,169.11) and (351.16,175.02) .. (347.64,178.79) .. controls (344.12,182.55) and (338.22,182.75) .. (334.45,179.23) -- cycle ;
%Shape: Circle [id:dp8513408904163751] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (400.27,241.21) .. controls (396.5,237.69) and (396.31,231.79) .. (399.83,228.02) .. controls (403.35,224.26) and (409.26,224.06) .. (413.02,227.58) .. controls (416.78,231.1) and (416.98,237.01) .. (413.46,240.77) .. controls (409.94,244.54) and (404.03,244.74) .. (400.27,241.21) -- cycle ;
%Shape: Circle [id:dp6849351464838338] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ] (557.61,155.43) .. controls (553.88,158.98) and (547.97,158.84) .. (544.42,155.11) .. controls (540.86,151.38) and (541.01,145.47) .. (544.74,141.91) .. controls (548.47,138.36) and (554.38,138.5) .. (557.93,142.23) .. controls (561.49,145.97) and (561.35,151.87) .. (557.61,155.43) -- cycle ;
%Shape: Circle [id:dp7218484159334866] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ] (580.84,242.81) .. controls (577.11,246.36) and (571.2,246.22) .. (567.64,242.49) .. controls (564.09,238.75) and (564.23,232.85) .. (567.96,229.29) .. controls (571.7,225.74) and (577.6,225.88) .. (581.16,229.61) .. controls (584.72,233.34) and (584.57,239.25) .. (580.84,242.81) -- cycle ;
%Shape: Circle [id:dp2642129916374887] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (647.62,179.09) .. controls (643.88,182.64) and (637.98,182.5) .. (634.42,178.77) .. controls (630.87,175.04) and (631.01,169.13) .. (634.74,165.57) .. controls (638.47,162.02) and (644.38,162.16) .. (647.94,165.89) .. controls (651.49,169.63) and (651.35,175.53) .. (647.62,179.09) -- cycle ;
%Shape: Circle [id:dp014386320314449419] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (360.42,329.95) .. controls (355.27,329.94) and (351.1,325.75) .. (351.11,320.59) .. controls (351.12,315.44) and (355.31,311.27) .. (360.47,311.28) .. controls (365.62,311.3) and (369.79,315.49) .. (369.78,320.64) .. controls (369.76,325.8) and (365.57,329.96) .. (360.42,329.95) -- cycle ;
%Shape: Circle [id:dp9452430731465025] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (272.29,560.54) .. controls (267.13,560.53) and (262.97,556.34) .. (262.98,551.18) .. controls (262.99,546.03) and (267.18,541.86) .. (272.34,541.87) .. controls (277.49,541.89) and (281.66,546.08) .. (281.65,551.23) .. controls (281.63,556.38) and (277.44,560.55) .. (272.29,560.54) -- cycle ;
%Shape: Circle [id:dp3135527844360546] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (340.29,480.7) .. controls (335.13,480.68) and (330.97,476.49) .. (330.98,471.34) .. controls (330.99,466.18) and (335.18,462.02) .. (340.34,462.03) .. controls (345.49,462.04) and (349.66,466.23) .. (349.65,471.39) .. controls (349.63,476.54) and (345.44,480.71) .. (340.29,480.7) -- cycle ;
%Shape: Circle [id:dp34753735981151346] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (440.09,379.89) .. controls (434.94,379.88) and (430.77,375.69) .. (430.78,370.53) .. controls (430.79,365.38) and (434.98,361.21) .. (440.14,361.22) .. controls (445.29,361.24) and (449.46,365.43) .. (449.45,370.58) .. controls (449.43,375.74) and (445.24,379.9) .. (440.09,379.89) -- cycle ;
%Shape: Circle [id:dp05218255876321343] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (410.96,501.48) .. controls (405.8,501.47) and (401.64,497.28) .. (401.65,492.12) .. controls (401.66,486.97) and (405.85,482.8) .. (411.01,482.81) .. controls (416.16,482.83) and (420.33,487.02) .. (420.32,492.17) .. controls (420.3,497.33) and (416.11,501.49) .. (410.96,501.48) -- cycle ;
%Shape: Circle [id:dp47555616451238714] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (461.96,600.64) .. controls (456.8,600.62) and (452.63,596.43) .. (452.65,591.28) .. controls (452.66,586.12) and (456.85,581.96) .. (462.01,581.97) .. controls (467.16,581.98) and (471.33,586.17) .. (471.31,591.33) .. controls (471.3,596.48) and (467.11,600.65) .. (461.96,600.64) -- cycle ;
%Shape: Circle [id:dp33341191367015255] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (539.42,379.95) .. controls (534.27,379.94) and (530.1,375.75) .. (530.11,370.59) .. controls (530.12,365.44) and (534.31,361.27) .. (539.47,361.28) .. controls (544.62,361.3) and (548.79,365.49) .. (548.78,370.64) .. controls (548.76,375.8) and (544.57,379.96) .. (539.42,379.95) -- cycle ;
%Shape: Circle [id:dp8218642078413914] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (520.29,600.54) .. controls (515.13,600.53) and (510.97,596.34) .. (510.98,591.18) .. controls (510.99,586.03) and (515.18,581.86) .. (520.34,581.87) .. controls (525.49,581.89) and (529.66,586.08) .. (529.65,591.23) .. controls (529.63,596.38) and (525.44,600.55) .. (520.29,600.54) -- cycle ;
%Shape: Circle [id:dp535582180760606] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (571.29,500.7) .. controls (566.13,500.68) and (561.97,496.49) .. (561.98,491.34) .. controls (561.99,486.18) and (566.18,482.02) .. (571.34,482.03) .. controls (576.49,482.04) and (580.66,486.23) .. (580.65,491.39) .. controls (580.63,496.54) and (576.44,500.71) .. (571.29,500.7) -- cycle ;
%Shape: Circle [id:dp7905851530391403] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ] (620.09,329.89) .. controls (614.94,329.88) and (610.77,325.69) .. (610.78,320.53) .. controls (610.79,315.38) and (614.98,311.21) .. (620.14,311.22) .. controls (625.29,311.24) and (629.46,315.43) .. (629.45,320.58) .. controls (629.43,325.74) and (625.24,329.9) .. (620.09,329.89) -- cycle ;
%Shape: Circle [id:dp5671066288064701] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (640.96,480.48) .. controls (635.8,480.47) and (631.64,476.28) .. (631.65,471.12) .. controls (631.66,465.97) and (635.85,461.8) .. (641.01,461.81) .. controls (646.16,461.83) and (650.33,466.02) .. (650.32,471.17) .. controls (650.3,476.33) and (646.11,480.49) .. (640.96,480.48) -- cycle ;
%Shape: Circle [id:dp4543680354831854] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ] (709.96,558.64) .. controls (704.8,558.62) and (700.63,554.43) .. (700.65,549.28) .. controls (700.66,544.12) and (704.85,539.96) .. (710.01,539.97) .. controls (715.16,539.98) and (719.33,544.17) .. (719.31,549.33) .. controls (719.3,554.48) and (715.11,558.65) .. (709.96,558.64) -- cycle ;
%Shape: Circle [id:dp4853740073057362] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (237,153.14) .. controls (238.69,148.27) and (244.01,145.69) .. (248.88,147.38) .. controls (253.75,149.07) and (256.33,154.39) .. (254.63,159.26) .. controls (252.94,164.13) and (247.62,166.71) .. (242.75,165.01) .. controls (237.89,163.32) and (235.31,158) .. (237,153.14) -- cycle ;
%Shape: Circle [id:dp2852054657012817] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (165.37,77.97) .. controls (167.06,73.1) and (172.38,70.52) .. (177.25,72.22) .. controls (182.12,73.91) and (184.7,79.23) .. (183,84.1) .. controls (181.31,88.97) and (175.99,91.54) .. (171.12,89.85) .. controls (166.26,88.16) and (163.68,82.84) .. (165.37,77.97) -- cycle ;
%Shape: Circle [id:dp7605994987546616] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (136.51,174.72) .. controls (138.2,169.85) and (143.52,167.28) .. (148.39,168.97) .. controls (153.26,170.66) and (155.84,175.98) .. (154.14,180.85) .. controls (152.45,185.72) and (147.13,188.29) .. (142.26,186.6) .. controls (137.4,184.91) and (134.82,179.59) .. (136.51,174.72) -- cycle ;
%Shape: Circle [id:dp11807998800668473] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (807.66,91.19) .. controls (802.81,89.45) and (800.28,84.11) .. (802.01,79.26) .. controls (803.75,74.4) and (809.09,71.88) .. (813.94,73.61) .. controls (818.79,75.34) and (821.32,80.69) .. (819.59,85.54) .. controls (817.86,90.39) and (812.51,92.92) .. (807.66,91.19) -- cycle ;
%Shape: Circle [id:dp05762758158264858] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (731.87,162.16) .. controls (727.02,160.43) and (724.49,155.08) .. (726.22,150.23) .. controls (727.96,145.38) and (733.3,142.85) .. (738.15,144.58) .. controls (743.01,146.32) and (745.54,151.66) .. (743.8,156.51) .. controls (742.07,161.37) and (736.73,163.89) .. (731.87,162.16) -- cycle ;
%Shape: Circle [id:dp5968876606975246] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (828.37,191.86) .. controls (823.51,190.13) and (820.98,184.79) .. (822.72,179.93) .. controls (824.45,175.08) and (829.79,172.55) .. (834.65,174.28) .. controls (839.5,176.02) and (842.03,181.36) .. (840.3,186.21) .. controls (838.56,191.07) and (833.22,193.6) .. (828.37,191.86) -- cycle ;
%Shape: Circle [id:dp08649508999546796] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (214.12,309.33) .. controls (210.03,306.19) and (209.26,300.34) .. (212.39,296.25) .. controls (215.53,292.16) and (221.39,291.38) .. (225.48,294.52) .. controls (229.57,297.66) and (230.34,303.52) .. (227.2,307.61) .. controls (224.07,311.7) and (218.21,312.47) .. (214.12,309.33) -- cycle ;
%Shape: Circle [id:dp12722863581469235] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (120.24,353.69) .. controls (116.15,350.55) and (115.38,344.69) .. (118.51,340.6) .. controls (121.65,336.51) and (127.51,335.74) .. (131.6,338.88) .. controls (135.69,342.02) and (136.46,347.87) .. (133.33,351.96) .. controls (130.19,356.05) and (124.33,356.83) .. (120.24,353.69) -- cycle ;
%Shape: Circle [id:dp5185596388669738] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (203.01,411.51) .. controls (198.92,408.37) and (198.14,402.52) .. (201.28,398.43) .. controls (204.42,394.34) and (210.28,393.56) .. (214.37,396.7) .. controls (218.46,399.84) and (219.23,405.7) .. (216.09,409.79) .. controls (212.95,413.88) and (207.1,414.65) .. (203.01,411.51) -- cycle ;
%Shape: Circle [id:dp26677095916384275] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (768.66,306.25) .. controls (765.48,310.3) and (759.61,311.01) .. (755.56,307.82) .. controls (751.5,304.64) and (750.8,298.77) .. (753.98,294.72) .. controls (757.17,290.66) and (763.04,289.96) .. (767.09,293.14) .. controls (771.14,296.33) and (771.85,302.2) .. (768.66,306.25) -- cycle ;
%Shape: Circle [id:dp3576312844817602] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (779.92,409.64) .. controls (776.73,413.69) and (770.86,414.4) .. (766.81,411.21) .. controls (762.76,408.03) and (762.05,402.16) .. (765.24,398.11) .. controls (768.42,394.05) and (774.29,393.35) .. (778.34,396.54) .. controls (782.4,399.72) and (783.1,405.59) .. (779.92,409.64) -- cycle ;
%Shape: Circle [id:dp537935916504316] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (862.7,350.56) .. controls (859.52,354.61) and (853.65,355.31) .. (849.6,352.13) .. controls (845.54,348.94) and (844.84,343.08) .. (848.03,339.02) .. controls (851.21,334.97) and (857.08,334.27) .. (861.13,337.45) .. controls (865.18,340.64) and (865.89,346.5) .. (862.7,350.56) -- cycle ;

% Text Node
\draw (515,36) node [scale=1.7280000000000002]  {$e$};
% Text Node
\draw (475,62) node [scale=1,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (449,105) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (537,103) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (538,192) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (384,138) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (441,194) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (301,139) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (230,99) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (149,35) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (304,250) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (203,188) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (128,111) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (99,170) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (169,301) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (87,350) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (168,442) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (131,400) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (600,142) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (144,228) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (238,356) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (679,244) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (685,139) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$4$};
% Text Node
\draw (777,190) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (759,103) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$5$};
% Text Node
\draw (841,38) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$6$};
% Text Node
\draw (859,116) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (888,176) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (815,298) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (848,250) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (235,450) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$4$};
% Text Node
\draw (370,258) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (536,288) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (620,263) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (448,292) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (32,211) node [rotate=-343.07]  {$\cdots $};
% Text Node
\draw (85,281) node [rotate=-301.76]  {$\cdots $};
% Text Node
\draw (29,412) node [rotate=-324.87]  {$\cdots $};
% Text Node
\draw (88,454) node [rotate=-290.85]  {$\cdots $};
% Text Node
\draw (155,505) node [rotate=-296.57]  {$\cdots $};
% Text Node
\draw (208,519) node [rotate=-267.51]  {$\cdots $};
% Text Node
\draw (929,107) node [rotate=-8.75]  {$\cdots $};
% Text Node
\draw (56,106) node [rotate=-347.74]  {$\cdots $};
% Text Node
\draw (73,16) node [rotate=-36.03]  {$\cdots $};
% Text Node
\draw (915,19) node [rotate=-328.74]  {$\cdots $};
% Text Node
\draw (953,219) node [rotate=-17.74]  {$\cdots $};
% Text Node
\draw (908,280) node [rotate=-48.81]  {$\cdots $};
% Text Node
\draw (746,350) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (904.41,451.65) node [rotate=-241.87]  {$\cdots $};
% Text Node
\draw (953.29,398.21) node [rotate=-207.85]  {$\cdots $};
% Text Node
\draw (773.32,518.87) node [rotate=-268.5]  {$\cdots $};
% Text Node
\draw (826.67,506.28) node [rotate=-239.44]  {$\cdots $};
% Text Node
\draw (750,457) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (851,401) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (817,436) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (904,345) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (307,401) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (374,381) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (219,651) node [rotate=-296.57]  {$\cdots $};
% Text Node
\draw (272,665) node [rotate=-267.51]  {$\cdots $};
% Text Node
\draw (712.32,664.87) node [rotate=-268.5]  {$\cdots $};
% Text Node
\draw (765.67,652.28) node [rotate=-239.44]  {$\cdots $};
% Text Node
\draw (235,581) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (293,593) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (312.82,584.71) node [rotate=-282.42]  {$\cdots $};
% Text Node
\draw (356.4,588.83) node [rotate=-259.9]  {$\cdots $};
% Text Node
\draw (313,522) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (379.29,596.01) node [rotate=-288.26]  {$\cdots $};
% Text Node
\draw (419.59,601.3) node [rotate=-263.39]  {$\cdots $};
% Text Node
\draw (365,516) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (407,418) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (384,529) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (433,536) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (466,450) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$4$};
% Text Node
\draw (513,451) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (575,417) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (608,383) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (678,406) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (409,693) node [rotate=-296.57]  {$\cdots $};
% Text Node
\draw (462,707) node [rotate=-267.51]  {$\cdots $};
% Text Node
\draw (425,623) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (480,638) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$5$};
% Text Node
\draw (521.32,704.87) node [rotate=-268.5]  {$\cdots $};
% Text Node
\draw (574.67,692.28) node [rotate=-239.44]  {$\cdots $};
% Text Node
\draw (506,638) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (567,621) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (696,590) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (570.74,598.66) node [rotate=-271.13]  {$\cdots $};
% Text Node
\draw (610.82,591.84) node [rotate=-246.26]  {$\cdots $};
% Text Node
\draw (555,534) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (606,527) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (625.44,586.86) node [rotate=-277.7]  {$\cdots $};
% Text Node
\draw (669.2,587.38) node [rotate=-255.18]  {$\cdots $};
% Text Node
\draw (624,515) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (674,521) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (754,584) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$4$};
% Text Node
\draw (515,81) node [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$1^{-1}$};
% Text Node
\draw (567,124) node [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$1^{-1} 2^{-1}$};
% Text Node
\draw (621,231) node [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$1^{-1} 2^{-1} 1^{-1}$};
% Text Node
\draw (677,318) node [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$1^{-1} 2^{-1} 1^{-1} 2^{-1}$};
% Text Node
\draw (778,546) node [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$1^{-1} 2^{-1} 1^{-1} 2^{-1} 3^{-1}$};

\end{tikzpicture}

}
\label{figure.emptyconfigurationrenewal}
\caption{The empty stem configuration of the renewal shift}
\end{figure}


Consider the set $R = \{\omega \in \mathbb{F}_+: \xi^0_{\omega^{-1}}=1\}$. Since $R_{\xi^0}(e) = \{1\}$, the set $R$ is precisely all the finite admissible positive words which ends with `$1$'. From now on we identify $i_2(X_A)$ with $X_A$ and $i_2\circ i_1(\Sigma_A)$ with $\Sigma_A$. Define
\begin{equation*}
    Y_A:= X_A \setminus \Sigma_A.
\end{equation*}
As the main objective of this section we will construct conformal measures that vanishes in $\Sigma_A$.

\begin{tikzpicture}

\node[circle,fill=black,inner sep=0pt,minimum size=8pt,label=below:{$1$}]      (maintopic)                              {};
\node[circle,fill=black,minimum size=8pt, label=right:{$j_1$}]        (j1)       [above right= 1.5cm and 1cm of maintopic] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_2$}]        (j2)       [above right= 1cm and 1.1cm of maintopic] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_3$}]        (j3)       [above right= 0.5cm and 1.2cm of maintopic] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_4$}]        (j4)       [above right= 0cm and 1.3cm of maintopic] {};

\draw[->,shorten >=0.1cm](maintopic.north) edge[bend left=45] (j1.west);
\draw[->,shorten >=0.1cm](maintopic.north) edge[bend left=45] (j2.west);
\draw[->,shorten >=0.1cm](maintopic.north) edge[bend left=45] (j3.west);
\draw[->,shorten <=0.7cm,ultra thick](j3.east) -- ($(j3.west)+(0:2.2)$);
\draw[->,shorten >=0.1cm](maintopic.north) edge[bend left=45] (j4.west);


\node[circle,fill=black,inner sep=0pt,minimum size=8pt,label=below:{$1$}]      (maintopic2) [right= 3.5cm of maintopic]                              {};
\node[circle,fill=white,draw,minimum size=8pt, label=right:{$j_1$}]        (j12)       [above right= 1.5cm and 1cm of maintopic2] {};
\node[circle,fill=black,draw,minimum size=8pt,label=right:{$j_2$}]        (j22)       [above right= 1cm and 1.1cm of maintopic2] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_3$}]        (j32)       [above right= 0.5cm and 1.2cm of maintopic2] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_4$}]        (j42)       [above right= 0cm and 1.3cm of maintopic2] {};

\draw[->,shorten >=0.1cm](maintopic2.north) edge[bend left=45] (j12.west);
\draw[->,shorten >=0.1cm](maintopic2.north) edge[bend left=45] (j22.west);
\draw[->,shorten >=0.1cm](maintopic2.north) edge[bend left=45] (j32.west);
\draw[->,shorten <=0.7cm,ultra thick](j32.east) -- ($(j32.west)+(0:2.2)$);
\draw[->,shorten >=0.1cm](maintopic2.north) edge[bend left=45] (j42.west);



\node[circle,fill=black,inner sep=0pt,minimum size=8pt,label=below:{$1$}]      (maintopic3) [right= 3.5cm of maintopic2]                              {};
\node[circle,fill=white,draw,minimum size=8pt, label=right:{$j_1$}]        (j13)       [above right= 1.5cm and 1cm of maintopic3] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_2$}]        (j23)       [above right= 1cm and 1.1cm of maintopic3] {};
\node[circle,fill=black,draw,minimum size=8pt,label=right:{$j_3$}]        (j33)       [above right= 0.5cm and 1.2cm of maintopic3] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_4$}]        (j43)       [above right= 0cm and 1.3cm of maintopic3] {};

\draw[->,shorten >=0.1cm](maintopic3.north) edge[bend left=45] (j13.west);
\draw[->,shorten >=0.1cm](maintopic3.north) edge[bend left=45] (j23.west);
\draw[->,shorten >=0.1cm](maintopic3.north) edge[bend left=45] (j33.west);
\draw[->,shorten <=0.7cm,ultra thick](j33.east) -- ($(j33.west)+(0:2.2)$);


\draw[->,shorten >=0.1cm](maintopic3.north) edge[bend left=45] (j43.west);

%asfdasf

\node[circle,fill=black,inner sep=0pt,minimum size=8pt,label=below:{$1$}]      (maintopic4) [right= 3.5cm of maintopic3]                              {};
\node[circle,fill=white,draw,minimum size=8pt, label=right:{$j_1$}]        (j14)       [above right= 1.5cm and 1cm of maintopic4] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_2$}]        (j24)       [above right= 1cm and 1.1cm of maintopic4] {};
\node[circle,fill=white,draw,minimum size=8pt,label=right:{$j_3$}]        (j34)       [above right= 0.5cm and 1.2cm of maintopic4] {};
\node[circle,fill=black,draw,minimum size=8pt,label=right:{$j_4$}]        (j44)       [above right= 0cm and 1.3cm of maintopic4] {};
\node     (dots)       [right= 2.0cm of j34] {$\bullet\bullet\bullet$};

\draw[->,shorten >=0.1cm](maintopic4.north) edge[bend left=45] (j14.west);
\draw[->,shorten >=0.1cm](maintopic4.north) edge[bend left=45] (j24.west);
\draw[->,shorten >=0.1cm](maintopic4.north) edge[bend left=45] (j34.west);
\draw[->,shorten <=0.7cm,ultra thick](j34.east) -- ($(j34.west)+(0:2.2)$);
\draw[->,shorten >=0.1cm](maintopic4.north) edge[bend left=45] (j44.west);

\end{tikzpicture}
\begin{lemma} The correspondence $\omega \mapsto \omega \xi^0$ is a map between $R$ and $Y_A$, which the inverse map sends $\xi \in Y_A$ to the stem of $\xi$.
\end{lemma}

\begin{proof} Since $\xi^0_{\omega^{-1}}=1$ for each $\omega \in R$, it follows that the translation $\omega\xi^0$, given by $(\omega\xi^0)_g=\xi^0_{\omega^{-1} g}$, is such that $\omega\xi^0_e = 1$, therefore $\omega\xi^0 \in X_A$ (the remaining properties are invariant by translation). It is straightforward to notice that $\omega$ is the stem of $\omega\xi^0$ and it does not belong to $\Sigma_A$, hence $\omega\xi^0 \in Y_A$. It is easy to verify that the map of the statement is injective.

For its surjectivity let $\xi \in Y_A$. Since $\xi \notin \Sigma_A$, the stem of $\xi$, $\kappa(\xi)$, is finite. Hence, there is no positive word filled in $\kappa(\xi)^{-1}\xi$ and $\kappa(\xi)^{-1}\xi = \xi^0$ by the uniqueness of $\xi^0$. Since $\xi_e=1$ we have that $\xi^0_{\kappa(\xi)^{-1}}=1$, therefore $\kappa(\xi) \in R$. By the equality $\xi = \omega \xi^0$, the surjectivity is evident. \qed
\end{proof}

\begin{figure}[H]
    \centering

\scalebox{0.7}{
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,452); %set diagram left start at 0, and has height of 452

%Straight Lines [id:da5252689526926522] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (328.67,284) -- (329.16,254.11) ;
\draw [shift={(329.22,250.11)}, rotate = 450.94] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da3692805759804776] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (328.94,267.06) -- (329.5,233.17) ;



%Straight Lines [id:da20445205651384657] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (276.93,232.78) -- (306.83,232.62) ;
\draw [shift={(310.83,232.6)}, rotate = 539.7] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da41403409180500206] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (293.88,232.69) -- (327.77,232.51) ;



%Straight Lines [id:da04321669133195849] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (502.53,93.47) -- (479.35,118.86) ;
\draw [shift={(476.65,121.81)}, rotate = 312.4] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da08509111213559928] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (489.59,107.64) -- (463.71,135.98) ;



%Straight Lines [id:da524055118748703] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (519.84,143.71) -- (485.46,143.75) ;
\draw [shift={(481.46,143.75)}, rotate = 359.93] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da49913150846570353] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (500.65,143.73) -- (462.27,143.78) ;



%Straight Lines [id:da3156491628199509] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (520.7,204.71) -- (486.32,204.75) ;
\draw [shift={(482.32,204.76)}, rotate = 359.93] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9384302974893177] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (501.51,204.73) -- (463.14,204.78) ;



%Straight Lines [id:da7134174521222101] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (456.63,144.71) -- (416.04,158.82) ;
\draw [shift={(412.26,160.14)}, rotate = 340.83000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da13364260247616477] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (434.44,152.42) -- (390.08,167.85) ;



%Shape: Circle [id:dp5733068139768824] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (465.9,150.83) .. controls (461.76,155.08) and (454.95,155.17) .. (450.7,151.03) .. controls (446.45,146.88) and (446.36,140.08) .. (450.51,135.82) .. controls (454.65,131.57) and (461.46,131.49) .. (465.71,135.63) .. controls (469.96,139.78) and (470.05,146.58) .. (465.9,150.83) -- cycle ;
%Straight Lines [id:da8875205825663077] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (501.75,252.53) -- (477.99,227.68) ;
\draw [shift={(475.23,224.79)}, rotate = 406.28] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7562384830218132] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (488.49,238.66) -- (461.97,210.92) ;



%Straight Lines [id:da021747329082931754] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (455.25,205.2) -- (416.44,186.73) ;
\draw [shift={(412.83,185.01)}, rotate = 385.45] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da22050636052500105] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (434.04,195.1) -- (391.62,174.92) ;



%Straight Lines [id:da7221229131712807] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (382.19,172.12) -- (352.3,172.21) ;
\draw [shift={(348.3,172.22)}, rotate = 359.83000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da6809420059874696] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (365.24,172.17) -- (331.35,172.27) ;



%Shape: Circle [id:dp8719118734029521] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (457.54,216.07) .. controls (451.61,216.18) and (446.7,211.46) .. (446.59,205.53) .. controls (446.47,199.59) and (451.19,194.69) .. (457.13,194.57) .. controls (463.06,194.46) and (467.97,199.18) .. (468.08,205.11) .. controls (468.2,211.05) and (463.48,215.95) .. (457.54,216.07) -- cycle ;
%Shape: Circle [id:dp7330284649760606] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (387.64,182.19) .. controls (381.7,182.3) and (376.79,177.58) .. (376.68,171.65) .. controls (376.56,165.71) and (381.28,160.81) .. (387.22,160.69) .. controls (393.15,160.58) and (398.06,165.29) .. (398.17,171.23) .. controls (398.29,177.17) and (393.57,182.07) .. (387.64,182.19) -- cycle ;
%Straight Lines [id:da7097094801439052] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (157.77,190.7) -- (180.89,165.26) ;
\draw [shift={(183.58,162.31)}, rotate = 492.27] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9810591816143968] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (170.68,176.5) -- (196.49,148.11) ;



%Straight Lines [id:da8241882505112161] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (140.35,140.5) -- (174.72,140.39) ;
\draw [shift={(178.72,140.37)}, rotate = 539.8] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da2611609868412743] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (159.54,140.44) -- (197.91,140.31) ;



%Straight Lines [id:da47614353526842845] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (139.35,79.5) -- (173.72,79.39) ;
\draw [shift={(177.72,79.37)}, rotate = 539.8] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da12353656022449266] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (158.54,79.44) -- (196.91,79.31) ;



%Straight Lines [id:da9244769567454383] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (203.56,139.36) -- (244.12,125.15) ;
\draw [shift={(247.89,123.83)}, rotate = 520.7] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da19116006636637506] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (225.72,131.59) -- (270.06,116.07) ;



%Shape: Circle [id:dp44715716478629] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (194.27,133.26) .. controls (198.4,129) and (205.21,128.89) .. (209.47,133.03) .. controls (213.73,137.16) and (213.83,143.97) .. (209.7,148.23) .. controls (205.56,152.49) and (198.76,152.59) .. (194.5,148.46) .. controls (190.24,144.32) and (190.13,137.52) .. (194.27,133.26) -- cycle ;
%Straight Lines [id:da596545588195249] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (158.19,31.65) -- (182.01,56.44) ;
\draw [shift={(184.78,59.32)}, rotate = 226.15] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9940274280178878] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (171.48,45.48) -- (198.07,73.16) ;



%Straight Lines [id:da6607449984446108] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (204.8,78.87) -- (243.65,97.25) ;
\draw [shift={(247.27,98.96)}, rotate = 205.32] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da44325328985882484] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (226.04,88.91) -- (268.5,109) ;



%Straight Lines [id:da8012937935295932] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (277.93,111.78) -- (307.83,111.62) ;
\draw [shift={(311.83,111.6)}, rotate = 539.7] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da5277710562867892] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (294.88,111.69) -- (328.77,111.51) ;



%Shape: Circle [id:dp059347471941975094] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (202.48,68) .. controls (208.41,67.88) and (213.33,72.58) .. (213.46,78.52) .. controls (213.59,84.45) and (208.88,89.37) .. (202.94,89.5) .. controls (197.01,89.63) and (192.09,84.92) .. (191.96,78.98) .. controls (191.84,73.05) and (196.54,68.13) .. (202.48,68) -- cycle ;
%Shape: Circle [id:dp6978541118066315] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (272.47,101.73) .. controls (278.4,101.6) and (283.32,106.31) .. (283.45,112.24) .. controls (283.57,118.18) and (278.87,123.09) .. (272.93,123.22) .. controls (266.99,123.35) and (262.08,118.64) .. (261.95,112.71) .. controls (261.82,106.77) and (266.53,101.86) .. (272.47,101.73) -- cycle ;
%Straight Lines [id:da3106511050794307] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (329.67,225) -- (330.16,195.11) ;
\draw [shift={(330.22,191.11)}, rotate = 450.94] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da5296371031776572] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (329.94,208.06) -- (330.5,174.17) ;



%Straight Lines [id:da29499948240738316] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (329.67,166) -- (330.16,136.11) ;
\draw [shift={(330.22,132.11)}, rotate = 450.94] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da6360867035234687] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (329.94,149.06) -- (330.5,115.17) ;



%Straight Lines [id:da4999975103500194] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (329.67,107) -- (330.16,77.11) ;
\draw [shift={(330.22,73.11)}, rotate = 450.94] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8472176228876076] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (329.94,90.06) -- (330.5,56.17) ;



%Shape: Circle [id:dp7065951899558089] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (319.5,171.25) .. controls (319.5,165.31) and (324.31,160.5) .. (330.25,160.5) .. controls (336.19,160.5) and (341,165.31) .. (341,171.25) .. controls (341,177.19) and (336.19,182) .. (330.25,182) .. controls (324.31,182) and (319.5,177.19) .. (319.5,171.25) -- cycle ;
%Shape: Circle [id:dp9504171711256482] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (319.5,52.25) .. controls (319.5,46.31) and (324.31,41.5) .. (330.25,41.5) .. controls (336.19,41.5) and (341,46.31) .. (341,52.25) .. controls (341,58.19) and (336.19,63) .. (330.25,63) .. controls (324.31,63) and (319.5,58.19) .. (319.5,52.25) -- cycle ;
%Shape: Circle [id:dp5605658018945323] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (319.5,112.25) .. controls (319.5,106.31) and (324.31,101.5) .. (330.25,101.5) .. controls (336.19,101.5) and (341,106.31) .. (341,112.25) .. controls (341,118.19) and (336.19,123) .. (330.25,123) .. controls (324.31,123) and (319.5,118.19) .. (319.5,112.25) -- cycle ;
%Shape: Circle [id:dp6601696988934032] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (319.5,232.25) .. controls (319.5,226.31) and (324.31,221.5) .. (330.25,221.5) .. controls (336.19,221.5) and (341,226.31) .. (341,232.25) .. controls (341,238.19) and (336.19,243) .. (330.25,243) .. controls (324.31,243) and (319.5,238.19) .. (319.5,232.25) -- cycle ;
%Shape: Square [id:dp6032586376577502] 
\draw   (207,211) -- (277,211) -- (277,261) -- (207,261) -- cycle ;
%Straight Lines [id:da9000073679519673] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (405.46,405.81) -- (380.32,382.37) ;
\draw [shift={(377.39,379.64)}, rotate = 402.99] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da1998052619947841] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (391.43,392.73) -- (363.36,366.56) ;



%Straight Lines [id:da10302102108762967] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (355.05,422.6) -- (355.37,388.22) ;
\draw [shift={(355.4,384.22)}, rotate = 450.52] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7906047029533418] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (355.23,403.41) -- (355.58,365.04) ;



%Straight Lines [id:da9785228238662227] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (294.04,422.83) -- (294.36,388.46) ;
\draw [shift={(294.39,384.46)}, rotate = 450.52] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9974253974360028] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (294.22,403.65) -- (294.57,365.27) ;



%Straight Lines [id:da02311236078039225] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (354.7,359.38) -- (341.01,318.65) ;
\draw [shift={(339.73,314.86)}, rotate = 431.41999999999996] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7142159691220271] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (347.22,337.12) -- (332.24,292.59) ;



%Shape: Circle [id:dp8561066271641096] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (348.48,368.59) .. controls (344.28,364.4) and (344.26,357.6) .. (348.45,353.39) .. controls (352.63,349.18) and (359.44,349.16) .. (363.65,353.35) .. controls (367.86,357.54) and (367.87,364.35) .. (363.69,368.55) .. controls (359.5,372.76) and (352.69,372.78) .. (348.48,368.59) -- cycle ;
%Straight Lines [id:da16305645154559456] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (246.43,403.39) -- (271.52,379.89) ;
\draw [shift={(274.44,377.15)}, rotate = 496.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8685297545803499] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (260.43,390.27) -- (288.44,364.04) ;



%Straight Lines [id:da8230445055099023] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (294.23,357.38) -- (313.1,318.76) ;
\draw [shift={(314.85,315.17)}, rotate = 476.04] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da1164446176253795] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (304.54,336.27) -- (325.16,294.06) ;



%Shape: Circle [id:dp2954932444079179] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (283.34,359.56) .. controls (283.28,353.63) and (288.05,348.77) .. (293.99,348.72) .. controls (299.93,348.66) and (304.78,353.43) .. (304.84,359.37) .. controls (304.89,365.3) and (300.12,370.16) .. (294.19,370.21) .. controls (288.25,370.27) and (283.39,365.5) .. (283.34,359.56) -- cycle ;
%Shape: Circle [id:dp5371637813682735] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (317.94,290.01) .. controls (317.88,284.07) and (322.65,279.21) .. (328.59,279.16) .. controls (334.53,279.1) and (339.38,283.87) .. (339.44,289.81) .. controls (339.49,295.75) and (334.72,300.6) .. (328.79,300.66) .. controls (322.85,300.71) and (317.99,295.94) .. (317.94,290.01) -- cycle ;

% Text Node
\draw (362,51) node [scale=1.2]  {$321$};
% Text Node
\draw (352,229) node [scale=1.2]  {$e$};
% Text Node
\draw (280.68,135.21) node [scale=1.2,rotate=-0.63]  {$321^{-1}$};
% Text Node
\draw (358,111) node [scale=1.2]  {$32$};
% Text Node
\draw (308,170) node [scale=1.2]  {$3$};
% Text Node
\draw (346,82) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (345,138) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (317,200) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (301,92) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (242,74) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (188,37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (239,146) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (168,97) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (188,185) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (358,187) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (417,138) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (471,100) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (473,244) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (169,121) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (416,212) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (491,160) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (492,187) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (243,234) node [scale=1.2]  {$\xi ^{0}\setminus \{e_1\}$};
% Text Node
\draw (391.68,194.21) node [scale=1.2,rotate=-0.63]  {$31^{-1}$};
% Text Node
\draw (300,214) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (347,260) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$4$};
% Text Node
\draw (358.68,289.21) node [scale=1.2,rotate=-0.63]  {$4^{-1}$};
% Text Node
\draw (296,318) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (359,322) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$5$};
% Text Node
\draw (262.68,348.21) node [scale=1.2,rotate=-0.63]  {$4^{-1} 1^{-1}$};
% Text Node
\draw (400.68,350.21) node [scale=1.2,rotate=-0.63]  {$4^{-1} 5^{-1}$};
% Text Node
\draw (251,373) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (339,397) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (312,397) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (400,374) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$6$};
% Text Node
\draw (152,22) node [rotate=-50.06]  {$\cdots $};
% Text Node
\draw (510,259) node [rotate=-49.4]  {$\cdots $};
% Text Node
\draw (414,412) node [rotate=-42.51]  {$\cdots $};
% Text Node
\draw (128,78) node [rotate=-358.09]  {$\cdots $};
% Text Node
\draw (129,138) node [rotate=-358.09]  {$\cdots $};
% Text Node
\draw (530,141) node [rotate=-358.09]  {$\cdots $};
% Text Node
\draw (531,202) node [rotate=-358.09]  {$\cdots $};
% Text Node
\draw (291,432) node [rotate=-270.55]  {$\cdots $};
% Text Node
\draw (352,432) node [rotate=-270.55]  {$\cdots $};
% Text Node
\draw (149,196) node [rotate=-311.7]  {$\cdots $};
% Text Node
\draw (508,84) node [rotate=-311.7]  {$\cdots $};
% Text Node
\draw (237,409) node [rotate=-315.69]  {$\cdots $};

\end{tikzpicture}

}
\caption{321 stem configuration for the renewal shift. The directed graph denoted by $\xi^0\setminus \{e_1\}$ is 
obtained removing the root $e$ and the edge $e_1$, labeled with $1$, from the directed graph associated to the 
empty configuration $\xi^0$ in the figure 3.}

\end{figure}
Since we can construct any infinite positive admissible word by finite positive admissible words, we may construct a sequence of configurations in $Y_A$ which converges to configurations in $\Sigma_A$, and therefore $Y_A$ is dense in $X_A$ as well as $\Sigma_A$. Also note that $Y_A$ is countable, therefore any  measure which vanishes on $\Sigma_A$ is necessarily an atomic measure. In other words, these measures are written in the form  $\mu(E) = \sum_{\omega \in R} \mathbbm{1}_{E}(\omega\xi^0) c_\omega$, for any measurable set $E \subset X_A$, the brackets denote the boolean value and

\begin{equation}\label{eq:coefficients_Y_A_confomal}
    c_\omega := \mu(\{\omega \xi^0\}), \quad \omega \in R.
\end{equation}
From now on, the idea is to consider the family of variables $\{c_\omega\}_{\omega \in R}$ and to solve the system of equations corresponding to the Denker-Urba\'nski conformality condition. In order to do it we describe the how the shift acts on $Y_A$. We will keep the notation $\sigma$ for the shift action on $Y_A\setminus\{\xi^0\}$, defined as
\begin{equation*}
    \sigma(\xi)_{\omega} = \xi_{\omega_0^{-1}\omega}.
\end{equation*}
The assignment above only makes sense for non-zero positive stem which justifies the exclusion of $\xi^0$ on the domain of the shift map. From now we will omit $\xi^0$ from $\omega \xi^0$. The Denker-Urba\'nski conformality condition \eqref{eq:conformal_Ur_sets_potential} here is written with
\begin{equation*}
    D(\omega) = e^{ F(\omega)},
\end{equation*}
and we get the general formulation for the conformal measures in $Y_A$ in the theorem below.


\begin{theorem}\label{theorem.coeficientes} A measure $\mu$ which vanishes on $\Sigma_A$ satisfies the Denker-Urba\'nski conformality condition if and only if the coefficients $c_\omega$ in \eqref{eq:coefficients_Y_A_confomal} satisfies
\begin{equation*}
    c_\omega D(\omega) = c_{\sigma(\omega)}.
\end{equation*}
\end{theorem}

\begin{proof}  It is straightforward from the Denker-Urba\'nski conformality condition for characteristic functions on the special set $\{\omega\}$, hence the condition above is necessary. The converse is clear because, for every special set $E$, $$\sum_{\omega\in E}D(\omega)c_\omega=\sum_{\omega\in E}c_{\sigma(\omega)}$$ implies the Denker-Urba\'nski corformality condition.  \qed
\end{proof}

\begin{proposition}\label{prop:cardinality_words_length} There is exactly one element in $Y_A$ whose stem has
length zero, namely $\xi^0$, and for each $n \geq 1$, there are exactly
$2^{n-1}$ elements in $Y_A$ whose stem has length $n$.

\end{proposition}

\begin{proof} Every stem of a configuration in $Y_A$ is admissible and it ends with $1$. Hence, for any $n \in \mathbb{N}$ we have that
\begin{equation*}
    \{\omega\xi^0 \in Y_A: |\omega| = n\} = \sigma^{-(n-1)}(1),
\end{equation*}
where $\sigma$ is the shift map restricted to $Y_A$. Since the transition matrix is given by $A(s+1,s) = A(1,s) = 1$ for all $s \in \mathbb{N}$ and zero in the rest of entries we conclude that $|\sigma^{-1}(\eta)| = 2$ for all $\eta \in Y_A$. It follows that
\begin{equation*}
    |\{\omega\xi^0 \in Y_A: |\omega| = n\}| = |\sigma^{-(n-1)}(1)| = 2^{n-1}.
\end{equation*}
Indeed, it is obvious for $n=1$. Then suppose that the result above follows for $k \in \mathbb{N}$, i.e.,
\begin{equation*}
    |\sigma^{-(k-1)}(1)| = 2^{k-1},
\end{equation*}
then for a word $\eta$ in $\sigma^{-(k-1)}(1)$ we have that $|\sigma^{-1}(\eta)| = 2$ and then
\begin{equation*}
    |\sigma^{-k}(1)| = |\sigma^{-1}(\sigma^{-(k-1)}(1))| = 2 |\sigma^{-(k-1)}(1)| = 2^{k}.
\end{equation*}
The proof is complete. \qed
\end{proof}

Now, observe that the identity $c_{\omega} D(\omega) = c_{\sigma(\omega)}$ leads to
\begin{equation*}
c_{\omega} \prod_{i=0}^{|\omega|-1}D(\sigma^i(\omega)) = c_{\emptyset}, \quad \omega \in R
\end{equation*}
where $c_\emptyset := \mu(\{\xi^0\})$. It is rewritten as
\begin{equation}\label{eq:c_omega_new}
c_{\omega} e^{ (S_{|\omega|}F)(\omega)} = c_{\emptyset}, \quad \omega \in R,
\end{equation}
where $S_n$ is the Birkhoff's sum
\begin{equation*}
    (S_n g)(x) := \sum_{i=0}^{n-1}g(\sigma^i(x)), \quad g \in C(Y_A).
\end{equation*}
In order to construct any potential which would give a $e^F$-conformal probability measure in $Y_A$ we must keep $c_\emptyset > 0$, otherwise all other $c_\omega$'s are zero by \eqref{eq:c_omega_new}. That is equivalent to impose $c_\omega > 0$ for all $\omega \in R$, since it is a necessary condition to obtain $c_\emptyset > 0$. At the same time we wish to have
\begin{equation}\label{eq:c_omega_probability}
    \sum_{\omega \in R}c_\omega = 1,
\end{equation}
which imposes that $\mu$ is in fact a probability measure.
\vv\noindent
\begin{example}We first look the class of potentials that depends only on the length of the word, i.e, $F(\omega)=F(|\omega|)$. In this case, the coefficients $c_\omega$'s have the same property, i.e., $c_\omega = c_{|\omega|}$. This imposition affects directly \eqref{eq:c_omega_probability}, one may rewrite it as
\begin{equation*}
    c_\emptyset+\sum_{n \in \mathbb{N}}\sum_{\substack{\omega \in R \\ |\omega| = n}}c_\omega \stackrel{\text{prop. \ref{prop:cardinality_words_length}}}{=} c_\emptyset + \sum_{n \in \mathbb{N}} 2^{n-1} c_{n}=1,
\end{equation*}
where $c_n$ is the coefficient $c_\omega$ when $|\omega|=n$. The equality above imposes $c_\emptyset \in (0,1)$. We summarize the conditions on the atomic probability $\mu$ which vanishes on $\Sigma_A$
\begin{equation*}
    \begin{cases}
        c_\emptyset + \sum_{n \in \mathbb{N}} 2^{n-1} c_{n}=1,\\
        c_\emptyset \in (0,1).
    \end{cases}
\end{equation*}
By \eqref{eq:c_omega_new} $|\omega|=n$ we have $c_n e^{(S_nF)(\omega)} = c_\emptyset$, then
\begin{equation}\label{eq:S_n_F}
    (S_nF)(\omega) = \log \left(\frac{c_\emptyset}{c_n}\right).
\end{equation}
The identity above allow us to determine $F$ in $Y_A\setminus\{\xi^0\}$,
\begin{align*}
    F(\omega) &= \sum_{i=0}^{n-1}F[\sigma^i(\omega)] - \sum_{i=1}^{n-1}F[\sigma^i(\omega)] = \log \left(\frac{c_{n-1}}{c_n}\right),
\end{align*}
where $c_0=c_\emptyset$. For $\alpha>2$, take $c_n = \frac{\alpha-2}{\alpha^n(\alpha-1)}$. The potential which makes $\mu$, defined by the coefficients $c_n$,  a $e^{F}$-conformal probability measure is given by the constant function $F = \log \alpha$ defined in $X_A \setminus \{\xi^0\}$. 
\vv \noindent
\end{example} 
\begin{remark}
In fact, because of the structure of our renewal shift, potentials that depends only on the length of the word, are the constant one. To see this, take any continuous potential $F:X_A\setminus\{\xi^0\} \to \mathbb{R}$ such that, for any $\omega \in Y_A$ we have $F(\omega)= g(|\omega|)$ where $g: \mathbb{N} \rightarrow \mathbb{R}$. In this case, $F$ is a constant function. Let $x \neq y$ on $\Sigma_A$ and consider two sequences $(x_n)_{n \in \mathbb{N}}$ and $(y_n)_{n \in \mathbb{N}}$ on $Y_A$ such that $x_n \rightarrow x$ and $y_n \rightarrow y$, with $|x_n| = |y_n|=n$, this choice is possible because $A(1,n) = 1$ for every $n \in \mathbb{N}$. This implies that $F(x)=F(y)$, since $\Sigma_A$ is dense on $X_A$,  $F$ is constant.
\end{remark} 
\begin{theorem}\label{theorem.potentialwithonecoordinate} Consider potential $F:X_A\setminus\{\xi^0\} \to \mathbb{R}$ and $\beta>0$, we have the following:
\begin{itemize}
    \item[(i)] If $M=\inf F>0$, for $\beta>\frac{\log 2}{M}$, there exists a unique $e^{\beta F}$-conformal probability measure $\mu_\beta$ that vanishes in $\Sigma_A$.
    \item[(ii)] If $0\leq \sup F < + \infty$ and $\beta\leq \frac{\log 2}{\sup F}$, there are no $e^{\beta F}$-conformal probability measures that vanish in $\Sigma_A$.
\end{itemize}
\end{theorem}

\begin{proof} The equations \eqref{eq:c_omega_new} and \eqref{eq:c_omega_probability} give us

\begin{equation}\label{eq:conformal_Y_A_formula}
    1 + \sum_{\omega \in R\setminus \{\xi^0\}} e^{-\beta\sum_{j=0}^{|\omega|-1}F(\sigma^j(\omega))} = \frac{1}{c_\emptyset}>0.
\end{equation}
Since $F(\omega) \geq M$ for all $\omega \in R$, by proposition \ref{prop:cardinality_words_length} we obtain
\begin{align*}
    1 + \sum_{\omega \in R\setminus \{\xi^0\}} e^{-\beta\sum_{j=0}^{|\omega|-1}F(\sigma^j(\omega))}\leq  1 + \frac{1}{2}\sum_{n \in \mathbb{N}} \left(\frac{2}{e^{\beta M}}\right)^{n}.
\end{align*}
The series $\sum_{n \in \mathbb{N}}  \left(\frac{2}{e^{\beta M}}\right)^{n}$ converges if $\beta > \frac{\log 2}{M}$, therefore the validity of the last inequality grants that the series $\sum_{\omega \in R\setminus \{\xi^0\}} e^{-\beta\sum_{j=0}^{|\omega|-1}F(\sigma^j(\omega))}$ converges and we obtain the existence of a $e^{\beta F}$-conformal probability measure $\mu_\beta$ that vanishes on $\Sigma_A$, given by the coefficients $c_\omega$ in equation \eqref{eq:c_omega_new}. The uniqueness is straightforward. This proves item (i) and a similar procedure proves item (ii). Indeed, it is clear that
\begin{equation}
-\beta \sum_{j=0}^{n-1}F(\sigma(\omega))\geq -\beta n \sup F.   
\end{equation}
Hence,
\begin{align*}
    \sum_{\omega \in R\setminus \{\xi^0\}} e^{-\beta\sum_{j=0}^{|\omega|-1}F(\sigma^j(\omega))}\geq 
    1/2\sum_{n\in \mathbb{N}}\left(\frac{2}{e^{\beta \sup F}}\right)^n.
\end{align*}
The last sum diverges if $\beta\leq \frac{\log 2}{\sup F}$, which means that no $e^{\beta F}$-conformal probability measure vanishing on $\Sigma_A$ can be obtained  in such interval.\qed
\end{proof}

\begin{corollary}\label{pt}
Let $F\equiv1$. Then, for the constant $\beta_c=\log 2$, the result follows:

\begin{itemize}
    \item[(i)] For $\beta>\beta_c$ we have a unique $e^\beta$-conformal probability measure that vanishes on $\Sigma_A$.
    \item[(ii)] For $\beta\leq\beta_c$ there is no $e^\beta$- conformal probability measure that vanishes on $\Sigma_A$.
\end{itemize}
\end{corollary}
\begin{proof}
Take $M=1$ and apply theorem \ref{theorem.potentialwithonecoordinate} for the constant potential $F\equiv 1$. For $\beta_c$, it is a straightforward calculation that the series associated with it diverges.\qed
\end{proof}
\medskip

Let $\mu_\beta$, $\beta > \log 2$, be the conformal measure of the corollary \ref{pt} for the inverse of temperature $\beta$. This measure is explicitly obtained by the equation \eqref{eq:conformal_Y_A_formula} combined with \eqref{eq:c_omega_new}. By denoting $\mu_\beta(\{\alpha \xi^0\}):= c_{\alpha}^\beta$ we obtain
\begin{equation}\label{eq:conformal_measure_Y_A_explicit}
     c_\alpha^\beta := \frac{e^{-\beta |\alpha|}}{1+\frac{1}{2}\sum_{n \in \mathbb{N}}e^{n(\log 2 - \beta)}} = \frac{e^{-|\alpha|\beta}(e^\beta-2)}{e^\beta-1}.
\end{equation}


 Perhaps the corollary \ref{pt} can be seen as a pathological fact in contrast with the Sarig's theorem in \cite{Sa1} about renewal shifts considering $\Sigma_A$ instead of $X_A$. He proved, for potentials regular enough, if we have a phase transition at some $\beta_c$, then there exist conformal measures at high temperatures ($\beta < \beta_c$)  and do not exist at low temperatures ($\beta > \beta_c$). Our theorem tells us the exact opposite behavior for the conformal measures which vanish on $\Sigma_A$. However, is not difficult to verify that this Renewal shift is positive recurrent for all $\beta>0$. Then, we have only one conformal measure at high temperatures and several conformal probability measures in low temperatures ($\beta > \beta_c$), the typical behavior of ferromagnetic systems in statistical mechanics. Nevertheless, the Sarig's conformal measure is 
intrinsically connected with the ones of the corollary \ref{pt}: there exists the weak$^*$-limit of the net of measures $\{\mu_\beta\}_{\beta > \beta_c}$ of the aforementioned corollary when $\beta \to \beta_c$. In order to verify this fact, we need to discuss some particularities of the topology of $X_A$ of the renewal shift to study the weak$^*$ convergence of measure on this space as it follows. In fact, we will study the weak convergence of probability measures on $X_A$ for general transitive transition matrices $A$ in the Section \ref{convergence}.

\section{Empty stems and extremal conformal measures on $Y_A$}
As we did in the previous section, here we will study conformal measures which live in $Y_A$, but for shifts that have more than one configuration with empty stem. The reader will notice some similarities with the renewal shift example. Essentially, there is a bijection between the number of extremal conformal probability measures living on $Y_A$ and configurations with empty stem.


\begin{example}(Pair Renewal Shift)\\
Consider the transition matrix satisfying
\begin{equation*}
    A(1,n)=A(2,2n)=A(n+1,n) = 1, \forall n\in \mathbb{N}
\end{equation*}
and zero otherwise. This shift will be called \emph{Pair Renewal Shift}. The associated transition matrix becomes
\begin{equation*}
    A = \begin{pmatrix}
    1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \cdots\\
    1 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & \cdots\\
    0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \cdots\\
    0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & \cdots\\
    0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 &\cdots\\
    \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \ddots
    \end{pmatrix}.
\end{equation*}
The current transition matrix $A$ has a full line of $1$`s in the first row and then $\mathcal{O}_A$ is unital as the renewal shift and therefore $X_A$ is compact. The only two possibilities for limit points on the space of columns of $A$ are
\begin{equation*}
    c_1 = \begin{pmatrix} 1 \\ 0 \\0 \\ 0 \\ 0 \\\vdots \end{pmatrix} \quad \text{and} \quad c_2 = \begin{pmatrix} 1 \\ 1 \\0 \\ 0 \\ 0 \\\vdots \end{pmatrix}.
\end{equation*}
By taking limits, the only possibilities for finite stems are:
\begin{enumerate}
    \item words ending with 1 (two configurations associated);
    \item words ending with 2 (unique configuration associated);
    \item empty word (two configurations associated);
\end{enumerate}
and the proof is similar to the example of the renewal shift. Consider a sequence $\{\xi(n)\}_{n \in \mathbb{N}}$ in $\Sigma_A$. In order to obtain the two possible configurations for a stem $\omega$ ending with 1, just choose $\xi(n)$ such that $\xi(n)_{\omega (2n-1)} = 1$ and you will get as a limit the configuration $\xi \in Y_A$ such that $\kappa(\xi) = \omega$ and $R_\xi(\omega) = c_1$. The another configuration is obtained by choosing $\xi(n)_{\omega (2n)} = 1$, and the limit is a configuration $\xi \in Y_A$ such that $\kappa(\xi) = \omega$ and $R_\xi(\omega) = c_2$. A similar argument is used for the empty stem case with roots $R_\xi(e) = c_1$ and $R_\xi(e) = c_2$. For finite stems ending with 2, we only have similar options for $\xi(n)_{\omega (2n)} = 1$, where $\omega$ ends with 2, and the root of the stem associated to the limit configuration $\xi$ is $R_\xi(\omega) = c_2$. The empty stem configurations are the following:
\vv

\scalebox{.7}{

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,397); %set diagram left start at 0, and has height of 397

%Straight Lines [id:da39196091510602704] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (111.54,196.48) -- (172.66,132.6) ;
\draw [shift={(175.42,129.71)}, rotate = 493.74] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da34693565982805175] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (143.48,163.1) -- (207.37,96.33) ;



%Straight Lines [id:da41660416136444123] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (27.71,317.16) -- (78.32,244.67) ;
\draw [shift={(80.6,241.39)}, rotate = 484.92] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da16835481109788386] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (54.16,279.28) -- (107.05,203.51) ;



%Straight Lines [id:da06301762596884275] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (94.68,262.26) -- (103.71,229.09) ;
\draw [shift={(104.76,225.23)}, rotate = 465.23] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da466612942400938] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (99.72,243.75) -- (109.8,206.72) ;



%Straight Lines [id:da21053471940405544] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (56.79,226.36) -- (87.36,210.63) ;
\draw [shift={(90.92,208.79)}, rotate = 512.76] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9839440216199387] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (73.85,217.58) -- (107.98,200.01) ;



%Shape: Circle [id:dp1080155478935676] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (101.07,194.5) .. controls (102.82,188.83) and (108.83,185.64) .. (114.51,187.39) .. controls (120.18,189.13) and (123.37,195.15) .. (121.62,200.82) .. controls (119.88,206.5) and (113.86,209.68) .. (108.19,207.94) .. controls (102.51,206.19) and (99.33,200.18) .. (101.07,194.5) -- cycle ;

%Straight Lines [id:da26969478088598686] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (193.35,154.16) -- (203.43,121.3) ;
\draw [shift={(204.61,117.48)}, rotate = 467.06] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da537479703459457] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (198.98,135.82) -- (210.24,99.13) ;



%Straight Lines [id:da1489422813835133] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (152.18,108.09) -- (185.54,99.81) ;
\draw [shift={(189.43,98.85)}, rotate = 526.05] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7792787876425982] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (170.8,103.47) -- (208.05,94.22) ;



%Straight Lines [id:da22761089753940977] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (214.77,89.7) -- (233.24,66.05) ;
\draw [shift={(235.7,62.89)}, rotate = 487.98] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9017850635623115] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (225.23,76.3) -- (246.17,49.49) ;



%Shape: Circle [id:dp3164357514391066] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (201.88,91.21) .. controls (203.47,85.48) and (209.39,82.13) .. (215.11,83.71) .. controls (220.83,85.29) and (224.19,91.22) .. (222.61,96.94) .. controls (221.02,102.66) and (215.1,106.02) .. (209.38,104.43) .. controls (203.66,102.85) and (200.3,96.93) .. (201.88,91.21) -- cycle ;
%Straight Lines [id:da8791965782966649] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (257.45,195.69) -- (277.58,173.6) ;
\draw [shift={(280.28,170.64)}, rotate = 492.35] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da25817402126581146] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (268.86,183.16) -- (291.7,158.12) ;



%Straight Lines [id:da14491035916354633] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (389.83,212.1) -- (353.73,199.07) ;


%Straight Lines [id:da19389458815653082] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (390.05,253.85) -- (367.99,227.49) ;
\draw [shift={(365.43,224.42)}, rotate = 410.08000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8301791594924218] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (377.74,239.13) -- (353.12,209.7) ;



%Straight Lines [id:da26403889763728317] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (407.88,218.61) -- (375.54,206.94) ;
\draw [shift={(371.78,205.58)}, rotate = 379.84000000000003] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da6000533250852014] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (349.25,200.83) -- (316.32,173.22) ;
\draw [shift={(313.26,170.65)}, rotate = 399.99] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8592052704483201] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (331.26,185.74) -- (295.26,155.55) ;



%Shape: Circle [id:dp49384290579378487] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (346.81,211.42) .. controls (341.04,210.04) and (337.48,204.25) .. (338.85,198.47) .. controls (340.23,192.7) and (346.03,189.13) .. (351.81,190.51) .. controls (357.58,191.89) and (361.15,197.69) .. (359.77,203.46) .. controls (358.39,209.24) and (352.59,212.8) .. (346.81,211.42) -- cycle ;
%Straight Lines [id:da8952680034543073] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (306.76,223.9) -- (297.71,181.89) ;
\draw [shift={(296.87,177.98)}, rotate = 437.85] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da26830176711736164] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (301.82,200.94) -- (291.92,155.02) ;



%Straight Lines [id:da17627874984611447] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (244.1,279.87) -- (248.16,237.08) ;
\draw [shift={(248.54,233.1)}, rotate = 455.43] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da23229515149196267] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (246.32,256.49) -- (250.76,209.72) ;



%Straight Lines [id:da05099536846064279] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (201.93,259.11) -- (229.05,225.77) ;
\draw [shift={(231.58,222.67)}, rotate = 489.14] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7647946153736895] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (216.75,240.89) -- (246.4,204.45) ;



%Shape: Circle [id:dp4824633300408676] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (244.4,195.69) .. controls (247.85,190.85) and (254.56,189.73) .. (259.4,193.18) .. controls (264.23,196.63) and (265.35,203.34) .. (261.91,208.17) .. controls (258.46,213.01) and (251.74,214.13) .. (246.91,210.68) .. controls (242.08,207.23) and (240.95,200.52) .. (244.4,195.69) -- cycle ;
%Straight Lines [id:da08597760571208113] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (292.25,149.93) -- (286.48,120.6) ;
\draw [shift={(285.71,116.68)}, rotate = 438.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da4890337805762177] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (288.98,133.31) -- (282.44,100.05) ;



%Shape: Circle [id:dp1540715774905974] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (283.41,157.19) .. controls (282.17,151.39) and (285.87,145.68) .. (291.67,144.43) .. controls (297.48,143.19) and (303.19,146.89) .. (304.43,152.7) .. controls (305.68,158.5) and (301.98,164.22) .. (296.17,165.46) .. controls (290.36,166.7) and (284.65,163) .. (283.41,157.19) -- cycle ;
%Straight Lines [id:da9137824962159418] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (350.29,111.5) -- (308.44,101.74) ;
\draw [shift={(304.55,100.83)}, rotate = 373.13] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7774708981572266] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (327.42,106.17) -- (281.67,95.5) ;



%Straight Lines [id:da7416988271961764] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (408.42,135.78) -- (377.1,121.62) ;
\draw [shift={(373.45,119.97)}, rotate = 384.33000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da6348644009458194] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (390.93,127.88) -- (355.97,112.06) ;



%Straight Lines [id:da1126287842062138] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (383.7,164.06) -- (363.79,136.04) ;
\draw [shift={(361.47,132.78)}, rotate = 414.6] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8953517291345314] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (372.59,148.42) -- (350.36,117.14) ;



%Shape: Circle [id:dp03518419711696785] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (352.9,122.05) .. controls (347.13,123.43) and (341.33,119.86) .. (339.95,114.09) .. controls (338.57,108.31) and (342.14,102.52) .. (347.91,101.14) .. controls (353.69,99.76) and (359.48,103.32) .. (360.86,109.1) .. controls (362.24,114.87) and (358.68,120.67) .. (352.9,122.05) -- cycle ;
%Straight Lines [id:da20065971342230404] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (279.02,92.2) -- (263.26,66.81) ;
\draw [shift={(261.15,63.41)}, rotate = 418.16999999999996] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da02217639431093721] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (270.08,77.81) -- (252.21,49.01) ;



%Shape: Circle [id:dp19775678602869995] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (273.32,102.12) .. controls (270.1,97.13) and (271.54,90.48) .. (276.54,87.26) .. controls (281.53,84.05) and (288.18,85.49) .. (291.39,90.48) .. controls (294.61,95.48) and (293.17,102.13) .. (288.17,105.34) .. controls (283.18,108.56) and (276.53,107.11) .. (273.32,102.12) -- cycle ;
%Shape: Circle [id:dp5438304644818241] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (239.5,46.62) .. controls (239.5,40.68) and (244.31,35.87) .. (250.25,35.87) .. controls (256.19,35.87) and (261,40.68) .. (261,46.62) .. controls (261,52.56) and (256.19,57.37) .. (250.25,57.37) .. controls (244.31,57.37) and (239.5,52.56) .. (239.5,46.62) -- cycle ;
%Straight Lines [id:da05083135509579295] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (99.25,150.25) -- (126.11,128.79) ;
\draw [shift={(129.23,126.3)}, rotate = 501.38] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da9779137006099309] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (114.24,138.27) -- (144.23,114.32) ;



%Straight Lines [id:da08500520747478735] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (85.3,115.38) -- (119.31,110.39) ;
\draw [shift={(123.27,109.8)}, rotate = 531.65] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8067435405491961] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (104.29,112.59) -- (142.26,107.02) ;



%Shape: Circle [id:dp8539216574088145] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (137.96,107.05) .. controls (139.04,101.21) and (144.65,97.36) .. (150.49,98.44) .. controls (156.33,99.53) and (160.18,105.14) .. (159.09,110.97) .. controls (158.01,116.81) and (152.4,120.66) .. (146.56,119.58) .. controls (140.73,118.5) and (136.87,112.89) .. (137.96,107.05) -- cycle ;
%Straight Lines [id:da7287805950151937] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (189.4,219.69) -- (191.38,185.38) ;
\draw [shift={(191.61,181.38)}, rotate = 453.3] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da28073553466919077] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (190.5,200.54) -- (192.71,162.23) ;



%Straight Lines [id:da08110274607275714] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (154.13,206.77) -- (173.14,178.13) ;
\draw [shift={(175.35,174.8)}, rotate = 483.57] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da38122358321418803] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (164.74,190.79) -- (185.97,158.81) ;



%Shape: Circle [id:dp6332306366072333] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (182.3,162.95) .. controls (178.94,158.05) and (180.18,151.36) .. (185.08,148) .. controls (189.97,144.64) and (196.66,145.89) .. (200.02,150.78) .. controls (203.38,155.68) and (202.14,162.37) .. (197.24,165.73) .. controls (192.35,169.09) and (185.66,167.84) .. (182.3,162.95) -- cycle ;
%Straight Lines [id:da5640519561262781] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (359.79,361.97) -- (328.27,279.38) ;
\draw [shift={(326.84,275.64)}, rotate = 429.11] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da42843158531235725] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (343.31,318.8) -- (310.36,232.47) ;



%Straight Lines [id:da3173768933400225] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (352,275.72) -- (329.64,249.61) ;
\draw [shift={(327.04,246.57)}, rotate = 409.41999999999996] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da5774372082399238] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (339.52,261.15) -- (314.56,232) ;



%Straight Lines [id:da3524474313532311] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (301.02,286.89) -- (305.18,252.76) ;
\draw [shift={(305.67,248.79)}, rotate = 456.95] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da48253821043119494] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (303.34,267.84) -- (307.99,229.74) ;



%Shape: Circle [id:dp7242997049224105] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (299.55,232.36) .. controls (295.84,227.72) and (296.58,220.96) .. (301.22,217.25) .. controls (305.85,213.53) and (312.61,214.28) .. (316.33,218.91) .. controls (320.04,223.54) and (319.29,230.31) .. (314.66,234.02) .. controls (310.03,237.74) and (303.26,236.99) .. (299.55,232.36) -- cycle ;



% Text Node
\draw (268,128.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (353,144.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (321,87.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (288,198.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (329,161.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (200.68,66.58) node [scale=1.2,rotate=-0.63]  {$2^{-1}$};
% Text Node
\draw (168,81.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (102,132.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (220,126.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (221,55.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (252,17.37) node [scale=1.2]  {$e$};
% Text Node
\draw (275,56.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (297.68,71.58) node [scale=1.2,rotate=-0.63]  {$1^{-1}$};
% Text Node
\draw (388.2,174.78) node [rotate=-232.89]  {$\cdots $};
% Text Node
\draw (417.11,142.19) node [rotate=-203.76]  {$\cdots $};
% Text Node
\draw (400,113.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (395.38,264.18) node [rotate=-228.37]  {$\cdots $};
% Text Node
\draw (417.05,224.31) node [rotate=-199.27]  {$\cdots $};
% Text Node
\draw (193.52,265.89) node [rotate=-311.27]  {$\cdots $};
% Text Node
\draw (243.95,291.82) node [rotate=-97.96]  {$\cdots $};
% Text Node
\draw (257,171.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (215,216.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (264,240.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (380,191.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (368,248.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (72.81,114.92) node [rotate=-354.57]  {$\cdots $};
% Text Node
\draw (133,153.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (89.59,155.08) node [rotate=-320.81]  {$\cdots $};
% Text Node
\draw (107,92.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (145.45,215.76) node [rotate=-306.49]  {$\cdots $};
% Text Node
\draw (186.54,230.11) node [rotate=-272.73]  {$\cdots $};
% Text Node
\draw (357.16,285.21) node [rotate=-228.85]  {$\cdots $};
% Text Node
\draw (297.12,297.83) node [rotate=-275.24]  {$\cdots $};
% Text Node
\draw (328,321.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (290,262.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (337,240.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (360.71,373.71) node [rotate=-249.33]  {$\cdots $};
% Text Node
\draw (18.51,324.52) node [rotate=-305.14]  {$\cdots $};
% Text Node
\draw (45.17,230.41) node [rotate=-327.98]  {$\cdots $};
% Text Node
\draw (90.56,271.55) node [rotate=-281.59]  {$\cdots $};
% Text Node
\draw (153,188.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (205,182.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (66,200.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (42,270.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (117,244.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};

\hspace{12cm}

\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (122.35,159.36) -- (152.24,158.9) ;
\draw [shift={(156.24,158.84)}, rotate = 539.11] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da25817402126581146] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (139.29,159.1) -- (173.18,158.57) ;



%Straight Lines [id:da17811792721925235] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (205.85,271.13) -- (186.5,238) ;


%Straight Lines [id:da005191481511867657] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (215.53,287.7) -- (198.19,258.02) ;
\draw [shift={(196.18,254.56)}, rotate = 419.71000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;



%Straight Lines [id:da19389458815653082] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (178.83,295.79) -- (179.37,261.42) ;
\draw [shift={(179.43,257.42)}, rotate = 450.9] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8301791594924218] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (179.13,276.61) -- (179.74,238.23) ;



%Straight Lines [id:da6000533250852014] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (181.49,229.77) -- (179.05,186.86) ;
\draw [shift={(178.83,182.87)}, rotate = 446.75] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8592052704483201] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (180.16,206.32) -- (177.49,159.42) ;



%Shape: Circle [id:dp49384290579378487] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (172.11,235.25) .. controls (169.16,230.09) and (170.94,223.52) .. (176.09,220.57) .. controls (181.24,217.62) and (187.81,219.41) .. (190.76,224.56) .. controls (193.71,229.71) and (191.93,236.28) .. (186.78,239.23) .. controls (181.63,242.18) and (175.06,240.4) .. (172.11,235.25) -- cycle ;
%Straight Lines [id:da8952680034543073] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (135.58,214.62) -- (159.99,179.24) ;
\draw [shift={(162.26,175.95)}, rotate = 484.61] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da26830176711736164] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (148.92,195.28) -- (175.6,156.62) ;



%Straight Lines [id:da17627874984611447] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (51.88,207.31) -- (85.83,180.96) ;
\draw [shift={(88.99,178.51)}, rotate = 502.19] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da23229515149196267] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (70.44,192.91) -- (107.55,164.1) ;



%Straight Lines [id:da05099536846064279] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (38.11,162.36) -- (80.98,159.29) ;
\draw [shift={(84.97,159)}, rotate = 535.9] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7647946153736895] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (61.54,160.68) -- (108.4,157.32) ;



%Shape: Circle [id:dp4824633300408676] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (113.41,149.86) .. controls (119.3,149.06) and (124.71,153.18) .. (125.51,159.06) .. controls (126.31,164.95) and (122.19,170.36) .. (116.31,171.16) .. controls (110.43,171.96) and (105.01,167.84) .. (104.21,161.96) .. controls (103.41,156.08) and (107.53,150.66) .. (113.41,149.86) -- cycle ;
%Straight Lines [id:da08597760571208113] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (179.53,153.37) -- (196.94,129.08) ;
\draw [shift={(199.27,125.83)}, rotate = 485.63] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da4890337805762177] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (189.4,139.6) -- (209.14,112.05) ;



%Shape: Circle [id:dp1540715774905974] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (168.18,151.91) .. controls (171.56,147.02) and (178.25,145.81) .. (183.14,149.18) .. controls (188.02,152.56) and (189.24,159.26) .. (185.86,164.14) .. controls (182.48,169.02) and (175.78,170.24) .. (170.9,166.86) .. controls (166.02,163.48) and (164.8,156.79) .. (168.18,151.91) -- cycle ;
%Straight Lines [id:da9137824962159418] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (245.68,163.69) -- (224.33,126.4) ;
\draw [shift={(222.34,122.92)}, rotate = 420.21000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7774708981572266] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (234.01,143.31) -- (210.67,102.54) ;



%Straight Lines [id:da7416988271961764] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (284.5,207.17) -- (262.88,180.44) ;
\draw [shift={(260.36,177.33)}, rotate = 411.03] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da6348644009458194] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (272.43,192.25) -- (248.3,162.41) ;



%Straight Lines [id:da1126287842062138] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (249.71,221.33) -- (244.51,187.35) ;
\draw [shift={(243.91,183.39)}, rotate = 441.3] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da8953517291345314] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (246.81,202.36) -- (241.01,164.42) ;



%Shape: Circle [id:dp03518419711696785] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (241.07,169.95) .. controls (235.29,168.59) and (231.71,162.8) .. (233.08,157.02) .. controls (234.44,151.24) and (240.23,147.67) .. (246.01,149.03) .. controls (251.79,150.39) and (255.37,156.18) .. (254,161.96) .. controls (252.64,167.74) and (246.85,171.32) .. (241.07,169.95) -- cycle ;
%Straight Lines [id:da20065971342230404] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (211.64,100.1) -- (210.68,70.23) ;
\draw [shift={(210.55,66.23)}, rotate = 448.16] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da02217639431093721] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (211.1,83.17) -- (210.01,49.29) ;



%Shape: Circle [id:dp19775678602869995] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (201.74,105.84) .. controls (201.45,99.91) and (206.03,94.87) .. (211.96,94.58) .. controls (217.89,94.29) and (222.93,98.87) .. (223.22,104.8) .. controls (223.5,110.73) and (218.93,115.77) .. (213,116.06) .. controls (207.07,116.34) and (202.03,111.77) .. (201.74,105.84) -- cycle ;
%Shape: Circle [id:dp5438304644818241] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (198.5,46.62) .. controls (198.5,40.68) and (203.31,35.87) .. (209.25,35.87) .. controls (215.19,35.87) and (220,40.68) .. (220,46.62) .. controls (220,52.56) and (215.19,57.37) .. (209.25,57.37) .. controls (203.31,57.37) and (198.5,52.56) .. (198.5,46.62) -- cycle ;
%Straight Lines [id:da7250818201298804] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (382.68,316.19) -- (325.42,248.83) ;
\draw [shift={(322.83,245.79)}, rotate = 409.63] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da7216284381439715] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (352.76,280.99) -- (292.9,210.59) ;



%Straight Lines [id:da9001962838605487] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (350.71,237.72) -- (319.79,222.69) ;
\draw [shift={(316.2,220.94)}, rotate = 385.90999999999997] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da4191474600649756] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (333.46,229.33) -- (298.94,212.56) ;



%Straight Lines [id:da5775276894536598] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (308.41,268.29) -- (298.62,235.34) ;
\draw [shift={(297.48,231.5)}, rotate = 433.44] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da12498606793231604] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (302.95,249.9) -- (292.01,213.11) ;



%Shape: Circle [id:dp45032523751151743] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (286.18,221) .. controls (280.93,218.25) and (278.9,211.75) .. (281.65,206.49) .. controls (284.41,201.23) and (290.91,199.2) .. (296.17,201.96) .. controls (301.42,204.72) and (303.45,211.21) .. (300.7,216.47) .. controls (297.94,221.73) and (291.44,223.76) .. (286.18,221) -- cycle ;
%Straight Lines [id:da5640519561262781] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (71.33,347.83) -- (109.9,268.28) ;
\draw [shift={(111.64,264.68)}, rotate = 475.87] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da42843158531235725] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (91.49,306.26) -- (131.8,223.11) ;



%Straight Lines [id:da3173768933400225] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (128.82,283.08) -- (132.53,248.9) ;
\draw [shift={(132.96,244.92)}, rotate = 456.18] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da5774372082399238] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (130.89,264) -- (135.02,225.84) ;



%Straight Lines [id:da3524474313532311] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (85.76,253.58) -- (113.47,233.24) ;
\draw [shift={(116.7,230.87)}, rotate = 503.71] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da48253821043119494] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (101.23,242.22) -- (132.17,219.51) ;





%Shape: Circle [id:dp161592333334187] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (124.48,215.15) .. controls (125.31,209.28) and (130.75,205.18) .. (136.63,206.02) .. controls (142.51,206.85) and (146.6,212.29) .. (145.77,218.17) .. controls (144.94,224.04) and (139.5,228.14) .. (133.62,227.3) .. controls (127.74,226.47) and (123.65,221.03) .. (124.48,215.15) -- cycle ;

%Straight Lines [id:da44891595477713475] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (274.85,265.13) -- (255.5,232) ;


%Straight Lines [id:da5317275851719263] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (284.53,281.7) -- (267.19,252.02) ;
\draw [shift={(265.18,248.56)}, rotate = 419.71000000000004] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;



%Straight Lines [id:da4495679345576372] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (247.83,289.79) -- (248.37,255.42) ;
\draw [shift={(248.43,251.42)}, rotate = 450.9] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=2.25]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

%Straight Lines [id:da2925419351824692] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (248.13,270.61) -- (248.74,232.23) ;



%Shape: Circle [id:dp36005890098485926] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (241.11,229.25) .. controls (238.16,224.09) and (239.94,217.52) .. (245.09,214.57) .. controls (250.24,211.62) and (256.81,213.41) .. (259.76,218.56) .. controls (262.71,223.71) and (260.93,230.28) .. (255.78,233.23) .. controls (250.63,236.18) and (244.06,234.4) .. (241.11,229.25) -- cycle ;

% Text Node
\draw (141,185.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (343,295.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (245,124.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (176,124.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (146,255.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (211,17.37) node [scale=1.2]  {$e$};
% Text Node
\draw (73,141.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (242.68,97.58) node [scale=1.2,rotate=-0.63]  {$1^{-1}$};
% Text Node
\draw (197,79.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (176.11,307.09) node [rotate=-269.19]  {$\cdots $};
% Text Node
\draw (27.41,160.88) node [rotate=-358.03]  {$\cdots $};
% Text Node
\draw (43.07,215.38) node [rotate=-144.72]  {$\cdots $};
% Text Node
\draw (146,136.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (95,188.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (167,268.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (212,250.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$4$};
% Text Node
\draw (231,190.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (195,192.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};
% Text Node
\draw (218.91,297.96) node [rotate=-239.14]  {$\cdots $};
% Text Node
\draw (95,225.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (125.45,293.33) node [rotate=-275.61]  {$\cdots $};
% Text Node
\draw (75.12,258.24) node [rotate=-322]  {$\cdots $};
% Text Node
\draw (80,296.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (63.4,356.54) node [rotate=-296.09]  {$\cdots $};
% Text Node
\draw (387.46,326.95) node [rotate=-229.85]  {$\cdots $};
% Text Node
\draw (283,166.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (309.21,279.88) node [rotate=-251.73]  {$\cdots $};
% Text Node
\draw (359.23,244.36) node [rotate=-205.34]  {$\cdots $};
% Text Node
\draw (290,241.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (245.11,301.09) node [rotate=-269.19]  {$\cdots $};
% Text Node
\draw (236,262.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$1$};
% Text Node
\draw (270,281.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$2$};
% Text Node
\draw (287.91,291.96) node [rotate=-239.14]  {$\cdots $};
% Text Node
\draw (334,205.37) node [scale=1.2,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$3$};


\end{tikzpicture}

}
\end{example}
\begin{example}(Prime Renewal Shift)\\

Take matrix $A$ as follows: for each $p$ prime number and  $n \in \mathbb{N}$ we have
\begin{equation*}
A(n+1,n)=A(1,n) = A(p,p^n) = 1
\end{equation*}
and zero for the other entries of $A$. From now on, we will call this shift \emph{Prime Renewal Shift}.

The transition matrix looks like:
\begin{equation*}
    A = \begin{pmatrix}
    1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \cdots\\
    1 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & \cdots\\
    0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 1 & \cdots\\
    0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & \cdots\\
    0 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 0 & 1 & 1 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 &\cdots\\
    \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \ddots
    \end{pmatrix}.
\end{equation*}
Consider the space of the columns of $A$ endowed with the product topology. By taking these vector columns we obtain the following limit points:
\begin{equation*}
    \mathfrak{c}(p) = \begin{pmatrix}
                        1\\
                        0\\
                        0\\
                        \vdots\\
                        0\\
                        1 \quad(p\text{-th coordinate})\\
                        0\\
                        \vdots
                      \end{pmatrix},
\end{equation*}
where $p$ is a prime number. That is, for every prime number $p$, the column vector $\mathfrak{c}(p)$ which assigns $1$ for the first and the $p$-th row and zero elsewhere is a limit point of the columns of $A$. Indeed, this can be shown by taking the sequence $\{\mathfrak{c}^n(p)\}_{n \in \mathbb{N}}$, where $\mathfrak{c}^n(p)$ is the $p^n$-th column of $A$. For every coordinate which is not $1$ or $p$ we have a finite number of $1$`s and therefore the row converges to zero. On the other hand, we have for all elements in the sequence that for both first and $p^n$-th row the column assigns always the value 1, proving the convergence. The unique remaining limit of this topological space is the same one of the renewal shift, by taking the sequence $\{\mathfrak{c}^n(n)\}_{n \text{ prime}}$, with similar proof as the one shown above. This limit is
\begin{equation*}
    \mathfrak{c} \equiv \mathfrak{c}(1) = \begin{pmatrix}
                        1\\
                        0\\
                        0\\
                        0\\
                        \vdots
                    \end{pmatrix}.
\end{equation*}

The prime renewal shift has a transition matrix with a full line of $1$`s in the first row and then $\mathcal{O}_A$ is unital as the renewal shift and therefore $X_A$ is compact.

We introduced in the renewal shift a family of infinite emitters in the graph associated to the matrix $A$ and now we present the consequences of such modification. Similarly to what we did for the renewal shift, we can take limits of elements from $\Sigma_A$ in order to obtain the elements of $Y_A$. We characterize these elements in the next proposition, in particular, we show the existence of infinitely many empty configurations on this space. By consequence, we will have infinitely many extremal conformal measures living on $Y_A$.

\begin{proposition}\label{varias_mesmo_tronco} Consider the prime renewal shift. The elements of $Y_A$ has as stems the finite words ending with $1$ or any prime number $p$, otherwise they have empty stem. Moreover,
\begin{itemize}
    \item[$(i)$] for each finite positive admissible word $\omega$ ending with a prime number $p$ there exists exactly one configuration in $Y_A$ which the stem is $\omega$;
    
    \item[$(ii)$] for each $k \in \{1\}\cup\{p \in \mathbb{N}:p\text{ is a prime number}\}$ and each $\omega$ positive admissible word ending with $1$ there exists exactly one configuration with stem $\omega$ and s.t. $\omega j^{-1}$ is filled only for $j \in \{1,k\}$;
    \item[$(iii)$] for each $k \in \{1\}\cup\{p \in \mathbb{N}:p\text{ is a prime number}\}$ there exists exactly one configuration with empty stem such that $j^{-1}$ is filled only for $j \in \{1,k\}$.
\end{itemize}
\end{proposition}

\begin{proof} We recall that the configurations of infinite stem are in bijection with the elements of $\Sigma_A$ and also with the set of infinite stems of any configuration of $X_A$. For any infinite emitter symbol, that is, for $a = 1$ or $a$ prime number $p$ we can take for any positive admissible word ending with $a$, $\omega'a$ (note that $\omega'$ can be empty), the sequence $\{\xi(n)\}_{n \in \mathbb{N}}$ in $\Sigma_A$ such that $\xi(n)_{\omega'aj_n} = 1$, where
\begin{equation*}
    j_n = \begin{cases}
            p^n, \quad \text{ if } a = p \text{ prime number};\\
            n , \quad \text{ if } a = 1.
          \end{cases}
\end{equation*}
Since $X_A$ is compact, there exists a convergent subsequence of $\{\xi(n)\}_{n \in \mathbb{N}}$ converging to $\xi \in X_A$. Then, necessarily we must have $\xi_{\omega'a} = 1$ and $\xi_{\omega'aj} = 0$ for every $j \in \mathbb{N}$, that is, $\kappa(\xi) = \omega'a$. On the other hand, if $a$ is not a infinite emitter, equation \eqref{eq:Omega_A_tau} implies that any convergent subsequence of $\{\xi(n)\}_{n \in \mathbb{N}}$ does not have stem $\omega'a$. The conclusion is: we necessarily have that the finite words ending with an infinite emitter and the empty word are the only possible words to be stem of some configuration in $Y_A$.

$Proof \ of \  (i):$ the existence can be proved by taking the sequence above for $\omega'aj_n = \omega j_n$ and then we use that $X_A$ is a compact set. The uniqueness follows by absurd: suppose that there exists at least two different configurations $\xi$ and $\eta$ in $Y_A$ such that $\kappa(\xi) = \kappa(\eta) = \omega \neq e$. Then there exists $\alpha$ and $\beta$ positive admissible words such that $g = \alpha \beta^{-1} \neq e$ is in the reduced form and satisfying $\xi_g \neq \eta_g$. Suppose without loss of generality that $\xi_g =1$, $\eta_g = 0$ and $\beta=j$ for some $j$. We must have that $\alpha = \omega$. Otherwise, $\alpha$ is a subword strictly smaller than $\omega$ and we have that $\xi_{\alpha} = \xi_{\alpha\omega_{|\alpha|}} = \eta_{\alpha\omega_{|\alpha|}}= \eta_{\alpha} = 1$. Therefore
\begin{equation*}
    \xi_{\alpha j^{-1}} = 1 \iff A(j,\omega_{|\alpha|}) \iff \eta_{\alpha j^{-1}} = 1.
\end{equation*}
Which is a contradiction with $\eta_g=0$.
  Due to corollary 7.7 of \cite{Exel}, $\xi \in Y_A$ if and only if $R_\xi(\omega)=R_\xi(\kappa(\eta))$ is a limit point of the columns of $A$ and the same is valid for $\eta$. Since every subword of $\omega$ is filled in $\xi$ and $\eta$ we have necessarily that $\omega_{|\omega|-1} \in R_\xi(\omega)$ and $\omega_{|\omega|-1} \in R_\eta(\omega)$. So, if $\omega$ ends with $p$ prime number, then $R_\xi(\omega) = R_\eta(\omega) = \{1,p\}$.

$Proof \ of \  (ii):$ the existence is obtained similarly as in $(i)$, we just describe the sequence $\{\xi^n\}_{\mathbb{N}}$ of elements of $\Sigma_A$ we take for each $p$ to converge to a configuration $\xi \in Y_A$ with $\kappa(\xi) = \omega$ and $\xi_{\omega j^{-1}} = 1$ for each $j \in \{1,p\}$. Here, $\xi^n$ is any element of $\Sigma_A$ such that $\xi^n_{\omega i_n} = 1$, where
\begin{equation*}
    i_n = \begin{cases}
            p^n, \quad \text{ if } p \text{ is a prime};\\
            n , \quad \text{ if } p = 1.
          \end{cases}
\end{equation*}
The proof of the uniqueness is the same of the previous case and so is item $(iii)$.\qed
\end{proof}
We denote by $\xi^0(p)$ the configuration with empty stem such that $\xi^0(p)_{1^{-1}}=\xi^0(p)_{p^{-1}}=1$, where $p$ is prime or one. It is straightforward to notice that, varying $p$ in the set of primes and the number one, the following sets form a partition of $Y_A$ in the prime renewal shift:
\begin{equation*}
    Y_A(\xi^0(p)) = \{\xi^0(p)\}\cup\{\xi \in Y_A: \kappa(\xi)_{|\kappa(\xi)|-1} \in \{1,p\} \text{ and } R_\xi(\kappa(\xi)) = \{1,p\}\}.
\end{equation*}

\begin{proposition}\label{prop:control_number_configurations} For the prime renewal shift we have that
\begin{equation*}
    2^{n-1}\leq |\{\xi \in Y_A(\xi^0(p)): |\kappa(\xi)|=n\}|\leq 3^n, \quad \forall n \in \mathbb{N},
\end{equation*}
for every $p \in \{1\}\cup\{p \in \mathbb{N}: p \text{ is a prime number}\}$.
\end{proposition}

\begin{proof} Given $j \in \mathbb{N}$, let us estimate $|\{i \in \mathbb{N}:A(i,j) = 1\}|$. We have two possibilities:
\begin{enumerate}
    \item $j = p^m$, with $m \in \mathbb{N}$ and $p$ prime number, and in this case $A(i,j) = 1$ if and only if $i = p^m+1$, $i = p$ or $i = 1$;
    \item Otherwise, $A(i,j) = 1$ if and only if $i = j+1$ or $i = 1$.
\end{enumerate}
If $p = 1$, then there exists only one $\xi$ in $Y_A(\xi^0(1))$ such that $|\kappa(\xi)| = 1$. Hence, by the possibilities shown above, we have
\begin{equation*}
    2^{n-1}\leq|\sigma^{-n}(\xi^0(1))| \leq 3^{n-1}, \quad \forall n \in \mathbb{N}.
\end{equation*}
For $p$ prime number, we have a similar calculation but with the difference that there exist exactly two different $\xi$ in $Y_A(\xi^0(p))$ such that $|\kappa(\xi)| = 1$, therefore $
    2^{n}\leq|\sigma^{-n}(\xi^0(p))| \leq 3^{n}, \ \forall  n \in \mathbb{N}$.

Then
\begin{equation*}
    2^{n-1}\leq |\{\xi \in Y_A(\xi^0(p)): |\kappa(\xi)|=n\}|\leq 3^n, \quad \forall n \in \mathbb{N},
\end{equation*}
for every $p \in \{1\}\cup\{p \in \mathbb{N}: p \text{ is a prime number}\}$.\qed
\end{proof}

Now we study the conformal measures on the prime renewal shift. We will see that the existence of infinitely many empty configurations implies the existence of infinite conformal measures living on $Y_A$. First, we characterize the conformal measures living on $Y_A$ as we made in the case of the standard renewal shift. Take $p \in \{1\}\cup\{p \in \mathbb{N}: p \text{ is a prime number}\}$, then define:
\begin{equation}\label{eq:coefficients_Y_A_confomal_prime_renewal_shift}
    c_{\omega,p}:= \mu(\{\xi(\omega,p)\}),
\end{equation}
where $\xi(\omega,p)$ is the configuration in $Y_A$ such that $\kappa(\xi(\omega,p)) = \omega$ and $R_{\xi(\omega,p)}(\omega) = \{1,p\}$, in this case $\omega$ ends with $1$ or $p$ prime. When $\omega$ ends with $p$ prime we have only one configuration which has stem $\omega$ and, when $\omega$ ends with $1$, we have a countable number of configurations with the same stem $\omega$, see proposition \ref{varias_mesmo_tronco}. Consider a potential $F:U \to \mathbb{R}$, where $U$ is the open set of elements for which we can apply the shift map, in $Y_A$ we use the following notation $F(\omega,p):=F(\xi(\omega,p))$, $p$ prime or one. As in the case of the standard renewal shift, we define:
\begin{equation*}
    D(\omega,p) = e^{F(\omega,p)}.
\end{equation*}
Now, we have the analogous result to the theorem \ref{theorem.coeficientes}, the proof is the same.

\begin{proposition}\label{theorem:coeficientes_prime_renewal_shift} A measure $\mu$ which vanishes on $\Sigma_A$ satisfies the Denker-Urba\'nski conformality condition if and only if for every $p \in \{1\}\cup\{p \in \mathbb{N}: p \text{ is a prime number}\}$ such that the coefficients $c_{\omega,p}$ in \eqref{eq:coefficients_Y_A_confomal_prime_renewal_shift} satisfy
\begin{equation*}
    c_{\omega,p} D(\omega,p) = c_{\sigma(\omega),p},
\end{equation*}
for $|\omega|>0$.
\end{proposition}

Now, observe that the identity $c_{\omega,p} D(\omega,p) = c_{\sigma(\omega),p}$ leads to
\begin{equation}\label{eq:c_omega_new_prime_renewal_shift}
c_{\omega,p} e^{(S_{|\omega|}F)(\omega,p)} = c_{e,p}, \quad \forall \  \xi(\omega,p) \in Y_A(\xi^0(p))\setminus\{\xi^0(p)\},
\end{equation}
for every $p \in \{1\}\cup\{p \in \mathbb{N}: p \text{ is a prime number}\}$.
In order to construct $e^F$-conformal probability measures living on $Y_A$ we must keep $c_{e,p} > 0$, for a $p$, otherwise all other $c_{\omega,p}$'s are zero by \eqref{eq:c_omega_new_prime_renewal_shift}. This is equivalent to impose $c_{\omega,p} > 0$ for all $\xi(\omega,p) \in Y_A(\xi^0(p))$. We will impose, as well, the condition
\begin{equation}\label{eq:c_omega_probability_PRS}
    \sum_{\xi(\omega,p) \in Y_A(\xi^0(p))}c_{\omega,p} = 1,
\end{equation}
for a $p \in \{1\}\cup\{p \in \mathbb{N}: p \text{ is a prime number}\}$, to guarantee that the measure which vanishes out of $Y_A(\xi^0(p))$ is a probability.

Now, we have an analogous result to the theorem \ref{theorem.potentialwithonecoordinate} for the case of countably infinite empty configurations.

\begin{theorem}\label{theorem:infinite_conformal_measures} Consider potentials $F:U \to \mathbb{R}$, we have the following:
\begin{itemize}
    \item[(i)] Suppose $\inf F>0$. For each $p \in \{1\}\cup\{p \in \mathbb{N}: p \text{ is a prime number}\}$ and $\beta>\frac{\log 3}{\inf F}$, there exists a unique $e^{\beta F}$-conformal probability measure $\mu_{\beta,p}$ that vanishes out of $Y_A(\xi^0(p))$.
    \item[(ii)] Suppose $0\leq \sup F < + \infty$ and $\beta\leq \frac{\log 2}{\sup F}$, there are no $e^{\beta F}$-conformal probability measures which vanish in $\Sigma_A$.
\end{itemize}
\end{theorem}

\begin{corollary}
Let $F\equiv 1$. Then, the result follows:

\begin{itemize}
    \item[(i)] For $\beta>\log(3)$ , all $e^{\beta}$-conformal probability measures $\mu_\beta$ that vanishes on $\Sigma_A$ can be written as a convex combination of the measures $\mu_{\beta,p}$.
    \item[(ii)] For $\beta\leq \log(2)$ there is no $e^\beta$- conformal probability measure that vanishes on $\Sigma_A$.
\end{itemize}
\end{corollary}
\begin{proof}
Apply theorem \ref{theorem:infinite_conformal_measures} for the constant potential $F\equiv 1$. For $\beta>\log(3)$, if $\mu_\beta$ is a $e^{\beta}$-conformal measure that vanishes on $\Sigma_A$, denote
$$J=\left\{p\in \{1\}\cup \{p\in \mathbb{N}: p \text{ is prime}\}: \mu_\beta(Y_A(\xi^0(p)))\neq 0\right\}$$
and we have for $E\subseteq Y_A$,
$$\mu_\beta(E)=\sum_{p\in J}\mu_\beta(E\cap Y_A(\xi^0(p)))=\sum_{p\in J}\mu_\beta(Y_A(\xi^0(p)))\dfrac{\mu_\beta(E\cap Y_A(\xi^0(p)))}{\mu_\beta(Y_A(\xi^0(p)))}=\sum_{p\in J}\mu_\beta(Y_A(\xi^0(p)))\mu_{\beta,p}(E).$$
Observe as well that $\mu_{\beta,p}$ are extremal measures.
For $\beta\leq \log(2)$ is a direct consequence of the previous theorem.
\qed
\end{proof}

We finish this section with an example of a matrix $A$ generating an unital Exel-Laca algebra $\mathcal{O}_A$ which has no lines of $1's$, in contrast with the others matrices above.
\end{example}
\begin{example}(Transition Matrix without full line of 1's)\\

Consider the matrix $A$ defined by the entries
\begin{equation*}
    A(1,2n) = A(2,2n-1) = A(n+1,n) = 1, \quad \text{ for all } n \in \mathbb{N},
\end{equation*}
and zero for the remaining entries. The matrix $A$ is the following:
\begin{equation*}
    A = \begin{pmatrix}
    0 & 1 & 0 & 1 & 0 & 1 & 0 & \cdots\\
    1 & 0 & 1 & 0 & 1 & 0 & 1 & \cdots\\
    0 & 1 & 0 & 0 & 0 & 0 & 0 & \cdots\\
    0 & 0 & 1 & 0 & 0 & 0 & 0 & \cdots\\
    0 & 0 & 0 & 1 & 0 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 1 & 0 & 0 &\cdots\\
    0 & 0 & 0 & 0 & 0 & 1 & 0 &\cdots\\
    \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \ddots
    \end{pmatrix}.
\end{equation*}
Although $A$ has not a full line of 1's, the corresponding Exel-Laca algebra is unital. 

Indeed, we have that $Q_1 + Q_2 = 1$, and therefore
\begin{equation*}
    1 \in \overline{\spann\left\{ \begin{array}{l l}
         & F \text{ finite}; \text{ }\alpha, \beta \text{ finite admissible words};\\
         T_\alpha \left(\prod_{i \in F}Q_i\right)T_\beta^*: &F \neq \emptyset \text{ or } \alpha \text{ is not the empty word} \\
         &\text{or }  \beta \text{ is not an empty word}
    \end{array}\right\} } \simeq \mathcal{O}_A,
\end{equation*}
that is, $\mathcal{O}_A$ is unital, and hence $X_A$ is compact. The graph associated to the matrix $A$ has 2 infinite emitters and therefore $\Sigma_A$ is not locally compact.  The only two possibilities for limit point on the space of columns of $A$ are
\begin{equation*}
    c_1 = \begin{pmatrix} 1 \\ 0 \\0 \\ 0 \\ 0 \\\vdots \end{pmatrix} \quad \text{and} \quad c_2 = \begin{pmatrix} 0 \\ 1 \\0 \\ 0 \\ 0 \\\vdots \end{pmatrix}.
\end{equation*}
By taking limits, the only possibilities for finite stems are:
\begin{enumerate}
    \item words ending with 1 (unique configuration associated);
    \item words ending with 2 (unique configuration associated);
    \item empty word (two configurations associated).
\end{enumerate}
The configurations are obtained similarly to the other examples.
\end{example} 








\section{Pressures}

Our main goal in this section is to present the concept of pressure at a point $x \in X_A$ and compare it with the Gurevich pressure defined on the setting of countable Markov shifts. For the pressure of a potential $F:U\to \mathbb{R}$ at a point $x$, denoted by $P(F,x)$, we follow \cite{DenYu}. This concept is introduced on a more general setting, called an \textit{Iterated Function System}, i.e a pair consisting of a Polish Space $X$ and a family $\mathcal{V}$ of homeomorphisms $v:D(v)\to v(D(v))\subset X$ defined on a closed nonempty subset $D(v)\subset X$. The authors require as well the existence of point which the orbit is infinite, but since our goal is to apply the theorems on the generalized symbolic space $X_A$, which contains $\Sigma_A$, this hypothesis is automatically satisfied.

For us, the polish space $X$ is the space $X_A$ and the family of homeomorphisms are chosen to be $\{(\sigma\restriction_{C_i})^{-1}: i\in \mathbb{N}\}$, the inverses of the shift map when restricted to the \textit{generalized  cylinder sets} $C_i := \{\xi \in X_A: \xi_i =1\}$. 

The Gurevich pressure is defined in \cite{Sa,Sa2,Sa4,Sa5}. In order to present them we define for any finite admissible word $\alpha$, $|\alpha| \leq n$, and $n \in \mathbb{N}$ the set $W_n^\alpha$ of the words of length $n$ which ends with $\alpha$.






As a subclass of examples, $F$ satisfies the hypothesis of the corollary \ref{cor:equal_pressures} if we take $g$ as being an increasing function. In particular, we are interested in the case $g(x) = \log x$ because in this case $F$ is transient for $\beta > \beta_c$, $\beta_c \in (1,2)$, and it is positive recurrent for $\beta < \beta_c$.




\section{Length-Type Phase Transitions}

 By a Buzzi-Sarig theorem in \cite{BS}, if we look for the set of equilibrium measures associated to a summable variations potential $\beta F$ defined on  $\Sigma_A$, the only options are the absence or the existence of an unique equilibrium measure for $\beta F$ for each $\beta$. In other words, the \textit{phase transition} is in the sense of the existence or not of the equilibrium state. In addition, when the equilibrium state $\mu_{\beta}$ does exist, $\mu_{\beta} = h_{\beta} d\nu_{\beta}$ where $h_{\beta}$ and $\nu_{\beta}$ are a eigenfunction associated to $L_{\beta F}$ and a eigenmeasure associated to $L^{*}_{\beta F}$, respectively. Both with to the eigenvalue $\lambda_\beta= e^{P_G(\beta F)}$.
 
 Since $\Sigma_A \subseteq X_A$ and, in many cases $X_A$ is compact, it is very natural to expect to find more eigenmeasures (they are constructed via subsequences of atomic measures) for the Ruelle transformation on $X_A$ than in the standard symbolic space $\Sigma_A$. 
 
 In this section, we will study the possibility of phase transitions on the set of the eigenmeasures $\nu_{\beta}$ when we vary the parameter $\beta$. We will exhibit a concrete example of a potential $F:U \to \mathbb{R}$ such that its restriction to the classical symbolic space presents a phase transition respect to the existence of the eigenmeasure which disappears when we consider the same potential defined on $U\subseteq X_A$.






\subsection{Existence of eigenmeasures}\\



In this section we shall give a fairly general condition on a potential $F:U\to \mathbb{R}$ for the existence of an eigenmeasure $m$ with eigenvalue $\lambda>0$ for the Ruelle transformation $L_F$, in other words,
\[\int f dm= \int L_{-(\log \lambda-F)} f dm \quad  \text{for every $f\in C_c(U)$},\]
by theorem \ref{theorem.princial.1}, $m$ is a $e^{\log\lambda-F}$-conformal measure. Our result for existence is direct consequence of theorem 3.6 on \cite{DenYu}, but due to some differences on notation and some changes on the statement of the theorem, we will be providing a proof below. 



\vspace{.3cm}\noindent

\subsection{Different thermodynamics for the same potential.\newline
Standard versus generalized symbolic spaces: a concrete example}\\


On this section we give an explicit example to illustrate the differences which can be found when we use the standard countable Markov shift $\Sigma_A$ and the generalized one $X_A$ as the configuration space for a fixed potential.

\begin{theorem}
Consider the potential $F:U \rightarrow \mathbb{R}$ given by  $F(x)=\log(x_0)-\log(x_0+1)$, defined on $U \subset X_A$, where $A$ is the matrix of the renewal shift. Then,
\begin{itemize}
    \item[(i)] For each $\beta >0$ there exists a probability eigenmeasure associated to the eigenvalue $e^{P_G(\beta F)}$ for the potential $\beta F$.
    \item[(ii)] When we consider the restrictions of the potential $F|_{\Sigma_A}$ and of the shift map $\sigma|_{\Sigma_A}$, there exists a critical $\beta_c$, with $\beta_c \in (1,2)$, such that:\\
    
   (ii)$_1$ For $0<\beta<\beta_c$ there exists an unique     conservative probability eigenmeasure \indent living on $\Sigma_A$ associated to the eigenvalue $e^{P_G(\beta F)}$.\\
    
    (ii)$_2$ For $\beta > \beta_c$ there is no conservative probability eigenmeasure living on $\Sigma_A$.\\
    
\end{itemize}
\end{theorem}

\begin{proof} The item (i) is a direct consequence of the theorem \ref{theorem.existence_of_eigen}. In fact, since $\log$ is a increasing function we have that $F$ is bounded above and $P(\beta F, x)=P_G(\beta F) <+\infty$ for every $x \in X_A.$ Now, using the theorem \ref{theorem.existence_of_eigen}, we have the existence of a measure $m_\beta$ such that $L_{\beta F}^*m_\beta=e^{P_G(\beta F)} m_\beta$ for every $\beta > 0$.

\end{proof}



\begin{remark}
The existence of eigenmeasures living on $\Sigma_A$ for transient potentials like in the previous example already was obtained in the standard thermodynamic formalism for countable Markov shifts by Van Cyr \cite{Cyr}, see also \cite{Sw}, assuming that $\Sigma_A$ is locally compact. We don't know if the eigenmeasure above lives on $\Sigma_A$, maybe the measure gives mass to the set $Y_A$. If the eigenmeasure of the example lives on $\Sigma_A$ for some $\beta$ such that $\beta F$ is transient, this would be an example of the existence of an eigenmensaure (not conservative) where we do not assume that $\Sigma_A$ is locally compact as in \cite{Cyr, Sw}.
\end{remark}


\section{Convergence of probability measures on $X_A$}\label{convergence}


When you are developing the thermodynamic formalism in some setting, one of the first facts which you need to know is how to control the weak convergence of probability measures over the configuration space (symbolic space). In the standard case of countable Markov shifts $\Sigma_A$ it is well known that a sequence of probability measures $(\mu_n)_{n \in \mathbb{N}}$ converges in the weak$^*$ topology (weak topology for the probabilists) to a probability measure $\mu$ when, for each cylinder set $[x_0, x_1,..., x_{m-1}]$, we have $\lim_{n \rightarrow \infty} \mu_{n}([x_0, x_1,..., x_{m-1}]) = \mu([x_0, x_1,..., x_{m-1}])$.

In fact, this is a particular case of a general theorem in probability theory which says that a net of Borel probability measures $(\mu_\lambda)_{\lambda \in \Lambda}$ on a metric space converges to a Borel probability measure $\mu$ if, and only if, for some basis of the topology $\mathcal{U}$ closed by finite intersections, we have $\lim_{\lambda \in \Lambda} \mu_\lambda(O) = \mu(O)$ for every $O \in \mathcal{U}$. For a reference of such result, see theorem 8.2.17 of \cite{Bogachev2007}.


Based on such result, we should find a topological basis which is useful to perform the use of the aforementioned theorem and then to connect the classical theory of countable Markov shifts with our generalized Markov shifts. First, we characterize the topological basis for a general $X_A$. After that, the general case is applied for the Renewal shift, giving us a simple characterization of a suitable basis for the hypotheses of the theorem 8.2.17 of \cite{Bogachev2007} and then, by this result, we prove that the conformal measures living in $Y_A$ for this particular case converges to the conformal measure of the classical theory for $\beta$ decreasing to its critical value $\beta_c = \log 2$.

We recall that the topology on $X_A$ is the subspace topology of the product topology on $\{0,1\}^\mathbb{F}$. In other words: the topology of $X_A$ is generated by the family of basic clopen sets $\{\pi_\omega^{-1}(B)\cap X_A: \omega \in \mathbb{F}, B \subseteq \{0,1\}\}$. It is straightforward to notice that the topology of $X_A$ is second countable. Consider the \textit{generalized cylinder sets} defined by $C_\omega = \{\xi \in X_A: \xi_\omega =1\}$, where $\omega \in \mathbb{F}$. We have that
\begin{equation*}
    \pi_\omega^{-1}(B)\cap X_A = \begin{cases}
                                    \emptyset, \quad \text{if }B = \emptyset, \\
                                    C_\omega, \quad \text{if }B = \{1\}, \\
                                    C_\omega^c, \quad \text{if }B = \{0\}, \\
                                    X_A, \quad \text{if }B = \{0,1\}.
                                 \end{cases}
\end{equation*}
If we consider the topological basis $\mathcal{B}$ of the finite intersections of the elements of the family $$\{C_g:g=\alpha \gamma^{-1}\}\cup\{C_g^c:g=\alpha \gamma^{-1}\}$$, then we already have a topological basis under the hypotheses of the theorem 8.2.17 of \cite{Bogachev2007}. However, many of the elements of $\mathcal{B}$ are redundant and we do not need to test the convergence for every $C_g$, $g \in \mathbb{F}$, as well as the are not needed to be part of the basis. Indeed, since for every $g \in \mathbb{F}$ which is not in the reduced form $\alpha \gamma^{-1}$ for all $\alpha, \gamma$ finite positive admissible words, we have that $\xi_g = 0$ for all $\xi \in X_A$, then $\pi_g^{-1}(B) \in \{\emptyset,X_A\}$ and such terms may be excluded of the basis without changes in the topology. In addition, we can simplify the basis even further by the following results. The main idea is to simplify the topological basis and prove the convergence of the measures on it. In the classical case, the convergence of measures on cylinders is sufficient to grant the weak$^*$ convergence and the same idea will be used here.


\begin{proposition}\label{prop:cylinder_reducing_inverse} For any $\alpha, \gamma$ positive admissible words with $\gamma= \gamma_0 \cdots \gamma_{|\gamma|-1}$, $|\gamma|>1$, we have that $C_{\alpha \gamma^{-1}}=C_{\alpha \gamma_{|\gamma|-1}^{-1}}$.
\end{proposition}

\begin{proof} The inclusion $C_{\alpha \gamma^{-1}}\subseteq C_{\alpha \gamma_{|\gamma|-1}^{-1}}$ is obvious from the convexity property and the fact that $\xi_e = 1$ for all configurations in $X_A$ give us the equivalence
\begin{equation} \label{eq:equiv_convex}
    \xi_\omega = 1 \iff \xi_\nu = 1, \forall \nu \in \llbracket \omega \rrbracket,
\end{equation}
which is valid for the particular case when $\xi \in C_{\alpha\gamma^{-1}}$ $\omega = \alpha \gamma^{-1}$ with $\nu = \alpha \gamma_{|\gamma|-1}^{-1}$. For the opposite inclusion, we recall that for any configuration $\xi \in X_A$ the following holds: if $\omega \in \mathbb{F}$ and $y \in \mathbb{N}$ satisfy $\xi_{\omega} = \xi_{\omega y}=1$, then for any $x \in \mathbb{N}$
\begin{equation}\label{eq:equiv_past_filled}
    \xi_{\omega x^{-1}} = 1 \iff A(x,y) = 1.
\end{equation}
In particular, we may apply the equivalence above for $\xi \in C_{\alpha \gamma_{|\gamma|-1}^{-1}}$, $\omega = \alpha \gamma_{|\gamma|-1}^{-1}$, $y = \gamma_{|\gamma|-1}$ and $x = \gamma_{|\gamma|-2}$. The rest of the proof follows by repeating the process for $\omega = \alpha (\gamma_{p} \cdots \gamma_{|\gamma|-1})^{-1}$, $y = \gamma_{p}$ and $x = \gamma_{p-1}$ for $p \in \{1,..., \gamma_{|\gamma|-2}\}$.\qed
\end{proof}

In order to proceed with more simplifications of the basis, we define the following. For given positive admissible words $\alpha$ and $\gamma$ we define the finite sets $F_\alpha := \{\xi \in Y_A: \kappa(\xi) \in  \llbracket \alpha \rrbracket\setminus\{\alpha\}\}$, $F_\alpha^* := \{\xi \in Y_A: \kappa(\xi) \in  \llbracket \alpha \rrbracket\}$ and $F_\gamma^\alpha := \{\xi \in F_\gamma: \alpha \in \llbracket \kappa(\xi) \rrbracket\}$. Note that $F_\gamma^\gamma = \emptyset$ and that $F_\gamma^\alpha = \emptyset$ if $\alpha \notin \llbracket\gamma\rrbracket$. Also, define for any $H,I \subseteq \mathbb{N}$ the sets $G(\alpha,H):=\{\xi \in X_A: \kappa(\xi)=\alpha, \xi_{\alpha j^{-1}}=1, \forall j \in H\}$, with $G(\alpha,j):=G(\alpha,\{j\})$, for $j \in \mathbb{N}$; $K(\alpha,H):=\{\xi \in X_A: \kappa(\xi)=\alpha, \xi_{\alpha j^{-1}}=0, \forall j \in H\}$, with $K(\alpha,j):= K(\alpha,\{j\})$, for $j \in \mathbb{N}$; and $GK(\alpha,H,I):= G(\alpha,H) \cap H(\alpha,I)$, with $GK(\alpha,j,k) := GK(\alpha,\{j\},\{k\})$, for $j,k \in \mathbb{N}$. Finally, for $m \in \{0,1,..., |\alpha|-1\}$, define the words $\delta^0(\alpha) = e$ and $\delta^m(\alpha) = \alpha_0 \cdots \alpha_{m-1}$, for $m \neq 0$. 

\begin{proposition}\label{prop:general_C_alpha_inverse_j} For every $\alpha$ positive admissible word and for every $j \in \mathbb{N}$ s.t. $j \neq \alpha_{|\alpha|-1}$ we have that
\begin{equation*}
    C_{\alpha j^{-1}} = G(\alpha,j)\sqcup \bigsqcup_{k:A(j,k)=1}C_{\alpha k}.
\end{equation*}
\end{proposition}

\begin{proof} The inclusion
\begin{equation*}
    C_{\alpha j^{-1}} \supseteq G(\alpha,j)\sqcup \bigsqcup_{k:A(j,k)=1}C_{\alpha k}
\end{equation*}
is straightforward. For the opposite inclusion, let $\xi \in C_{\alpha j^{-1}}$. If $\kappa(\xi)= \alpha$, then $\xi \in G(\alpha,j)$. Suppose then $\kappa(\xi)\neq \alpha$. By convexity and $\xi_e=1$ we get $\alpha \in \llbracket\kappa(\xi)\rrbracket\setminus\{\kappa(\xi)\}$, and hence $\alpha k \in \llbracket\kappa(\xi)\rrbracket$ for some $k \in \mathbb{N}$. Since $\xi_{\alpha j^{-1}}=1$, we have necessarily that $A(j,k)=1$. \qed
\end{proof}
\begin{remark} On the notations of the proposition above, it is straightforward to notice that
\begin{equation*}
    G(\alpha,j) = \overline{\bigsqcup_{k:A(j,k)=1}C_{\alpha k}}\mathbin{\Big\backslash}\left\{\bigsqcup_{k:A(j,k)=1}C_{\alpha k}\right\} = \partial\left(\bigsqcup_{k:A(j,k)=1}C_{\alpha k}\right),
\end{equation*}
in other words,
\begin{equation*}
    C_{\alpha j^{-1}} = \overline{\bigsqcup_{k:A(j,k)=1}C_{\alpha k}}. 
\end{equation*}
\end{remark}

\begin{proposition}\label{prop:general_C_alpha_complement} Let $\alpha$ be a non-empty positive admissible word. Then,
\begin{equation*}
    C_\alpha^c = F_\alpha\sqcup\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} C_{\delta^m(\alpha)k}.
\end{equation*}
\end{proposition}
\begin{proof} The inclusion 
\begin{equation*}
    C_\alpha^c \supseteq F_\alpha\sqcup\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} C_{\delta^m(\alpha)k}
\end{equation*}
is straightforward. Let $\xi \in C_\alpha^c$. If $\kappa(\xi) \in \llbracket \alpha \rrbracket$ then we necessarily have that $\xi \in F_\alpha$. Suppose that $\kappa(\xi) \notin \llbracket \alpha \rrbracket$. Then there exists $m \in \{0,...,|\alpha|-1\}$ and $k \in \mathbb{N}\setminus\{\alpha_m\}$ such that $\delta^m(\alpha)k \in \llbracket\kappa(\xi)\rrbracket$ and therefore $\xi \in C_{\delta^m(\alpha)k}$. \qed
\end{proof}

\begin{proposition}\label{prop:general_C_alpha_j_inverse_complement} Let $\alpha$ be a non-empty positive admissible word and $j \neq \alpha_{|\alpha|-1}$. Then,
\begin{equation*}
    C_{\alpha j^{-1}}^c = K(\alpha,j) \sqcup F_\alpha \sqcup \left( \bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{p\neq \alpha_m}  C_{\delta^m(\alpha )p}\right)\sqcup \bigsqcup_{\substack{p: A(j,p)=0}}  C_{\alpha p}.
\end{equation*}
\end{proposition}
\begin{proof} By the propositions \ref{prop:general_C_alpha_inverse_j} and \ref{prop:general_C_alpha_complement} we obtain
\begin{align*}
    C_{\alpha j^{-1}}^c =  \bigcap_{k:A(j,k)=1} \left(\left(G(\alpha,j)^c\cap F_{\alpha k}\right)\sqcup\bigsqcup_{m=0}^{|\alpha|}\bigsqcup_{p\neq (\alpha k)_m} G(\alpha,j)^c\cap C_{\delta^m(\alpha k)p}\right).
\end{align*}
In order to characterize the sets $G(\alpha,j)^c\cap F_{\alpha k}$ we use the following identity,
\begin{align*}
    G(\alpha,j)^c &= \Sigma_A \sqcup G_1\sqcup G_2 \sqcup K(\alpha,j),\text{ where  }G_1 = C_\alpha^c \cap Y_A \quad \text{and}\\
    G_2 &= \left\{\xi \in Y_A:\alpha \in \llbracket\kappa(\xi)\rrbracket\setminus\{\kappa(\xi)\}\right\}.
\end{align*}
It is straightforward to verify that
\begin{equation*}
    F_{\alpha k} \cap \Sigma_A = F_{\alpha k} \cap G_2 = \emptyset, \quad  F_{\alpha k} \cap G_1 = F_\alpha, \quad F_{\alpha k} \cap K(\alpha,j) = K(\alpha,j).
\end{equation*}
Now we use the decomposition
\begin{equation*}
    G(\alpha,j)^c = G_3\sqcup K(\alpha,j),\text{ where  }  G_3 =\left\{\xi \in X_A:\kappa(\xi) \neq \alpha \right\},
\end{equation*}
in order to obtain for $m \in \{0,...,|\alpha|\}$ and $p \neq (\alpha k)_m$ the identities
\begin{equation*}
    C_{\delta^m(\alpha k)p}\cap G_3 = C_{\delta^m(\alpha k)p} \quad \text{and} \quad C_{\delta^m(\alpha k)p}\cap K(\alpha,j) = \emptyset.
\end{equation*}
Thus we have \vspace{-3mm}
\begin{align*}
    C_{\alpha j^{-1}}^c &= K(\alpha,j) \sqcup F_\alpha \sqcup \bigcap_{k:A(j,k)=1}\left( \bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{p\neq \alpha_m}  C_{\delta^m(\alpha )p}\right)\sqcup \bigcap_{k:A(j,k)=1}\bigsqcup_{p\neq k}  C_{\alpha p}\\
    &= K(\alpha,j) \sqcup F_\alpha \sqcup \left( \bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{p\neq \alpha_m}  C_{\delta^m(\alpha )p}\right)\sqcup \bigsqcup_{\substack{p: A(j,p)=0}}  C_{\alpha p}.
\end{align*} \qed
\end{proof}

\begin{remark} The propositions \ref{prop:general_C_alpha_inverse_j} and \ref{prop:general_C_alpha_j_inverse_complement} are also valid for $\alpha = e$, removing the hypothesis $j \neq \alpha_{|\alpha|-1}$. The proof is the same as presented above.
\end{remark}

We moved some auxiliary lemmas to the appendix to avoid technicalities. The lemmas are used to prove the next theorem and identities involving intersections of generalized cylinders, the most obvious is the following:
\begin{equation}\label{eq:C_cap_C}
    C_\alpha \cap C_\gamma = \begin{cases}
                                C_\alpha, \quad \text{if } \gamma \in \llbracket \alpha \rrbracket,\\
                                C_\gamma, \quad \text{if } \alpha \in \llbracket \gamma \rrbracket,\\
                                \emptyset, \quad \text{otherwise};
                            \end{cases} 
\end{equation}
which holds for every $\alpha$ and $\gamma$ positive admissible words.

Summarizing the results, the proposition \ref{prop:cylinder_reducing_inverse} grants that we only need to consider the basis of the finite intersections of generalized cylinders in the form $C_\alpha$ and $C_{\alpha j^{-1}}$, $\alpha$ positive admissible word and $j \in \mathbb{N}$, and their complements. However the propositions \ref{prop:general_C_alpha_inverse_j}, \ref{prop:general_C_alpha_complement} and \ref{prop:general_C_alpha_j_inverse_complement} show that $C_{\alpha j^{-1}}$ as much as $C_\alpha$ and $C_{\alpha j^{-1}}$ can be written as a disjoint union of generalized cylinders disjointly united with a subset of $Y_A$. It is noticeable that for any finite intersection of these elements we obtain again a disjoint union between a subset of $Y_A$ and a disjoint union of cylinders. It is important to emphasize that all these open sets are actually clopen sets, and then any limit of a net of measures calculated on these elements of the topology can be performed by calculating the limit in the explicit formula of the measure.

In the particular case of the renewal shift, we have a more simple characterization which is consequent from the general case and which we present now.

\begin{lemma}\label{lemma:G_K_renewal}
For the renewal shift we have
\begin{equation*}
    G(\alpha,F) = \begin{cases}
        \{\alpha \xi^0\}, \quad \alpha_{|\alpha| - 1} = 1 \text{ and } F = \{1\},\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
and
\begin{equation*}
    K(\alpha,F) = \begin{cases}
        \{\alpha \xi^0\}, \quad \alpha_{|\alpha| - 1} = 1 \text{ and } F \neq \{1\},\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
for $\alpha$ non-empty finite admissible word.
\end{lemma}

\begin{proof} From the renewal shift we have that there exists $\xi \in Y_A$ such that $\kappa(\xi) = \alpha$, that is, $\xi = \alpha \xi^0$, if and only if $\alpha_{|\alpha|-1} = 1$. We complete the proof by recalling that $R_{\alpha\xi^0}(\alpha) = \{1\}$ for $\alpha$ ending with $1$.
\end{proof}

\begin{remark} The lemma above is also valid for $\alpha = e$, just by removing the condition $\alpha_{|\alpha| - 1} = 1$.
\end{remark}

\begin{corollary}\label{cor:C_alpha_j_inv_renewal} Consider the set $X_A$ of the renewal Markov shift. For any $\alpha$ positive admissible word, $|\alpha|\neq 0$, and any $j \in \mathbb{N}$, we have that $C_{\alpha j^{-1}}$ is the empty set or $C_{\alpha j^{-1}} = C_\gamma$, where $\gamma$ is a positive admissible word.
\end{corollary}

\begin{proof} If $j = \alpha_{|\alpha|-1}$ then the statement is obvious. So consider $j \neq \alpha_{|\alpha|-1}$. By the lemma \ref{lemma:G_K_renewal} we have $G(\alpha,F) = \emptyset$. Also,
\begin{equation*}
    \bigsqcup_{k:A(j,k)=1} C_{\alpha k} = \begin{cases}
        C_{\alpha (\alpha_{|\alpha|-1} -1)}, \quad \alpha_{|\alpha|-1} > 1 \text{ and } j = 1,\\
        C_{\alpha (j-1)}, \quad \alpha_{|\alpha|-1} = 1,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
and therefore, by the proposition \ref{prop:general_C_alpha_inverse_j} we conclude that
\begin{equation*}
    C_{\alpha j^{-1}} = \begin{cases}
        C_{\alpha (\alpha_{|\alpha|-1} -1)}, \quad \alpha_{|\alpha|-1} > 1 \text{ and } j = 1,\\
        C_{\alpha (j-1)}, \quad \alpha_{|\alpha|-1} = 1,\\
        \emptyset, \quad \text{otherwise}.
    \end{cases}
\end{equation*}\qed
\end{proof}
\begin{remark} If $\alpha = e$, then
\begin{equation*}
    C_{j^{-1}} = \begin{cases}
        X_A, \quad j = 1,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
which is straightforward from the renewal shift.
\end{remark}

\begin{remark} In the renewal shift, for given positive admissible words $\alpha$ and $\gamma$, and for any $H \subseteq \mathbb{N}$ we have that
\begin{align*}
    F_\alpha &= \{\eta \xi^0 \in Y_A: \eta_{|\eta|-1|} = 1, \eta \in \llbracket \alpha \rrbracket \setminus \{\alpha\}\}, \quad F_\alpha^* = \{\eta \xi^0 \in Y_A: \eta_{|\eta|-1|} = 1, \eta \in \llbracket \alpha \rrbracket\},\\
    F_\gamma^\alpha &= \{\eta \xi^0 \in F_\gamma: \alpha \in \llbracket \eta \rrbracket\},
\end{align*}
both finite sets.
\end{remark}

\begin{corollary}\label{cor:C_alpha_j_inv_comp_renewal} Let $\alpha$ be a non-empty positive admissible word and $j \neq \alpha_{|\alpha|-1}$. Then,
\begin{equation*}
    C_{\alpha j^{-1}}^c = \begin{cases}
        C_{\alpha (\alpha_{|\alpha|-1} -1)}^c, \quad \alpha_{|\alpha|-1} > 1 \text{ and } j = 1,\\
        C_{\alpha (j-1)}^c, \quad \alpha_{|\alpha|-1} = 1,\\
        X_A, \quad \text{otherwise}
    \end{cases}
\end{equation*}
\end{corollary}

\begin{proof} It is straightforward from the proof of the corollary \ref{cor:C_alpha_j_inv_renewal}. \qed
\end{proof}

\begin{remark} By the proposition \ref{prop:general_C_alpha_complement} we have
\begin{equation}\label{eq:c_alpha_inverse_comp_renewal}
    C_{\alpha j^{-1}}^c = \begin{cases}
        F_{\alpha (\alpha_{|\alpha|-1} -1)}\sqcup\bigsqcup_{m=0}^{|\alpha|}\bigsqcup_{k\neq ({\alpha (\alpha_{|\alpha|-1} -1)})_m} C_{\delta^m({\alpha (\alpha_{|\alpha|-1} -1)})k}, \quad \alpha_{|\alpha|-1} > 1 \text{ and } j = 1,\\
        F_{\alpha(j-1)}\sqcup\bigsqcup_{m=0}^{|\alpha|} \bigsqcup_{k\neq (\alpha (j-1))_m} C_{\delta^m(\alpha (j-1))k}, \quad \alpha_{|\alpha|-1} = 1,\\
        X_A, \quad \text{otherwise}.
    \end{cases}
\end{equation}
\end{remark}



The previous results lead to the conclusion that the generators studied on the general shift are, when we specify the theory to the renewal shift, are the cylinders on positive words and their complements. Moreover, we just need to consider those words ending with `$1$'. We consider the topological basis of the finite intersections of these sets, and in order to identify how these intersections are, we present their pairwise intersections on the next corollary.
















\section{Empty stems and extremal conformal measures on $Y_A$}

As in the previous section, now we shall study conformal measures which live in $Y_A$, but for shifts that have more than one configuration with empty stem. The reader will notice some similarities with the renewal shift example. Due to corollary \ref{thm:uniqueness_conformal_probabilities_Y_A_families}, we have at most a bijection between the number of extremal conformal probability measures living on $Y_A$ and configurations with empty stem. However, for generalized shifts as the renewal or with similar construction, as the pair and prime renewal shifts, we observe that, for lower temperatures and potentials bounded away from zero, we have in fact a bijection between the extremal conformal measures living on $Y_A$ and the family of empty stem configurations, see theorems \ref{thm:pair_renewal_general_phase_transition_conditions} and \ref{theorem:infinite_conformal_measures}.

LALALALALALAALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALALA

Let us consider the measures $\mu_\beta$, $\beta > \log 2$, which live on $Y_A$ associated to the potential $1$. These measures are given by the coefficients in \eqref{eq:conformal_measure_Y_A_explicit}. Since for every admissible word $\alpha$ we have that $C_\alpha = C_{\hat{\alpha}}$, we only consider the case that $\alpha$ ends with $1$. Hence,
\begin{equation*}
    \mu_\beta(C_\alpha) = \sum_{\omega \in Y_A: \alpha \in \llbracket\omega\rrbracket} c_\omega^\beta,
\end{equation*}
and then,
\begin{equation*}
    \mu_\beta(C_\alpha) = \sum_{n \in \mathbb{N}}\sum_{\substack{\omega \in Y_A: \alpha \in \llbracket\omega\rrbracket \\ |\omega| = n}} c_n^\beta,
\end{equation*}
where
\begin{equation*}
    c_n^\beta := \frac{e^\beta-2}{e^{n \beta }(e^\beta-1)}.
\end{equation*}
However, if $\alpha \in \llbracket \omega \rrbracket$ then $|\omega|\geq |\alpha|$ and hence
\begin{equation*}
    \mu_\beta(C_\alpha) = \sum_{n = |\alpha|}^\infty\sum_{\substack{\omega \in Y_A: \alpha \in \llbracket\omega\rrbracket \\ |\omega| = n}} c_n^\beta.
\end{equation*}
\begin{lemma} Let $\omega \in Y_A$ s.t. $\alpha \in \llbracket \omega \rrbracket$. Write $n=|\omega| = |\alpha| + p$, $p \in \mathbb{N}_0$. If $p=0$, then there exists a unique word in $Y_A$ s.t. $\alpha \in \llbracket \omega \rrbracket$. If $p \in \mathbb{N}$, then there are $2^{p-1}$ words in $Y_A$ which satisfies $\alpha \in \llbracket \omega \rrbracket$.
\end{lemma}

\begin{proof} If $p=0$, the result is obvious, then suppose that $p \in \mathbb{N}$, that is, $|\omega|>|\alpha|$. Then, $\omega = \alpha \gamma$, where both $\alpha$ and $\gamma$ end with `$1$' and $|\gamma|=p$ and therefore the number of possibilities for $\gamma$, and consequently $\omega$, is $2^{p-1}$ due to the proposition \ref{prop:cardinality_words_length}.\qed
\end{proof}

By the lemma above we have that
\begin{equation*}
    \mu_\beta(C_\alpha) = c_{|\alpha|}^\beta + \sum_{n=|\alpha|+1}^\infty 2^{n-|\alpha|-1}c_n^\beta = c_{|\alpha|}^\beta + \sum_{k=1}^\infty 2^{k-1}c_{k + |\alpha|}^\beta,
\end{equation*}
where in the last equality we used the change of index $k = n-|\alpha|$ in the sum. It follows that
\begin{align*}
    \mu_\beta(C_\alpha) &= \frac{e^\beta-2}{e^\beta-1}\left[\frac{1}{e^{|\alpha|\beta}} + \sum_{k=1}^\infty \frac{2^{k-1}}{e^{(k + |\alpha|)\beta}}\right] =  e^{-|\alpha|\beta}.
\end{align*}
By taking the limit, we get
\begin{align*}
    \lim_{\beta \to \log 2}\mu_\beta(C_\alpha) &= 2^{-|\alpha|}.
\end{align*}
Before we proceed the calculation of the limit above for the remaining elements of $\mathcal{B}$, we will show that $\lim_{\beta \to \log 2}\mu_\beta(F)=0$, for every finite $F\subset Y_A$, which implies that the limit for the basic elements can be evaluated just by ignoring the part which is not a union of generalized cylinders and that if there exists the limit measure, then in fact it lives only in $\Sigma_A$.

As we discussed in the section \ref{sec:conformal_renewal}, any $\xi \in Y_A$ is in the form $\alpha \xi^0$, $\alpha$ positive admissible word ending with $1$. 
We calculate the following limit,
\begin{align*}
   \lim_{\beta \to \log 2}\mu_\beta(\{\alpha\xi^0\})=\lim_{\beta \to \log 2} \frac{e^\beta-2}{e^{|\alpha|\beta}(e^\beta-1)}=0.
\end{align*}
This implies that for finite $F\subset Y_A$, $\lim_{\beta\to \log 2}\mu(F)=0$ and hence for any clopen of $\mathcal{B}$ which is in the form
\begin{equation*}
    F\sqcup \bigsqcup_{p \in \mathbb{N}} \widetilde{C}_p, 
\end{equation*}
where $F \subseteq Y_A$ is finite and $\tilde{C}_p$ are pairwise disjoint generalized cylinders which are associated to words ending with 1 we have that
\begin{align}\label{eq:limit_mu_beta_complement}
    \lim_{\beta \to \log 2}\mu_\beta\left(F\sqcup \bigsqcup_{p \in \mathbb{N}} \widetilde{C}_p\right) &= \lim_{\beta \to \log 2}\mu_\beta \left(\bigsqcup_{p \in \mathbb{N}} \widetilde{C}_p\right) = \lim_{\beta \to \log 2}\sum_{p\in \mathbb{N}}\mu_\beta \left(\widetilde{C}_p\right) = \sum_{p\in \mathbb{N}}\lim_{\beta \to \log 2}\mu_\beta \left(\widetilde{C}_p\right).
\end{align}

Now we will compare this result with the measure of Sarig's work, which we call $\nu$. We recall that $\nu$ is a probability living on $\Sigma_A$ which is an eigenmeasure of the Ruelle operator $L_F$ with eigenvalue $e^{P_G(F)}$, where $P_G$ is the Gurevich pressure for the potential $F$. On our case, for the potential $F = \beta f$, $f=1$, we have that $\nu$ is the same unique eigenmeasure for all $\beta \in \mathbb{R}_+^*$. We have that $P_G(\beta) = \log 2 + \beta$ and then
\begin{equation*}
    2e^\beta \int f d\nu = \int L g d\nu, \quad g \in L^1(\nu),
\end{equation*}
where $L$ is the Ruelle operator for $F = 1$. Before we proceed, we observe that for any $n \in \mathbb{N}$ it follows that
\begin{equation}\label{eq:eigenmeasure_n_times}
    (2e^\beta)^n \int f d\nu = \int L^n g d\nu, \quad g \in L^1(\nu),
\end{equation}
and that 
\begin{equation}\label{eq:Ruelle_n_times}
    (L^n g)(x)  = \sum_{\sigma^n(y)=x}e^{\beta(S_n1)(y)}g(y) = \sum_{\sigma^n(y)=x}e^{\beta n}g(y) \quad \nu-\text{a.e.}, \quad g\in L^1(\nu).
\end{equation}
And for any $\alpha \in W_A$ ending with $1$ we get
\begin{align*}
    (2e^\beta)^{|\alpha|}\nu(C_\alpha) &= (2e^\beta)^{|\alpha|}\nu([\alpha]) \stackrel{\text{\eqref{eq:eigenmeasure_n_times}}}{=} \sum_{a \in \mathbb{N}}\int_{[a]} L^{|\alpha|} \mathbbm{1}_{[\alpha]} d\nu \stackrel{\text{\eqref{eq:Ruelle_n_times}}}{=} \sum_{a \in \mathbb{N}}\int_{[a]} \sum_{\sigma^{|\alpha|}(y)=x}e^{\beta|\alpha|} \mathbbm{1}_{[\alpha]}(y) d\nu(x).
\end{align*}
Now we claim that for given $a \in \mathbb{N}$, it follows that
\begin{equation*}
    \sum_{\sigma^{|\alpha|}(y)=x} \mathbbm{1}_{[\alpha]}(y) = 1, \quad x \in [a].
\end{equation*}
Indeed, the system of equations
\begin{equation*}
    \begin{cases}
        \mathbbm{1}_{[\alpha]}(y) = 1,\\
        \sigma^{|\alpha|}(y)=x;
    \end{cases}
\end{equation*}
admits the unique solution $y=\alpha x$ for all $x \in \mathbb{N}^{\mathbb{N}_0}$. Since $\alpha \in W_A$, such solution belongs to $[a]$ if and only if $A(\alpha_{|\alpha|-1},a)=1$, which is trivially satisfied since $\alpha_{|\alpha|-1}=1$. The claim is proved and consequently we get
\begin{align*}
    2^{|\alpha|}\nu(C_\alpha) &= \sum_{a \in \mathbb{N}}\int_{[a]} 1 d\nu(x) = \nu(\Sigma_A) = 1.
\end{align*}
Therefore,
\begin{equation*}
    \nu(C_\alpha) = 2^{-|\alpha|}
\end{equation*}
and finally
\begin{equation*}
    \nu(C_\alpha) = \lim_{\beta \to \log 2}\mu_\beta(C_\alpha)
\end{equation*}



%\begin{proposition}\label{prop:Z_alpha_j_inv_renewal} Consider the set $X_A$ of the renewal Markov shift. For any $\alpha$ positive admissible word, $|\alpha|\neq 0$, and any $j \in \mathbb{N}$, we have that $C_{\alpha j^{-1}}$ is the empty set or $C_{\alpha j^{-1}} = C_\gamma$, where $\gamma$ is a positive admissible word.
%\end{proposition}
%\begin{proof} If $j = \alpha_{|\alpha|-1}$ then the statement is obvious. So consider $j \neq \alpha_{|\alpha|-1}$. We have two cases as follows.
%\textbf{Case I:} $\alpha$ does not end with $1$. We have that $\alpha = \alpha_0 \cdots p$, $p \neq 1$. By the convexity and the fact that $\xi_e=1$ e have that $\xi_{\alpha j^{-1}}=1$ implies that $\xi_\alpha =1$. Define $\gamma:= \alpha (p-1)(p-2) \cdots 1$. It is straightforward to see that $C_\alpha = C_\gamma$. Hence, we have that $\xi_{\alpha j^{-1}} = 1$ if and only if $\xi_\gamma = 1$ and $A(j,\gamma_{|\alpha|})=A(j,p-1)=1$. We conclude that
%\begin{equation*}
 %   C_{\alpha j^{-1}} = \begin{cases}
  %                      C_\gamma, \quad \text{if }A(j,p-1)=1;\\
   %                     \emptyset, \quad \text{otherwise}.
    %                  \end{cases}
%\end{equation*}
%\textbf{Case II:} $\alpha$ does end with $1$. We recall that we have necessarily that $\xi_\alpha =1$. For given $\xi \in C_{\alpha j^{-1}}$ we have two possibilities, namely $\alpha = \kappa(\xi)$ or $\alpha \in \llbracket \kappa(\xi) \rrbracket \setminus \{\kappa(\xi)\}$. We claim that the first case never happens. Indeed, if $\alpha = \kappa(\xi)$ then $R_\xi(\alpha) = \{1\}$, hence $\xi_{\alpha j^{-1}}=1$ if and only if $j =1$, which was already excluded in the beginning of the proof. Now we deal with the second case. The assertion $\alpha \in \llbracket \kappa(\xi) \rrbracket \setminus \{\kappa(\xi)\}$ is equivalent to the statement that there exists $k \in \mathbb{N}$ s.t. $\xi_{\alpha k}=1$. Then, $\xi \in C_{\alpha j^{-1}}$ if and only if $A(j,k)=1$, which occurs if and only if $k=j-1$. We conclude that
%\begin{equation*}
 %   C_{\alpha j^{-1}} = C_{\alpha (j-1)}
%\end{equation*}
%and the proof is complete.
%\end{proof}
%From this point, for given positive admissible words $\alpha$ and $\gamma$ we define the finite sets \newline $F_\alpha := \{\alpha'\xi^0\in Y_A: \alpha' \in  \llbracket \alpha \rrbracket\setminus\{\alpha\}\}$ and $F_\gamma^\alpha := \{\gamma'\xi^0 \in F_\gamma: \alpha \in \llbracket \gamma' \rrbracket\}$. Note that $F_\gamma^\gamma = \emptyset$ and that $F_\gamma^\alpha = \emptyset$ if $\alpha \notin \llbracket\gamma\rrbracket$. Also define 
%\begin{equation*}
 %   \hat{\alpha} := \begin{cases}
  %                      \alpha, \quad \alpha = e \text{ or } \alpha_{|\alpha|-1} = 1,\\
   %                     \alpha (\alpha_{|\alpha|-1}-1) \cdots 1, \quad \text{otherwise};
    %                \end{cases}
%\end{equation*}
%i.e., the completion of $\alpha$ to the first time reaching the symbol 1. We notice that $F_\alpha = F_{\hat{\alpha}}$. Indeed, if $\alpha = e$ or $\alpha$ ends with 1 we conclude it directly from the definition of completion. On other hand, take $\xi \in F_{\hat{\alpha}}$, that is, $\xi = \gamma'\xi^0$ for some $\gamma' \in \llbracket \hat{\alpha} \rrbracket \setminus\{\hat{\alpha}\}$. If $\gamma' \notin \llbracket \alpha \rrbracket \setminus\{\alpha\}$ then $\gamma = \hat{\alpha}$ because there is only one 1 after $\alpha$, leading to a contradiction. The opposite inclusion is straightforward.
%\begin{proposition}\label{prop:Z_alpha_complement} The sets $C_\alpha^c$, $\alpha$ positive admissible with $|\alpha|>0$ can be written in the following form
%\begin{equation}\label{eq:Z_alpha_complement}
 %   C_\alpha^c = F_\alpha \sqcup \bigsqcup_{m=0}^{|\alpha|-1}\left(\bigsqcup_{k\neq \alpha_m}C_{\delta^m(\alpha)k}\right),
%\end{equation}    
 %   where $\delta^n:=\alpha_0\cdots\alpha_{n-1}$ (we understand $\delta^0$ being the element $e$).
%\end{proposition}
%\begin{proof} Let $\xi\in C_\alpha^c$, i.e, $\xi_\alpha=0$; then the set $\{m\in \mathbb{N}: \xi_{\delta^m(\alpha)}=0, m\leq |\alpha|\}$ is non empty, thus, by the well-ordering principle, have a least element, which we call $n$. We must have $\xi_{\delta^{n-1}(\alpha)}=1$; thus we either have that $|\kappa(\xi)|=n-1$, which implies that $\xi=\delta^{n-1}(\alpha)\xi^{0}$ or $|\kappa(\xi)|>n-1$, which implies that there exists a $k$ such that $\xi_{\delta^{n-1}(\alpha)k}=1$. Observe that $k\neq \alpha_{n-1}$, since if it was, it would be in contradiction with $\xi_{\delta^{n}(\alpha)}=0$. In the first possibility, $\xi\in F_\alpha$. In the second one, $\xi\in C_{\delta^{n-1}(\alpha)k}$, which was taken into account on the right hand side of \eqref{eq:Z_alpha_complement}. The opposite inclusion is straightforward. \qed
%\end{proof} 
%The next lemma will help us out to characterize the some important intersections of the elements of the basis which we will use later. In order to prove the lemma below, we present identity
%\begin{equation}\label{eq:C_cap_C}
    %C_\alpha \cap C_\gamma = \begin{cases}
     %                           C_\alpha, \quad \text{if } \gamma \in \llbracket \alpha \rrbracket,\\
      %                          C_\gamma, \quad \text{if } \alpha \in \llbracket \gamma \rrbracket,\\
       %                         \emptyset, \quad \text{otherwise};
        %                    \end{cases} 
%\end{equation}
%which holds for every $\alpha$ and $\gamma$ positive admissible words.
%\begin{lemma}\label{lemma:CF_intersections} For any two positive admissible words $\alpha$ and $\gamma$ it is true that
%\begin{itemize}
 %   \item[$(i)$]
  %  \begin{equation*}
   %     C_\alpha \cap F_\gamma =  F_{\gamma}^{\alpha};
    %\end{equation*}
    %\item[$(ii)$] 
    %\begin{equation*}
     %   F_\alpha \cap F_\gamma = \begin{cases}
    %                                F_\alpha, \quad \alpha \in \llbracket \gamma \rrbracket,\\
    %                                F_\gamma, \quad \gamma \in \llbracket \alpha \rrbracket,\\
     %                               F_{\alpha'}^*, \quad \text{otherwise},
      %                           \end{cases}
    %\end{equation*}
    %where $\alpha'$ is the longest word in $\llbracket \alpha \rrbracket \cap \llbracket \gamma \rrbracket$ and $k \in \mathbb{N}$;
    %\item[$(iii)$] for fixed $n \in \mathbb{N}$ with $n \in \{0,1,...,|\gamma|-1\}$, let be the natural number $j \neq \gamma_n$. We have
    %\begin{equation*}
     %   C_\alpha \cap C_{\delta^{n}(\gamma)j} = \begin{cases}
                         %C_{\delta^{n}(\gamma)j}, \quad            \alpha \in \llbracket             \gamma \rrbracket                 \text{ and } n \geq               |\alpha|,\\
                              %              C_\alpha, \quad                   \alpha \notin                     \llbracket \gamma                 \rrbracket,                        \gamma \notin                     \llbracket \alpha                 \rrbracket, n =                  |\alpha'| \text{ and }           j=\alpha_{|\alpha'|},           \\
                              %              \emptyset, %\quad                  \text{otherwise};
                               %          \end{cases}
    %\end{equation*}
    %where $\alpha'$ is the biggest word in $\llbracket \alpha \rrbracket \cap \llbracket \gamma \rrbracket$ which is a stem.
%\end{itemize}
%\end{lemma}
%\begin{proof} For $(i)$, we have that
%\begin{align*}
 %   C_\alpha \cap F_\gamma &= \{\xi \in X_A: \xi_\alpha = 1\} \cap \{\gamma'\xi^0\in Y_A: \gamma' \in  \llbracket \gamma \rrbracket\setminus\{\gamma\}\}\\
  %  &= \{\gamma'\xi^0 \in F_\gamma: (\gamma'\xi^0)_\alpha = 1\} = \{\gamma'\xi^0 \in F_\gamma: \alpha \in \llbracket \gamma'\rrbracket\} = F_\gamma^\alpha
%\end{align*}
%the result is immediate for $\alpha \neq \llbracket \gamma \rrbracket$, so let $\alpha \in \llbracket \gamma \rrbracket$, which is equivalent to say that $\alpha \in \llbracket \gamma' \rrbracket$ for every $\gamma' \in \llbracket \gamma \rrbracket$ such that $|\gamma'|\geq |\alpha|$, hence
%\begin{equation*}
 %   C_\alpha \cap F_\gamma = \{\gamma'\xi^0 \in F_\gamma: |\gamma'|=|\alpha|\} = F_\gamma^{|\alpha|}.
%\end{equation*}
%Now, for proof of $(ii)$, we notice from the definition of $F_\alpha$ that 
%\begin{equation*}
 %   F_\alpha\cap F_\gamma = \left\{\gamma'\xi^0 \in Y_A: \gamma'\in (\llbracket\alpha\rrbracket \cap \llbracket\gamma\rrbracket)\setminus\{\alpha,\gamma\}\right\}.
%\end{equation*}
%If $\alpha \in \llbracket\gamma\rrbracket$ then $\llbracket\alpha\rrbracket \subseteq \llbracket \gamma \rrbracket$ and therefore $(\llbracket\alpha\rrbracket \cap \llbracket\gamma\rrbracket)\setminus\{\alpha,\gamma\}= \llbracket\alpha\rrbracket\setminus\{\alpha\}$. In this case, we obtain $F_\alpha\cap F_\gamma = F_\alpha$. A similar proof holds for the case that $\gamma \in \llbracket \alpha \rrbracket$. The remaining possibility occurs when $\alpha \notin \llbracket\gamma\rrbracket$ is simultaneous to $\gamma \notin \llbracket \alpha \rrbracket$, and here we consider $\alpha'$ as in the statement. It follows immediately that $(\llbracket\alpha\rrbracket \cap \llbracket\gamma\rrbracket)\setminus\{\alpha,\gamma\}= \llbracket \alpha'\rrbracket$, since we only must have $|\alpha'|<\min\{|\alpha|,|\gamma|\}$. Moreover, $\alpha'$ is $e$ or it does end with 1, because $e$ and words ending with $1$ are the unique positive words which can be connected with more than one symbol still being admissible. We conclude that $\xi=\gamma' \xi^0  \in F_\alpha\cap F_\gamma$ if and only if $\gamma' \in \llbracket\alpha'\rrbracket$ and therefore $F_\alpha\cap F_\gamma = F_{\alpha'}^*$, for any $k \in \mathbb{N}$. 
%To prove $(iii)$ we use \eqref{eq:C_cap_C} and obtain
%\begin{equation*}
 %   C_\alpha \cap C_{\delta^{n}(\gamma)j} = \begin{cases}
  %                              C_\alpha, \quad \text{if } \delta^{n}(\gamma)j \in \llbracket \alpha \rrbracket,\\
   %                             C_{\delta^{n}(\gamma)j}, \quad \text{if } \alpha \in \llbracket \delta^{n}(\gamma)j \rrbracket,\\
    %                            \emptyset, \quad \text{otherwise}.
     %                       \end{cases} 
%\end{equation*}
%When $\alpha \in \llbracket \gamma \rrbracket$ it never occurs that $\delta^{n}(\gamma) j \in \llbracket \alpha \rrbracket$, for any $n$ and $j$. Indeed, if $\delta^{n}(\gamma) j \in \llbracket \alpha \rrbracket$ then $\delta^{n}(\gamma) j = \alpha_0 \cdots \alpha_n$ and $n \leq |\alpha|-1$, and consequently $j = \alpha_n = \gamma_n$, a contradiction. If $\alpha \in \llbracket \delta^{n}(\gamma) j \rrbracket$ and $n \geq |\alpha|$, then $C_\alpha \supseteq C_{\delta^{n}(\gamma)j}$ and $C_\alpha \cap C_{\delta^{n}(\gamma)j} = C_{\delta^{n}(\gamma)j}$. On other hand, if $n < |\alpha|$ then it is clear that $C_\alpha \cap C_{\delta^{n}(\gamma)j} = \emptyset$ since $j \neq \alpha_n$. Now, let us consider $\alpha \notin \llbracket \gamma \rrbracket$, which implies that $|\alpha|>0$ because, otherwise, we would get $\alpha = e$, which is subword of every positive admissible word. If $\gamma \in \llbracket \alpha \rrbracket$, observe that $\delta^{n}(\gamma)j \notin \llbracket \alpha \rrbracket$ because $j \neq \gamma_n = \alpha_n$, and hence $C_{\delta^{n}(\gamma)j} \subseteq C_\alpha^c$, that is, $C_{\delta^{n}(\gamma)j} \cap C_\alpha = \emptyset$. For the case that $\gamma \notin \llbracket \alpha \rrbracket$, let $\alpha'$ be the biggest word of $\llbracket \alpha \rrbracket \cap \llbracket \gamma \rrbracket$ which ends with 1 or it is the word $e$ as we concluded before. If $n = |\alpha'|$ and $j=\alpha_{|\alpha'|}$, then it follows directly that $C_\alpha \subseteq C_{\delta^{n}(\gamma)j}$ and hence $C_\alpha \cap C_{\delta^{n}(\gamma)j}= C_\alpha$. If $n = |\alpha'|$ and $j\neq\alpha_{|\alpha'|}$ then it is clear that $C_\alpha \cap C_{\delta^{n}(\gamma)j}= \emptyset$. Now, if $n < |\alpha'|$, then also occurs $C_\alpha \cap C_{\delta^{n}(\gamma)j}= \emptyset$ because $j \neq \gamma_n = \alpha'_n$. The same happens for $n > |\alpha'|$ since $\alpha \notin \llbracket \gamma' \rrbracket$ for any $\gamma' \in \llbracket\gamma\rrbracket$ with $|\gamma'|>|\alpha|$.\qed
%\end{proof}
%\begin{proposition}\label{prop:Z_intersections} For any $\alpha$ and $\gamma$ positive admissible words, we have the following.
%\begin{align}
 %   C_\alpha \cap C_\gamma^c &= \begin{cases}
  %                              F_{\gamma}^{\alpha}\sqcup \bigsqcup_{n=|\alpha|}^{|\gamma|-1} \bigsqcup_{j\neq \gamma_n} C_{\delta^{n}(\gamma)j},\quad \alpha \in \llbracket \gamma \rrbracket,\\
   %                             C_\alpha,\quad \alpha \notin \llbracket \gamma \rrbracket \text{ and } \gamma \notin \llbracket \alpha \rrbracket, \\
    %                            \emptyset, \quad \text{otherwise};
                               %\end{cases}\label{eq:C_cap_C_comp}\\
    %C_\alpha^c \cap C_\gamma^c &= \begin{cases}
     %                               C_\alpha^c, \quad \alpha \in \llbracket \gamma \rrbracket,\\
      %                              C_\gamma^c, \quad \gamma \in \llbracket \alpha \rrbracket,\\
       %                             F_{\alpha'}^* \sqcup F_\alpha^{\alpha'\alpha_{|\alpha'|}} \sqcup F_\gamma^{\alpha'\gamma_{|\alpha'|}} \sqcup  \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{j=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_j}C_{\delta^{m}(\alpha)k} \cap C_{\delta^{n}(\gamma)j}\right), \quad \text{otherwise}. \end{cases}\label{eq:C_comp_cap_C_comp}
%\end{align}
%\end{proposition}
%\begin{proof} First we prove \eqref{eq:C_cap_C_comp}. Let $\alpha \in \llbracket \gamma \rrbracket$, then by the proposition \ref{prop:Z_alpha_complement} we have that
%\begin{equation*}
 %   C_\alpha \cap C_\gamma^c = (C_\alpha \cap F_\gamma) \sqcup \bigsqcup_{n=0}^{|\gamma|-1}\left(\bigsqcup_{j\neq \gamma_n}C_\alpha \cap C_{\delta^{n}(\gamma)j}\right).
%\end{equation*}
%By the lemma \ref{lemma:CF_intersections} $(i)$ and $(iii)$ it is clear that \eqref{eq:C_cap_C_comp} holds for this case. Similarly the same proof holds for when $\alpha \notin \llbracket \gamma \rrbracket \text{ and } \gamma \notin \llbracket \alpha \rrbracket$. If $\gamma \in \llbracket \alpha \rrbracket$ then for every $\xi \in C_\alpha$ we have that $\xi_\gamma = 1$ and therefore $\xi \notin C_\gamma^c$, implying that $C_\alpha \cap C_\gamma^c= \emptyset$. Now, to prove \eqref{eq:C_comp_cap_C_comp}, we notice that if $\alpha \in \llbracket \gamma \rrbracket$ is equivalent to affirm that $C_\alpha \supseteq C_\gamma$, which is equivalent to state that $C_\alpha^c \subseteq C_\gamma^c$ and hence $C_\alpha^c \cap C_\gamma^c = C_\alpha^c$. A similar proof is used when $\gamma \in \llbracket \alpha \rrbracket$. The last case, when  $\alpha \notin \llbracket\gamma\rrbracket$ and $\gamma \notin \llbracket \alpha \rrbracket$, gives us that
%\begin{align*}
 %   C_\alpha^c \cap C_\gamma^c &= (F_\alpha \cap F_\gamma) \sqcup \left(\bigsqcup_{n=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_n}F_\alpha \cap C_{\delta^{n}(\gamma)j}\right) \sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} F_\gamma \cap C_{\delta^{m}(\alpha)k} \right)\\
  %  &\sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{j=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_j}C_{\delta^{m}(\alpha)k} \cap C_{\delta^{n}(\gamma)j}\right).
%\end{align*}
%By the lemma \ref{lemma:CF_intersections} $(i)$ and $(ii)$ we obtain
%\begin{align*}
 %   C_\alpha^c \cap C_\gamma^c &= F_{\alpha'}^* \sqcup \left(\bigsqcup_{n=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_n}F_\alpha^{\delta^{n}(\gamma)j}\right) \sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} F_\gamma^{\delta^{m}(\alpha)k} \right)\\
 %   &\sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{j=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_j}C_{\delta^{m}(\alpha)k} \cap C_{\delta^{n}(\gamma)j}\right).
%\end{align*}
%Since $\alpha'$ is the largest word in $\llbracket \alpha \rrbracket \cap \llbracket \gamma \rrbracket$, which we recall that $\alpha=e$ or it ends with 1, we separate in the possibilities as follows. If $0 \leq m < |\alpha'|$ (for $|\alpha'|>0$), we have that $\delta^{m}(\alpha)k \notin \llbracket\gamma'\rrbracket$ for any $\gamma' \in \llbracket\gamma\rrbracket$ because $k \neq \alpha_m = \gamma_m$. The same occurs for $m = |\alpha'|$ with $k \neq \gamma_m$ and for $m > |\alpha'|$. If $m = |\alpha'|$ with $k = \gamma_m$, we have that $\delta^{m}(\alpha)k \in \llbracket\gamma'\rrbracket$ for every $\gamma' \in \llbracket\gamma\rrbracket\setminus \{\gamma\}$ s.t. $|\gamma'|\geq m+1$. Hence, 
%\begin{equation*}
 %   F_\gamma^{\delta^{m}(\alpha)k} = \begin{cases}
  %                          F_\gamma^{\alpha'\gamma_{|\alpha'|}}, \quad m=|\alpha'|, k = \gamma_m,\\
   %                         \emptyset, \quad \text{otherwise}.
    %                       \end{cases}
%\end{equation*}
%Analogously we obtain
%\begin{equation*}
 %   F_\alpha^{\delta^{n}(\gamma)j} = \begin{cases}
  %                          F_\alpha^{\alpha'\alpha_{|\alpha'|}}, \quad n=|\alpha'|, j = \alpha_n,\\
   %                         \emptyset, \quad \text{otherwise}.
    %                       \end{cases}
%\end{equation*}
%Therefore,
%\begin{align*}
 %   C_\alpha^c \cap C_\gamma^c &= F_{\alpha'}^* \sqcup F_\alpha^{\alpha'\alpha_{|\alpha'|}} \sqcup F_\gamma^{\alpha'\gamma_{|\alpha'|}} \sqcup  \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{j=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_j}C_{\delta^{m}(\alpha)k} \cap C_{\delta^{n}(\gamma)j}\right).
%\end{align*}\qed
%\end{proof} 



%The proposition \ref{prop:cylinder_reducing_inverse} reduces the quantity of generalized cylinders we need to deal to those related to positive words and positive words with at max one inverse letter from $\mathbb{F}$. If the cylinder is related to the last case, the proposition \ref{prop:Z_alpha_j_inv_renewal} allows us to writte it as a cylinder related to a positive word. On the other hand, the proposition \ref{prop:Z_alpha_complement} deal with the remaining case, that is, the complement of the positive cylinders. Also, the equation \eqref{eq:Z_alpha_complement} gives us that every complement of a generalized cylinder related to a positive admissible word $\alpha$ is a disjoint union of cylinders together with the finite set $F_\alpha$, the subwords strictly shorter than $\alpha$ which correspond to configurations in $Y_A$. Since the generalized cylinders are clopen, their complements are also clopen. In addition, we emphasize that the renewal shift imposes that for any $C_\alpha$ s.t. $\alpha$ is positive admissible and does not end with $1$ it follows that $C_\alpha = C_\gamma$, where $\gamma$ is the continuation of $\alpha$ ending on the first possible time which we may add the symbol $1$, therefore we may always suppose that $C_\alpha$ ends with $1$. Consider the family $\mathcal{B}$ of all finite intersections of the elements of the collection
%\begin{equation*}
 %   \left\{C_\alpha: \alpha \in W_A \text{ and } \alpha_{|\alpha|-1}=1\right\}\cup\left\{C_\alpha^c: \alpha \in W_A \text{ and } \alpha_{|\alpha|-1}=1\right\},
%\end{equation*}
%which is a topological basis of clopen sets for $X_A$ of the renewal shift and, of course, closed by finite intersections. The proposition \ref{prop:Z_intersections}, combined with \eqref{eq:C_cap_C}, gives a natural consequence: every element of $\mathcal{B}$ is a disjoint union of elements of $Y_A$ with a disjoint union of generalized cylinders. Now we calculate $\lim_{\beta \to \log 2} \mu_\beta(C_\alpha)$, for $\alpha$ finite admissible word ending with $1$.


%TEOREMAO DO CONJUNTAO


%\textbf{Proof of \eqref{eq:C_inverse_cap_C_inverse_comp}:} we have that
%\begin{align*}
%    C_{\alpha j^{-1}} \cap C_{\gamma l^{-1}}^c &= (G(\alpha,j) \cap K(\gamma,l)) \sqcup (G(\alpha,j) \cap F_\gamma) \sqcup \left( \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} G(\alpha,j) \cap C_{\delta^n(\gamma)p} \right) \\
%    &\sqcup \left( \bigsqcup_{m:A(l,m)=0} G(\alpha,j) \cap C_{\gamma m} \right)\sqcup \left( \bigsqcup_{k:A(j,k)=1}  C_{\alpha k} \cap K(\gamma,l)\right) \\
%    &\sqcup \left( \bigsqcup_{k:A(j,k)=1}  C_{\alpha k} \cap F_\gamma\right) \sqcup \left( \bigsqcup_{k:A(j,k)=1} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\alpha k} \cap C_{\delta^n(\gamma)p}\right)\\
%    &\sqcup \left( \bigsqcup_{k:A(j,k)=1} \bigsqcup_{m:A(l,m)=0} C_{\alpha k} \cap C_{\gamma m}\right)
%\end{align*}
%due to the propositions \ref{prop:general_C_alpha_inverse_j} and \ref{prop:general_C_alpha_j_inverse_complement}. By definition of $GK(\alpha,j,l)$ we have that
%\begin{equation*}
%    G(\alpha,j) \cap K(\gamma,l) = \begin{cases}
%    GK(\alpha,j,l), \quad \alpha = \gamma,\\
%    \emptyset, \quad \text{otherwise}.
%    \end{cases}
%\end{equation*}
%The lemma \ref{lemma:CF_intersections_general} $(viii)$ gives
%\begin{equation*}
%    G(\alpha,j) \cap F_\gamma = \begin{cases}
%    G(\alpha,j), \quad \alpha \in \llbracket\gamma\rrbracket \setminus \{\gamma\},\\
%    \emptyset, \quad \text{otherwise}.
%    \end{cases}
%\end{equation*}
%From the lemma \ref{lemma:CF_intersections_general} $(iv)$ we have
%\begin{equation*}
%    G(\alpha,j) \cap C_{\delta^n(\gamma)p} = \begin{cases}
%        G(\gamma,j), \quad \delta^n(\gamma)p \in \llbracket \alpha \rrbracket,\\
%        \emptyset, \quad \text{otherwise};
%    \end{cases}
%\end{equation*}
%and from the lemma \ref{lemma:CF_intersections_general} $(i)$ we get
%\begin{equation*}
%    C_{\alpha k} \cap F_{\gamma} = F_{\gamma}^{\alpha k},
%\end{equation*}
%which is empty if\footnote{It can be empty even satisfying the opposite of the conditions stated, but these cases are included in the definition of the $F$'s, we are just simplyfing the statements.} $\alpha \notin \llbracket \gamma \rrbracket\setminus \{\gamma\}$ or $k \neq \gamma_{|\alpha|}$, and then
%\begin{equation*}
%    \bigsqcup_{k:A(j,k)=1}  C_{\alpha k} \cap F_\gamma = \begin{cases}
%        F_\gamma^{\alpha \gamma_{|\alpha|}}, \quad \alpha \in \llbracket \gamma \rrbracket\setminus\{\gamma\} \text{ and } A(j,\gamma_{|\alpha|}) = 1,\\
%        \emptyset, \quad \text{otherwise}.
%    \end{cases}
%\end{equation*}

%If $\gamma \in \llbracket \alpha \rrbracket$, then $\delta^n(\gamma)p \notin \llbracket \alpha \rrbracket$ because $p \neq \gamma_n = \alpha_n$. The same happens when $\alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\}$ and $n \leq |\alpha| -1$. Now, if $\alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\}$ and $n < |\alpha| -1$ we have also that $\delta^n(\gamma)p \notin \llbracket \alpha \rrbracket$ because we must have $p \neq \gamma_n = \alpha_n$. The last possibility consists in $\alpha \notin \llbracket \gamma \rrbracket$ and $\gamma \notin \llbracket \alpha \rrbracket$, where we consider $\alpha'$, the longest word in $\llbracket \alpha \rrbracket \cap \llbracket \gamma \rrbracket$. We have the same result as before, except when $n = |\alpha'|$, where it is straightforward that $\delta^n(\gamma)p \in \llbracket \alpha \rrbracket$ if and only if $p = \alpha_{|\alpha'|} \neq \gamma_{|\alpha'|}$. We conclude that
%\begin{equation}\label{eq:union_intersection_G_C_delta}
%    \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} G(\alpha,j) \cap C_{\delta^n(\gamma)p} = \begin{cases}
%        G(\alpha,j), \quad \alpha \notin \llbracket \gamma \rrbracket, \text{ }\gamma \notin \llbracket \alpha \rrbracket,\\
%        \emptyset, \quad \text{otherwise}.
%    \end{cases}
%\end{equation}

%The intersection $C_{\gamma m} \cap G(\alpha,j)$ was already explicited in \eqref{eq:G_alpha_j_cap_C_gamma_m} and therefore
%\begin{equation*}
%    \bigsqcup_{m:A(l,m)=0} G(\alpha,j) \cap C_{\gamma m} = \begin{cases}
%        G(\alpha,j), \quad \gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\} \text{ and } A(l,\alpha_{|\gamma|}) = 0,\\
%        \emptyset, \quad \text{otherwise}.
%    \end{cases}
%\end{equation*}
%We also have
%\begin{equation*}
%     C_{\alpha k} \cap K(\gamma,l) = \begin{cases}
%        K(\gamma,l), \quad \alpha \in \llbracket \gamma \rrbracket\setminus \{\gamma\} \text{ and } k=\gamma_{|\alpha|},\\
%        \emptyset, \quad \text{otherwise},
%    \end{cases}
%\end{equation*}
%which is proved similarly as in \eqref{eq:C_alpha_k_cap_G_gamma_j} and gives
%\begin{equation}\label{eq:union_C_alpha_k_cap_K}
%     \bigsqcup_{k:A(j,k)=1}  C_{\alpha k} \cap K(\gamma,l) = \begin{cases}
%        K(\gamma,l), \quad \alpha \in \llbracket \gamma \rrbracket\setminus \{\gamma\} \text{ and } A(j,\gamma_{|\alpha|}) = 1,\\
%        \emptyset, \quad \text{otherwise}.
%    \end{cases}
%\end{equation}
%Now, if $\alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\}$, then by \eqref{eq:C_german_equals_triple_union} we have that
%\begin{equation*}
%    \mathfrak{C}[\gamma,\alpha,j] = \bigsqcup_{k:A(j,k)=1} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\alpha k} \cap C_{\delta^n(\gamma)p}.
%\end{equation*}
%The remaining case, when $\alpha \notin  \llbracket \gamma \rrbracket \setminus \{\gamma\}$, is separated into two possibilities, namely $\gamma \in  \llbracket \alpha \rrbracket$ and $\gamma \notin  \llbracket \alpha \rrbracket$. For the first one, we have necessarily that $\delta^n(\gamma) \in \llbracket \alpha \rrbracket \setminus \{\alpha\}$ for every $n$ possible. Since $p \neq \gamma_n = \alpha_n$, we conclude that $ C_{\alpha k} \cap C_{\delta^n(\gamma)p} = \emptyset$ for every $n$ and $k$ and therefore
%\begin{equation*}
%    \bigsqcup_{k:A(j,k)=1} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\alpha k} \cap C_{\delta^n(\gamma)p} = \emptyset.
%\end{equation*}
%The second case is equivalent to the condition $\gamma \notin \llbracket \alpha \rrbracket$ and $\alpha %\notin \llbracket \gamma \rrbracket$, and we have that
%\begin{equation*}
%    C_{\delta^n(\gamma)p}\cap C_{\alpha k} = \begin{cases}
%        C_{\alpha k}, \quad n = |\alpha'| \text{ and } p = \alpha_{|\alpha'|},\\
%        \emptyset, \quad \text{otherwise};    \end{cases}
%\end{equation*}
%obtained from lemma \ref{lemma:CF_intersections_general} $(iii)$ and considering that %$C_{\delta^n(\gamma)p}\cap C_{\alpha k} = (C_{\delta^n(\gamma)p}\cap C_{\alpha})\cap C_{\alpha k}$. %Therefore, in this case we have
%\begin{equation*}
%    \bigsqcup_{k:A(j,k)=1} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\alpha k} \cap C_{\delta^n(\gamma)p} = \bigsqcup_{k:A(j,k)=1} C_{\alpha k}.
%\end{equation*}
%Summarizing, we get
%\begin{equation}\label{eq:triple_union_C_alpha_k_C_delta}
%    \bigsqcup_{k:A(j,k)=1} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\alpha k} \cap C_{\delta^n(\gamma)p} = \begin{cases}
%        \mathfrak{C}[\gamma,\alpha,j], \quad \alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\},\\
%        \bigsqcup_{k:A(j,k)=1} C_{\alpha k}, \quad \alpha \notin \llbracket \gamma \rrbracket \text{ and } \gamma \notin \llbracket \alpha \rrbracket,\\
%        \emptyset, \quad \text{otherwise}.
%    \end{cases}
%\end{equation}
%From \eqref{eq:C_alpha_k_cap_C_gamma_m} we obtain
%\begin{equation}\label{eq:double_union_matix_conditions}
%    \bigsqcup_{k:A(j,k)=1} \bigsqcup_{m:A(l,m)=0} C_{\alpha k} \cap C_{\gamma m} = \begin{cases}
%        \bigsqcup_{k:A(j,k) = 1, A(l,k)=0}C_{\alpha k}, \quad \alpha = \gamma, \\
%        \bigsqcup_{m:A(l,m)=0}  C_{\gamma m}, \quad \alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\} \text{ and }A(j,\gamma_{|\alpha|}) = 1,\\
%        \bigsqcup_{k:A(j,k)=1}  C_{\alpha k}, \quad \gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\} \text{ and }A(l,\alpha_{|\gamma|}) = 0,\\
%        \emptyset, \quad \text{otherwise}.
%    \end{cases} 
%\end{equation}


\textbf{Proof of \eqref{eq:C_inverse_comp_cap_C_inverse_comp}:} proposition \ref{prop:general_C_alpha_j_inverse_complement} gives
\begin{align*}
    C_{\alpha j^{-1}}^c \cap C_{\gamma l^{-1}}^c &= (K(\alpha,j) \cap K(\gamma,l)) \sqcup (K(\alpha,j) \cap F_\gamma) \sqcup \left(\bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} K(\alpha,j) \cap C_{\delta^n(\gamma)p} \right) \\
    &\sqcup \left(\bigsqcup_{p:A(l,p)=0} K(\alpha,j) \cap C_{\gamma p} \right) \sqcup (F_\alpha \cap K(\gamma,l)) \sqcup (F_\alpha \cap F_\gamma) \\
    &\sqcup \left(\bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} F_\alpha \cap C_{\delta^n(\gamma)p} \right) \sqcup \left( \bigsqcup_{p:A(l,p)=0} F_\alpha \cap C_{\gamma p}\right)\\
    &\sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} C_{\delta^m(\alpha)k} \cap K(\gamma,l)\right) \sqcup \left( \bigsqcup_{m=0}^{|\alpha|-1} \bigsqcup_{k \neq \alpha_m} C_{\delta^m(\alpha)k} \cap F_\gamma \right) \\
    &\sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\delta^m(\alpha)k} \cap C_{\delta^n(\gamma) p}\right)
    \sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{p:A(l,p)=0}   C_{\delta^m(\alpha)k} \cap C_{\gamma p} \right)\\
    &\sqcup \left(\bigsqcup_{k:A(j,k)=0}  C_{\alpha k} \cap K(\gamma,l) \right) \sqcup \left(\bigsqcup_{k:A(j,k)=0}  C_{\alpha k} \cap F_\gamma \right) \\
    &\sqcup \left(\bigsqcup_{k:A(j,k)=0} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\alpha k} \cap C_{\delta^n(\gamma)p}\right) \sqcup \left(\bigsqcup_{k:A(j,k)=0} \bigsqcup_{p:A(l,p)=0} C_{\alpha k} \cap C_{\gamma p} \right).
\end{align*}
The lemma \ref{lemma:CF_intersections_general} $(vii)$ gives
\begin{equation*} 
    K(\alpha,j) \cap K(\gamma,l) = \begin{cases}
                        K(\alpha,\{j,l\}), \quad \alpha = \gamma,\\
                        \emptyset, \quad \text{otherwise}.
                        \end{cases}
\end{equation*}
Also we have
\begin{equation*}
    K(\alpha,j) \cap F_\gamma = \begin{cases}
                        K(\alpha,j), \quad \alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\},\\
                        \emptyset, \quad \text{otherwise};
                        \end{cases}
\end{equation*}
and 
\begin{equation*}
    F_\alpha \cap K(\gamma,l)  = \begin{cases}
                        K(\gamma,l), \quad \gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\},\\
                        \emptyset, \quad \text{otherwise};
                        \end{cases}
\end{equation*}
due to the lemma \ref{lemma:CF_intersections_general} $(ix)$. In addition,
\begin{equation*} 
    \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} K(\alpha,j) \cap C_{\delta^n(\gamma)p} = \begin{cases}
        K(\alpha,j), \quad \alpha \notin \llbracket \gamma \rrbracket, \text{ }\gamma \notin \llbracket \alpha \rrbracket,\\
        \emptyset, \quad \text{otherwise};
         \end{cases}
\end{equation*}
and
\begin{equation*} 
    \bigsqcup_{n=0}^{|\alpha|-1} \bigsqcup_{k \neq \alpha_k} C_{\delta^m(\alpha)k} \cap K(\gamma,l) = \begin{cases}
        K(\gamma,l), \quad \alpha \notin \llbracket \gamma \rrbracket, \text{ }\gamma \notin \llbracket \alpha \rrbracket,\\
        \emptyset, \quad \text{otherwise};
         \end{cases}
\end{equation*}
due to a similar proof as it was done to prove \eqref{eq:union_intersection_G_C_delta}. In analogous way, the identities
\begin{equation*}
    \bigsqcup_{p:A(l,p)=0} K(\alpha,j) \cap C_{\gamma p} = \begin{cases}
        K(\alpha,j), \quad \gamma \in \llbracket \alpha \rrbracket\setminus \{\alpha\} \text{ and } A(l,\alpha_{|\gamma|}) = 0,\\
        \emptyset, \quad \text{otherwise};
        \end{cases}
\end{equation*}
and
\begin{equation*}
    \bigsqcup_{k:A(j,k)=0}  C_{\alpha k} \cap K(\gamma,l) = \begin{cases}
        K(\gamma,l), \quad \alpha \in \llbracket \gamma \rrbracket\setminus \{\gamma\} \text{ and } A(j,\gamma_{|\alpha|}) = 0,\\
        \emptyset, \quad \text{otherwise}.
    \end{cases}
\end{equation*}
are proved similarly to what is done to proof \eqref{eq:union_C_alpha_k_cap_K}. As presented in the lemma \ref{lemma:CF_intersections_general} $(ii)$,
\begin{equation*}
        F_\alpha \cap F_\gamma = \begin{cases}
                                    F_\alpha, \quad \alpha \in \llbracket \gamma \rrbracket,\\
                                    F_\gamma, \quad \gamma \in \llbracket \alpha \rrbracket,\\
                                    F_{\alpha'}^*, \quad \text{otherwise}.
                                 \end{cases}
\end{equation*}
Moreover, by the lemma \ref{lemma:CF_intersections_general} $(i)$ we have
\begin{equation*}
    F_\alpha \cap C_{\delta^n(\gamma)p} = \begin{cases}
                                 F_\alpha^{\alpha'\alpha_{|\alpha'|}}, \quad \alpha \notin \llbracket \gamma \rrbracket \setminus \{\gamma\}, \quad  \gamma \notin \llbracket \alpha \rrbracket \setminus \{\alpha\} \text{ and } n = |\alpha'|\\
                                 \emptyset, \quad \text{otherwise};
                                 \end{cases}
\end{equation*}
and the proof is straightforward for $\alpha \notin \llbracket \gamma \rrbracket \setminus \{\gamma\} \text{ and }  \gamma \notin \llbracket \alpha \rrbracket \setminus \{\alpha\}$. For $\alpha = \gamma$, the proof is the same as for $\gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\}$ and for $\alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\}$ with $0 \leq n < |\alpha|-1$, because in all these cases we have $p \neq \gamma_n = \alpha_n$. For the remaining case, $\alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\}$ and $n \geq |\alpha|-1$ it follows that $|\delta^n(\gamma)p|\geq |\alpha|$, however for every $\xi \in F_\alpha$ it is true that $|\kappa(\xi)| \leq |\alpha|-1$ and therefore $F_\alpha \cap C_{\delta^n(\gamma)p} = \emptyset$ for this case. Then,
\begin{equation*}
    \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} F_\alpha \cap C_{\delta^n(\gamma)p} =  \begin{cases}
        F_\alpha^{\alpha'\alpha_{|\alpha'|}}, \quad \alpha \notin \llbracket \gamma \rrbracket \setminus \{\gamma\} \text{ and } \gamma \notin \llbracket \alpha \rrbracket \setminus \{\alpha\},\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
and
\begin{equation*}
    \bigsqcup_{m=0}^{|\alpha|-1} \bigsqcup_{k \neq \alpha_m} C_{\delta^m(\alpha)k} \cap F_\gamma =  \begin{cases}
        F_\gamma^{\alpha'\gamma_{|\alpha'|}}, \quad \alpha \notin \llbracket \gamma \rrbracket \setminus \{\gamma\} \text{ and } \gamma \notin \llbracket \alpha \rrbracket \setminus \{\alpha\},\\
        \emptyset, \quad \text{otherwise}.
    \end{cases}
\end{equation*}
On the other hand, the lemma \ref{lemma:CF_intersections_general} $(i)$ gives\footnote{It may happen that $\gamma$ is the longest word in $\llbracket \alpha \rrbracket \setminus \{\alpha\}$. In this case we have $F_\alpha^{\gamma p} = F_\alpha^\alpha = \emptyset$.}
\begin{equation*}
    F_\alpha \cap C_{\gamma p} = \begin{cases}
        F_\alpha^{\gamma p}, \quad \gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\} \text{ and } p=\alpha_{|\gamma|},\\
        \emptyset, \quad \text{otherwise}.
    \end{cases}
\end{equation*}
Hence, we have
\begin{equation*}
    \bigsqcup_{p:A(l,p)=0} F_\alpha \cap C_{\gamma p} = \begin{cases}
        F_\alpha^{\gamma \alpha_{|\gamma|}}, \quad \gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\} \text{ and } A(l,\alpha_{|\gamma|})=0,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
and
\begin{equation*}
    \bigsqcup_{k:A(j,k)=0}  C_{\alpha k} \cap F_\gamma = \begin{cases}
        F_\gamma^{\alpha \gamma_{|\alpha|}}, \quad \alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\} \text{ and } A(j,\gamma_{|\alpha|})=0,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
In addition,
\begin{equation*}
    \bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{p:A(l,p)=0}   C_{\delta^m(\alpha)k} \cap C_{\gamma p} = \begin{cases}
        \mathfrak{D}[\alpha,\gamma,l], \quad \gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\},\\
        \bigsqcup_{p:A(l,p)=0} C_{\gamma p}, \quad \alpha \notin \llbracket \gamma \rrbracket \text{ and } \gamma \notin \llbracket \alpha \rrbracket,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
and
\begin{equation*}
    \bigsqcup_{k:A(j,k)=0} \bigsqcup_{n=0}^{|\gamma|-1} \bigsqcup_{p \neq \gamma_n} C_{\alpha k} \cap C_{\delta^n(\gamma)p} = \begin{cases}
        \mathfrak{D}[\gamma,\alpha,j], \quad \alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\},\\
        \bigsqcup_{k:A(j,k)=0} C_{\alpha k}, \quad \alpha \notin \llbracket \gamma \rrbracket \text{ and } \gamma \notin \llbracket \alpha \rrbracket,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
as analogously we proved \eqref{eq:triple_union_C_alpha_k_C_delta}. Also we have
\begin{equation*}
    \bigsqcup_{k:A(j,k)=0} \bigsqcup_{p:A(l,p)=0} C_{\alpha k} \cap C_{\gamma p} = \begin{cases}
        \bigsqcup_{k:A(j,k) = 0, A(l,k)=0}C_{\alpha k}, \quad \alpha = \gamma, \\
        \bigsqcup_{m:A(l,m)=0}  C_{\gamma m}, \quad \alpha \in \llbracket \gamma \rrbracket \setminus \{\gamma\} \text{ and }A(j,\gamma_{|\alpha|}) = 0,\\
        \bigsqcup_{k:A(j,k)=0}  C_{\alpha k}, \quad \gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\} \text{ and }A(l,\alpha_{|\gamma|}) = 0,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}
\end{equation*}
analogous to the proof of \eqref{eq:double_union_matix_conditions}. The remaining parcel
\begin{align*}
    \bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{n=0}^{|\gamma|-1}\bigsqcup_{p\neq \gamma_n}  C_{\delta^m(\alpha)k} \cap C_{\delta^n(\gamma )p}
\end{align*}
was already studied in the corollary \ref{cor:4_tuple_union_delta}.


\textbf{Proof of \eqref{eq:C_inverse_cap_C_inverse}:} proposition \ref{prop:general_C_alpha_inverse_j} gives
\begin{align*}
    C_{\alpha j^{-1}} \cap C_{\gamma l^{-1}} &= (G(\alpha,j) \cap G(\gamma,l)) \sqcup \left(\bigsqcup_{m:A(l,m)=1} G(\alpha,j) \cap C_{\gamma m} \right) \\
    &\sqcup \left(\bigsqcup_{k:A(j,k)=1} C_{\alpha k} \cap G(\gamma,l) \right) \sqcup \bigsqcup_{k:A(j,k)=1} \bigsqcup_{m:A(l,m)=1} C_{\alpha k} \cap C_{\gamma m}.
\end{align*}
The proof is concluded by taking by applying the lemma \ref{lemma:CF_intersections_general} $(iv)$ and $(vi)$ in order to obtain
\begin{align}
    G(\alpha,j) \cap G(\gamma,l) = \begin{cases}
        G(\alpha,\{j,l\}), \quad \alpha = \gamma,\\
        \emptyset, \quad \text{otherwise};
    \end{cases}\nonumber\\
    G(\alpha,j) \cap C_{\gamma m} = \begin{cases}
        G(\alpha,j), \quad \gamma \in \llbracket\alpha \rrbracket\setminus \{\alpha\} \text{ and } m=\alpha_{|\gamma|},\\
        \emptyset, \quad \text{otherwise};
    \end{cases}\label{eq:G_alpha_j_cap_C_gamma_m}\\
   C_{\alpha k} \cap G(\gamma,l) = \begin{cases}
        G(\gamma,l), \quad \alpha \in \llbracket \gamma \rrbracket\setminus \{\gamma\} \text{ and } k=\gamma_{|\alpha|},\\
        \emptyset, \quad \text{otherwise};
    \end{cases}\label{eq:C_alpha_k_cap_G_gamma_j}
\end{align}
and by noticing that
\begin{align} \label{eq:C_alpha_k_cap_C_gamma_m}
     C_{\alpha k} \cap C_{\gamma m} = \begin{cases}
        C_{\alpha k}, \quad \gamma \in \llbracket\alpha \rrbracket\setminus \{\alpha\} \text{ and } m=\alpha_{|\gamma|},\\
        C_{\gamma m}\quad \alpha \in \llbracket \gamma \rrbracket\setminus \{\gamma\} \text{ and } k=\gamma_{|\alpha|},\\
        C_{\alpha k} = C_{\gamma m}, \quad \alpha = \gamma \text{ and } k = m,\\
        \emptyset, \quad \text{otherwise}.
    \end{cases}
\end{align}


\textbf{Proof of \eqref{eq:C_comp_cap_C_comp}:} we notice that if $\alpha \in \llbracket \gamma \rrbracket$ is equivalent to affirm that $C_\alpha \supseteq C_\gamma$, which is equivalent to state that $C_\alpha^c \subseteq C_\gamma^c$ and hence $C_\alpha^c \cap C_\gamma^c = C_\alpha^c$. A similar proof is used when $\gamma \in \llbracket \alpha \rrbracket$. For the last case, when  $\alpha \notin \llbracket\gamma\rrbracket$ and $\gamma \notin \llbracket \alpha \rrbracket$, we write
\begin{align*}
    C_\alpha^c \cap C_\gamma^c &= (F_\alpha \cap F_\gamma) \sqcup \left(\bigsqcup_{n=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_n}F_\alpha \cap C_{\delta^{n}(\gamma)j}\right) \sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} F_\gamma \cap C_{\delta^{m}(\alpha)k} \right)\\
    &\sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} \bigsqcup_{j=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_j}C_{\delta^{m}(\alpha)k} \cap C_{\delta^{n}(\gamma)j}\right).
\end{align*}
By the lemma \ref{lemma:CF_intersections_general} $(i)$ and $(ii)$ and the corollary \ref{cor:4_tuple_union_delta} we obtain
\begin{align*}
    C_\alpha^c \cap C_\gamma^c &= F_{\alpha'}^* \sqcup \left(\bigsqcup_{n=0}^{|\gamma|-1}\bigsqcup_{j\neq \gamma_n}F_\alpha^{\delta^{n}(\gamma)j}\right) \sqcup \left(\bigsqcup_{m=0}^{|\alpha|-1}\bigsqcup_{k\neq \alpha_m} F_\gamma^{\delta^{m}(\alpha)k} \right)\\
    &\sqcup \left(\bigsqcup_{m = 0}^{|\alpha|-1} \bigsqcup_{k\neq \alpha_m} C_{\delta^m(\alpha)k}\right) \sqcup \left(\bigsqcup_{|\alpha'| < n < |\gamma|-1} \bigsqcup_{p\neq \gamma_n} C_{\delta^n(\gamma )p}\right).
\end{align*}
Since $\alpha'$ is the largest word in $\llbracket \alpha \rrbracket \cap \llbracket \gamma \rrbracket$, we separate in the possibilities as follows. If $0 \leq m < |\alpha'|$ (for $|\alpha'|>0$), we have that $\delta^{m}(\alpha)k \notin \llbracket\kappa(\xi)\rrbracket$ for any $\xi \in Y_A$ such that $\kappa(\xi) \in \llbracket\gamma\rrbracket$ because $k \neq \alpha_m = \gamma_m$. The same occurs for $m = |\alpha'|$ with $k \neq \gamma_m$ and for $m > |\alpha'|$. If $m = |\alpha'|$ with $k = \gamma_m$, we have that $\delta^{m}(\alpha)k \in \llbracket\kappa(\xi)\rrbracket$ for every $\xi \in Y_A$ such that $\kappa(\xi) \in \llbracket\gamma\rrbracket\setminus\{\gamma\}$ and $|\kappa(\xi)|\geq m+1$. Hence, 
\begin{equation*}
    F_\gamma^{\delta^{m}(\alpha)k} = \begin{cases}
                            F_\gamma^{\alpha'\gamma_{|\alpha'|}}, \quad m=|\alpha'|, k = \gamma_m,\\
                            \emptyset, \quad \text{otherwise}.
                           \end{cases}
\end{equation*}
Analogously we obtain
\begin{equation*}
    F_\alpha^{\delta^{n}(\gamma)j} = \begin{cases}
                            F_\alpha^{\alpha'\alpha_{|\alpha'|}}, \quad n=|\alpha'|, j = \alpha_n,\\
                            \emptyset, \quad \text{otherwise}.
                           \end{cases}
\end{equation*}
Therefore,
\begin{align*}
    C_\alpha^c \cap C_\gamma^c &= F_{\alpha'}^* \sqcup F_\alpha^{\alpha'\alpha_{|\alpha'|}} \sqcup F_\gamma^{\alpha'\gamma_{|\alpha'|}} \sqcup  \left(\bigsqcup_{m = 0}^{|\alpha|-1} \bigsqcup_{k\neq \alpha_m} C_{\delta^m(\alpha)k}\right) \sqcup \left(\bigsqcup_{|\alpha'| < n < |\gamma|-1} \bigsqcup_{p\neq \gamma_n} C_{\delta^n(\gamma )p}\right).
\end{align*}

\textbf{Proof\footnote{Alternatively, the equality can be proved by using the lemma \ref{lemma:CF_intersections_general}.} of \eqref{eq:C_cap_C_inverse}:} if $\alpha \in \llbracket \gamma \rrbracket$, then it is straightforward that $C_{\gamma j^{-1}} \subseteq C_{\gamma} \subseteq C_\alpha$ and hence $C_\alpha \cap C_{\gamma j^{-1}}=C_{\gamma j^{-1}}$. A similar argument follows when $\gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\} \text{ and } A(j,\alpha_{|\gamma|})=1$, leading to $C_{\gamma j^{-1}} \supseteq C_\alpha$. If $\alpha \notin \llbracket \gamma \rrbracket$ and $\gamma \notin \llbracket \alpha \rrbracket \setminus \{\alpha\}$ it is straighforward that $C_{\gamma j^{-1}}^c \supseteq C_\alpha$, and the same happens when $\gamma \in \llbracket \alpha \rrbracket \setminus \{\alpha\}$ and $A(j,\alpha_{|\gamma|})=0$.




==> prop_fixed.tex <==
\textbf{Case I:} $\alpha$ does not end with $1$. Writing $\alpha = \alpha_0 \cdots p$, $p > 1$, define $\gamma:= \alpha (p-1)(p-2) \cdots 1$. It is straightforward that $C_\alpha = C_\gamma$. Let $\xi \in C_{\alpha j^{-1}}$, then $\xi_\alpha = 1$ and, since $C_\alpha = C_\gamma$, we have that $\xi_\gamma=1$, proving $C_{\alpha j^{-1}}\subseteq C_\gamma$. First, suppose that $A(j,\gamma_{|\alpha|})=1$. Take $\xi \in C_\gamma$, since $\xi_\alpha = \xi_{\alpha \gamma_{|\alpha|}}=1$ we use \eqref{eq:equiv_past_filled} in order to obtain $\xi \in C_{\alpha j^{-1}}$, that is $C_{\alpha j^{-1}}=C_\gamma$. Now, if $A(j,\gamma_{|\alpha|})=0$, consider $\xi \in C_{\alpha j^{-1}}$ and hence $\xi_\gamma = 1$. However, again by \eqref{eq:equiv_past_filled} it is true that $\xi_{\alpha j^{-1}}=0$, a contradiction. We conclude that $C_{\alpha j^{-1}}=\emptyset$.

\textbf{Case II:} $\alpha$ does end with $1$. For given $\xi \in C_{\alpha j^{-1}}$ we have again that $\xi_\alpha =1$. If $\alpha = \kappa(\xi)$ then $R_\xi(\alpha) = \{1\}$, and we deduce that $\xi_{\alpha j^{-1}}=1$ holds if and only if $j=1=\alpha_{|\alpha|-1}$, which is out of our assumptions. Thus for each $\xi \in C_{\alpha j^{-1}}$ there exists $p = p(\xi) \in \mathbb{N}$ such that $\xi_{\alpha p}=1$. The equivalence \eqref{eq:equiv_past_filled} and the renewal shift matrix imposes that $\xi_{\alpha j^{-1}}=1$ if and only if $p = j-1$ because $j-1$ is the unique value which $A(j,p)=1$ holds, so $C_{\alpha j^{-1}}\subseteq C_{\alpha (j-1)}$. The opposite inclusion follows because for every $\xi \in C_{\alpha (j-1)}$ we have that $A(j,j-1)=1$ and $\xi_{\alpha j^{-1}}=1$ immediately holds because \eqref{eq:equiv_past_filled}, concluding that $C_{\alpha j^{-1}} = C_{\alpha (j-1)}$.


